Holomorphic Hartree-Fock theory: an inherently multireference approach

We investigate the existence of holomorphic Hartree-Fock solutions using a revised SCF algorithm. We use this algorithm to study the Hartree-Fock solutions for H$_{2}$ and H$_{4}^{2+}$ and report the emergence of holomorphic solutions at points of symmetry breaking. Finally, we find these holomorphic solutions for H$_{4}$ and use them as a basis for Non-Orthogonal Configuration Interaction at a range of rectangular geometries and show them to produce energies in good agreement with Full Configuration Interaction.

==> H2standard/graphData <==
(lp0
(F0.10000000000000009
(lp1
F2.715887
aFnan
aFnan
a(lp2
cnumpy.core.multiarray
scalar
p3
(cnumpy
dtype
p4
(S'f8'
p5
I0
I1
tp6
Rp7
(I3
S'<'
p8
NNNI-1
I-1
I0
tp9
bS'p\xb9E+#\xba\x05@'
p10
tp11
Rp12
aFnan
aFnan
a(lp13
F2.709960769681468
aF4.5866131825263725
aF4.89895370072149
aF6.831072750323683
atp14
a(F0.10999999999999988
(lp15
F2.242039
aFnan
aFnan
a(lp16
g3
(g7
S'A\xc8if\xb2\xef\x01@'
p17
tp18
Rp19
aFnan
aFnan
a(lp20
F2.2360593400736564
aF4.09759054316002
aF4.410188391277358
aF6.327113375599449
atp21
a(F0.1200000000000001
(lp22
F1.848938
aFnan
aFnan
a(lp23
g3
(g7
S'\xa8n\x96n@\x95\xfd?'
p24
tp25
Rp26
aFnan
aFnan
a(lp27
F1.842899603015322
aF3.688159980043121
aF4.00103878385224
aF5.901614042110543
atp28
a(F0.1299999999999999
(lp29
F1.518053
aFnan
aFnan
a(lp30
g3
(g7
S'\xc4\x8a(k\xf1I\xf8?'
p31
tp32
Rp33
aFnan
aFnan
a(lp34
F1.5119499306948465
aF3.3398598399978923
aF3.6530429913540705
aF5.5361830640460905
atp35
a(F0.14000000000000012
(lp36
F1.236136
aFnan
aFnan
a(lp37
g3
(g7
S'\xc4\x8ed\x176\xc7\xf3?'
p38
tp39
Rp40
aFnan
aFnan
a(lp41
F1.2299640981433733
aF3.0395163306936706
aF3.3530269700372717
aF5.217719069420714
atp42
a(F0.1499999999999999
(lp43
F0.993465
aFnan
aFnan
a(lp44
g3
(g7
S'\xc0\xedx\xebv\xca\xef?'
p45
tp46
Rp47
aFnan
aFnan
a(lp48
F0.987219400017895
aF2.7774809410943107
aF3.0913419406448894
aF4.9366477232207515
atp49
a(F0.16000000000000014
(lp50
F0.78274
aFnan
aFnan
a(lp51
g3
(g7
S'\xc0S8L5\x0c\xe9?'
p52
tp53
Rp54
aFnan
aFnan
a(lp55
F0.7764155735803145
aF2.5465286829202505
aF2.8607626306140714
aF4.685819286306144
atp56
a(F0.16999999999999993
(lp57
F0.598371
aFnan
aFnan
a(lp58
g3
(g7
S'\x1c\xfaa\xd7\xdb%\xe3?'
p59
tp60
Rp61
aFnan
aFnan
a(lp62
F0.5919624254993672
aF2.3411450606680804
aF2.655774244885818
aF4.459794927653009
atp63
a(F0.17999999999999972
(lp64
F0.436003
aFnan
aFnan
a(lp65
g3
(g7
S'xa\x85\x15{\xe7\xdb?'
p66
tp67
Rp68
aFnan
aFnan
a(lp69
F0.429504993150028
aF2.1570506097342714
aF2.4720970048635498
aF4.254370638242759
atp70
a(F0.18999999999999995
(lp71
F0.292192
aFnan
aFnan
a(lp72
g3
(g7
S'`<\xcdME\xb3\xd2?'
p73
tp74
Rp75
aFnan
aFnan
a(lp76
F0.2855987202846417
aF1.9908754901934904
aF2.3063607430685904
aF4.066251241921886
atp77
a(F0.19999999999999973
(lp78
F0.164175
aFnan
aFnan
a(lp79
g3
(g7
S'0\xf4\x9d\xd0\xaf\x03\xc5?'
p80
tp81
Rp82
aFnan
aFnan
a(lp83
F0.15748213424198565
aF1.8399316297722006
aF2.1558770470304616
aF3.892822003115384
atp84
a(F0.20999999999999996
(lp85
F0.049712
aFnan
aFnan
a(lp86
g3
(g7
S'\xc0r]J\xe5s\xa9?'
p87
tp88
Rp89
aFnan
aFnan
a(lp90
F0.04291451625421627
aF1.7020499125839401
aF2.0184764489753593
aF3.73198533299065
atp91
a(F0.21999999999999975
(lp92
F-0.053034
aFnan
aFnan
a(lp93
g3
(g7
S"\x00v\x17\xf5K'\xab\xbf"
p94
tp95
Rp96
aFnan
aFnan
a(lp97
F-0.05994212260584397
aF1.5754617297916502
aF1.8923899774752095
aF3.582041913875511
atp98
a(F0.22999999999999998
(lp99
F-0.145587
aFnan
aFnan
a(lp100
g3
(g7
S'\x80\xeadw\x98\xa2\xc2\xbf'
p101
tp102
Rp103
aFnan
aFnan
a(lp104
F-0.1526102517140857
aF1.4587114025665302
aF1.7761615814229492
aF3.4416027545502237
atp105
a(F0.23999999999999977
(lp106
F-0.229219
aFnan
aFnan
a(lp107
g3
(g7
S'\x00\xbe\x837\x08W\xcd\xbf'
p108
tp109
Rp110
aFnan
aFnan
a(lp111
F-0.2363622118954401
aF1.3505904838034903
aF1.6685824327905894
aF3.309523183823068
atp112
a(F0.25
(lp113
F-0.305001
aFnan
aFnan
a(lp114
g3
(g7
S'\x18\xa8\xe4\xf5 \x85\xd3\xbf'
p115
tp116
Rp117
aFnan
aFnan
a(lp118
F-0.31226990312279634
aF1.2500878223053609
aF1.5686409918779591
aF3.184852665815795
atp119
a(F0.2599999999999998
(lp120
F-0.373843
aFnan
aFnan
a(lp121
g3
(g7
S'\x98\x17\x9c6\n\xed\xd7\xbf'
p122
tp123
Rp124
aFnan
aFnan
a(lp125
F-0.38124300269189865
aF1.1563511542384999
aF1.4754845998505801
aF3.0667962003447475
atp126
a(F0.27
(lp127
F-0.436522
aFnan
aFnan
a(lp128
g3
(g7
S'\xcc#K\x8f\xfb\xef\xdb\xbf'
p129
tp130
Rp131
aFnan
aFnan
a(lp132
F-0.4440586927477855
aF1.0686572405763501
aF1.3883896172787498
aF2.954684324721653
atp133
a(F0.2799999999999998
(lp134
F-0.493707
aFnan
aFnan
a(lp135
g3
(g7
S't\xf5\x06\xf5\xe6\x98\xdf\xbf'
p136
tp137
Rp138
aFnan
aFnan
a(lp139
F-0.5013850244219568
aF0.9863884200217256
aF1.306737978163606
aF2.847949583223687
atp140
a(F0.29000000000000004
(lp141
F-0.545975
aFnan
aFnan
a(lp142
g3
(g7
S'\xc2l\x1b2\xa1x\xe1\xbf'
p143
tp144
Rp145
aFnan
aFnan
a(lp146
F-0.5537994584687899
aF0.9090140335828003
aF1.22999861562064
aF2.7461079164798683
atp147
a(F0.2999999999999998
(lp148
F-0.593828
aFnan
aFnan
a(lp149
g3
(g7
S'H%y\x12\xa3\x00\xe3\xbf'
p150
tp151
Rp152
aFnan
aFnan
a(lp153
F-0.6018037110956456
aF0.8360755876453473
aF1.1577126260577075
aF2.6487438331575586
atp154
a(F0.31000000000000005
(lp155
F-0.637703
aFnan
aFnan
a(lp156
g3
(g7
S'P\x02Z\x89\x0fh\xe4\xbf'
p157
tp158
Rp159
aFnan
aFnan
a(lp160
F-0.6458357418583655
aF0.767174813836095
aF1.0894813301373152
aF2.5554985174220546
atp161
a(F0.31999999999999984
(lp162
F-0.677984
aFnan
aFnan
a(lp163
g3
(g7
S'\xd2\xa4_\xc4\x0b\xb2\xe5\xbf'
p164
tp165
Rp166
aFnan
aFnan
a(lp167
F-0.6862795107363906
aF0.701963993505852
aF1.0249565983467723
aF2.4660602349423737
atp168
a(F0.33000000000000007
(lp169
F-0.71501
aFnan
aFnan
a(lp170
g3
(g7
S'rEgx\\\xe1\xe6\xbf'
p171
tp172
Rp173
aFnan
aFnan
a(lp174
F-0.7234729789765654
aF0.6401380671091847
aF0.9638329614472847
aF2.380156552592143
atp175
a(F0.33999999999999986
(lp176
F-0.749079
aFnan
aFnan
a(lp177
g3
(g7
S'\x1ae\x9d\xbcs\xf8\xe7\xbf'
p178
tp179
Rp180
aFnan
aFnan
a(lp181
F-0.7577147161587948
aF0.5814281609353222
aF0.9058411382515817
aF2.297547999208357
atp182
a(F0.3500000000000001
(lp183
F-0.780455
aFnan
aFnan
a(lp184
g3
(g7
S'\xf8\x151\x8f|\xf9\xe8\xbf'
p185
tp186
Rp187
aFnan
aFnan
a(lp188
F-0.7892693926683757
aF0.5255962470709841
aF0.8507426966054437
aF2.2180228783590232
atp189
a(F0.3599999999999999
(lp190
F-0.809374
aFnan
aFnan
a(lp191
g3
(g7
S'\xd4\x94\x07xd\xe6\xe9\xbf'
p192
tp193
Rp194
aFnan
aFnan
a(lp195
F-0.8183723743437403
aF0.47243071513836704
aF0.7983256261110271
aF2.1413930069706635
atp196
a(F0.3700000000000001
(lp197
F-0.836046
aFnan
aFnan
a(lp198
g3
(g7
S'\xec\xbez\xa4\xe3\xc0\xea\xbf'
p199
tp200
Rp201
aFnan
aFnan
a(lp202
F-0.845233588876203
aF0.42174268187162794
aF0.7484006486505482
aF2.0674902015208887
atp203
a(F0.3799999999999999
(lp204
F-0.860659
aFnan
aFnan
a(lp205
g3
(g7
S'\xb2\xe0\xdb\xc3\x83\x8a\xeb\xbf'
p206
tp207
Rp208
aFnan
aFnan
a(lp209
F-0.8700407975591548
aF0.37336290095239444
aF0.7007981291257743
aF1.9961633702282424
atp210
a(F0.3900000000000001
(lp211
F-0.88338
aFnan
aFnan
a(lp212
g3
(g7
S'\x0eU\x9e\xdd\xa5D\xec\xbf'
p213
tp214
Rp215
aFnan
aFnan
a(lp216
F-0.8929623783508431
aF0.3271391635836802
aF0.6553654768880404
aF1.927276098159893
atp217
a(F0.3999999999999999
(lp218
F-0.904361
aFnan
aFnan
a(lp219
g3
(g7
S'\xd8\xdd\x93N\x87\xf0\xec\xbf'
p220
tp221
Rp222
aFnan
aFnan
a(lp223
F-0.9141497048421945
aF0.28293410210055014
aF0.6119649501530297
aF1.8607046344379834
atp224
a(F0.41000000000000014
(lp225
F-0.923739
aFnan
aFnan
a(lp226
g3
(g7
S':\x9b\xb3\x11F\x8f\xed\xbf'
p227
tp228
Rp229
aFnan
aFnan
a(lp230
F-0.9337391890671931
aF0.2406233260219802
aF0.5704717928007799
aF1.7963362082838827
atp231
a(F0.41999999999999993
(lp232
F-0.941637
aFnan
aFnan
a(lp233
g3
(g7
S'\x94t\xe5q\xe4!\xee\xbf'
p234
tp235
Rp236
aFnan
aFnan
a(lp237
F-0.9518540430621601
aF0.20009383344083
aF0.5307726464537298
aF1.734067614591499
atp238
a(F0.4299999999999997
(lp239
F-0.958166
aFnan
aFnan
a(lp240
g3
(g7
S'2\xa2\xc4<L\xa9\xee\xbf'
p241
tp242
Rp243
aFnan
aFnan
a(lp244
F-0.9686058037844877
aF0.16124265137181
aF0.49276419145024986
aF1.6738040208706375
atp245
a(F0.43999999999999995
(lp246
F-0.973428
aFnan
aFnan
a(lp247
g3
(g7
S'":\xee\x89Q&\xef\xbf'
p248
tp249
Rp250
aFnan
aFnan
a(lp251
F-0.9840956578686595
aF0.1239756672352501
aF0.45635197888793
aF1.6154579563816889
atp252
a(F0.44999999999999973
(lp253
F-0.987513
aFnan
aFnan
a(lp254
g3
(g7
S' \xc8\xf2&\xb5\x99\xef\xbf'
p255
tp256
Rp257
aFnan
aFnan
a(lp258
F-0.9984155961941316
aF0.08820662053489017
aF0.42144942279313
aF1.5589484515422307
atp259
a(F0.45999999999999996
(lp260
F-1.000507
aFnan
aFnan
a(lp261
g3
(g7
S'\x0b\xed\x9bZ\x13\x02\xf0\xbf'
p262
tp263
Rp264
aFnan
aFnan
a(lp265
F-1.0116494230439335
aF0.05385622933452032
aF0.3879769270194802
aF1.5042003015799834
atp266
a(F0.46999999999999975
(lp267
F-1.012485
aFnan
aFnan
a(lp268
g3
(g7
S']\xe7kB#3\xf0\xbf'
p269
tp270
Rp271
aFnan
aFnan
a(lp272
F-1.0238736404520705
aF0.0208514306294799
aF0.3558611259702594
aF1.45114343320959
atp273
a(F0.48
(lp274
F-1.023517
aFnan
aFnan
a(lp275
g3
(g7
S'Ql\xde\x9aS`\xf0\xbf'
p276
tp277
Rp278
aFnan
aFnan
a(lp279
F-1.0351582249518179
aF-0.010875282638150024
aF0.3250342218926301
aF1.3997123570290575
atp280
a(F0.48999999999999977
(lp281
F-1.033668
aFnan
aFnan
a(lp282
g3
(g7
S'\xfe2]\x93\xe7\x89\xf0\xbf'
p283
tp284
Rp285
aFnan
aFnan
a(lp286
F-1.0455673111882988
aF-0.04138644219554999
aF0.29543340446869026
aF1.3498456915358483
atp287
a(F0.5
(lp288
F-1.042996
aFnan
aFnan
a(lp289
g3
(g7
S'\xe5F\x9a\xdc\x1c\xb0\xf0\xbf'
p290
tp291
Rp292
aFnan
aFnan
a(lp293
F-1.0551597946206213
aF-0.07074011453465985
aF0.2670003408553201
aF1.301485747276541
atp294
a(F0.5099999999999998
(lp295
F-1.051556
aFnan
aFnan
a(lp296
g3
(g7
S'd\xcbs7,\xd3\xf0\xbf'
p297
tp298
Rp299
aFnan
aFnan
a(lp300
F-1.0639898636936964
aF-0.09899035034447978
aF0.2396807263163202
aF1.2545781617822367
atp301
a(F0.52
(lp302
F-1.059397
aFnan
aFnan
a(lp303
g3
(g7
S']6I\xf3I\xf3\xf0\xbf'
p304
tp305
Rp306
aFnan
aFnan
a(lp307
F-1.0721074703514517
aF-0.1261875815143003
aF0.21342388721433983
aF1.2090715776794911
atp308
a(F0.5299999999999998
(lp309
F-1.066565
aFnan
aFnan
a(lp310
g3
(g7
S'*\xb8\xcc]\xa6\x10\xf1\xbf'
p311
tp312
Rp313
aFnan
aFnan
a(lp314
F-1.0795587465009353
aF-0.15237897260342015
aF0.1881824294685602
aF1.164917357781745
atp315
a(F0.54
(lp316
F-1.073103
aFnan
aFnan
a(lp317
g3
(g7
S'\xbct\x14&n+\xf1\xbf'
p318
tp319
Rp320
aFnan
aFnan
a(lp321
F-1.0863863730019963
aF-0.17760873258491996
aF0.16391192667304022
aF1.1220693321083859
atp322
a(F0.5499999999999998
(lp323
F-1.079051
aFnan
aFnan
a(lp324
g3
(g7
S'\xca\x7fr\xb4\xcaC\xf1\xbf'
p325
tp326
Rp327
aFnan
aFnan
a(lp328
F-1.0926299068734286
aF-0.20191839176766005
aF0.14057064297438
aF1.0804835727023183
atp329
a(F0.56
(lp330
F-1.084444
aFnan
aFnan
a(lp331
g3
(g7
S'\xa4\xaehx\xe2Y\xf1\xbf'
p332
tp333
Rp334
aFnan
aFnan
a(lp335
F-1.0983260716800705
aF-0.22534704806994987
aF0.11811928653848994
aF1.0401181928527201
atp336
a(F0.5699999999999998
(lp337
F-1.089318
aFnan
aFnan
a(lp338
g3
(g7
S'2H\xe2-\xd9m\xf1\xbf'
p339
tp340
Rp341
aFnan
aFnan
a(lp342
F-1.103509015438403
aF-0.24793158620955996
aF0.09652079004508021
aF1.0009331679213527
atp343
a(F0.5800000000000001
(lp344
F-1.093704
aFnan
aFnan
a(lp345
g3
(g7
S'\x1eF\xb9\x1a\xd0\x7f\xf1\xbf'
p346
tp347
Rp348
aFnan
aFnan
a(lp349
F-1.1082105398488775
aF-0.2697068728788301
aF0.07574011514539022
aF0.962890175434427
atp350
a(F0.5899999999999999
(lp351
F-1.097632
aFnan
aFnan
a(lp352
g3
(g7
S'\xd5\xcemE\xe6\x8f\xf1\xbf'
p353
tp354
Rp355
aFnan
aFnan
a(lp356
F-1.112460304210782
aF-0.2907059305635001
aF0.055744078228359834
aF0.9259524524708811
atp357
a(F0.6000000000000001
(lp358
F-1.101128
aFnan
aFnan
a(lp359
g3
(g7
S'Z\x81\xdb\xa58\x9e\xf1\xbf'
p360
tp361
Rp362
aFnan
aFnan
a(lp363
F-1.1162860069811649
aF-0.31096009232511024
aF0.03650119518002996
aF0.8900846686629448
atp364
a(F0.6099999999999999
(lp365
F-1.10422
aFnan
aFnan
a(lp366
g3
(g7
S'J\x15\xa1P\xe2\xaa\xf1\xbf'
p367
tp368
Rp369
aFnan
aFnan
a(lp370
F-1.1197135476027908
aF-0.33049913958656046
aF0.017981543100999673
aF0.8552528133493402
atp371
a(F0.6200000000000001
(lp372
F-1.10693
aFnan
aFnan
a(lp373
g3
(g7
S',\x1c\xda\x9d\xfc\xb5\xf1\xbf'
p374
tp375
Rp376
aFnan
aFnan
a(lp377
F-1.1227671709242804
aF-0.3493514247248602
aF0.0001566371829800313
aF0.8214240955929806
atp378
a(F0.6299999999999999
(lp379
F-1.109283
aFnan
aFnan
a(lp380
g3
(g7
S'R7\xb9K\x9f\xbf\xf1\xbf'
p381
tp382
Rp383
aFnan
aFnan
a(lp384
F-1.125469596280778
aF-0.3675439800804401
aF-0.017000678860600058
aF0.7885668559094577
atp385
a(F0.6400000000000001
(lp386
F-1.111298
aFnan
aFnan
a(lp387
g3
(g7
S'\xb4\xba\x80\x9d\xe0\xc7\xf1\xbf'
p388
tp389
Rp390
aFnan
aFnan
a(lp391
F-1.127842133065166
aF-0.38510261482337005
aF-0.03351633024495021
aF0.7566504886554861
atp392
a(F0.6499999999999999
(lp393
F-1.112997
aFnan
aFnan
a(lp394
g3
(g7
S'r%Jw\xd5\xce\xf1\xbf'
p395
tp396
Rp397
aFnan
aFnan
a(lp398
F-1.12990478442215
aF-0.40205200097663035
aF-0.04941509774067026
aF0.7256453741085895
atp399
a(F0.6600000000000001
(lp400
F-1.114397
aFnan
aFnan
a(lp401
g3
(g7
S'\x8c\xcf\xffv\x91\xd4\xf1\xbf'
p402
tp403
Rp404
aFnan
aFnan
a(lp405
F-1.1316763405075814
aF-0.4184157497707003
aF-0.06472069464638015
aF0.695522819333161
atp406
a(F0.6699999999999999
(lp407
F-1.115516
aFnan
aFnan
a(lp408
g3
(g7
S"&S\xe1\n'\xd9\xf1\xbf"
p409
tp410
Rp411
aFnan
aFnan
a(lp412
F-1.1331744625973534
aF-0.43421647939817026
aF-0.07945583517112995
aF0.6662550069822831
atp413
a(F0.6799999999999997
(lp414
F-1.116371
aFnan
aFnan
a(lp415
g3
(g7
S'R\xe3\xe0\x85\xa7\xdc\xf1\xbf'
p416
tp417
Rp418
aFnan
aFnan
a(lp419
F-1.1344157591797694
aF-0.44947587513953996
aF-0.0936422951930797
aF0.6378149512300391
atp420
a(F0.69
(lp421
F-1.116977
aFnan
aFnan
a(lp422
g3
(g7
S'\x92\x88\x1e2#\xdf\xf1\xbf'
p423
tp424
Rp425
aFnan
aFnan
a(lp426
F-1.1354158550310094
aF-0.46421474274432023
aF-0.10730096627431995
aF0.6101764600696
atp427
a(F0.6999999999999997
(lp428
F-1.117349
aFnan
aFnan
a(lp429
g3
(g7
S'\x821\xbea\xa9\xe0\xf1\xbf'
p430
tp431
Rp432
aFnan
aFnan
a(lp433
F-1.1361894541563926
aF-0.47845305587431985
aF-0.12045190373419999
aF0.5833141032512229
atp434
a(F0.71
(lp435
F-1.117501
aFnan
aFnan
a(lp436
g3
(g7
S'\xb7\x19N~H\xe1\xf1\xbf'
p437
tp438
Rp439
aFnan
aFnan
a(lp440
F-1.1367503973721784
aF-0.4922099983439402
aF-0.13311436951205982
aF0.5572031851711493
atp441
a(F0.7199999999999998
(lp442
F-1.117445
aFnan
aFnan
a(lp443
g3
(g7
S'@-\xec\x16\x0e\xe1\xf1\xbf'
p444
tp445
Rp446
aFnan
aFnan
a(lp447
F-1.137111715203038
aF-0.5055040018238801
aF-0.14530687048213986
aF0.531819722059178
atp448
a(F0.73
(lp449
F-1.117194
aFnan
aFnan
a(lp450
g3
(g7
S'&\x15S\xed\x06\xe0\xf1\xbf'
p451
tp452
Rp453
aFnan
aFnan
a(lp454
F-1.1372856766835928
aF-0.5183527796130603
aF-0.1570471928217598
aF0.5071404228513727
atp455
a(F0.7399999999999998
(lp456
F-1.116759
aFnan
aFnan
a(lp457
g3
(g7
S'\xca-\xf2\x01?\xde\xf1\xbf'
p458
tp459
Rp460
aFnan
aFnan
a(lp461
F-1.1372838345738225
aF-0.5307733570246403
aF-0.1683524329754601
aF0.4831426731724125
atp462
a(F0.75
(lp463
F-1.116151
aFnan
aFnan
a(lp464
g3
(g7
S'\xd9\xf4.\x9f\xc1\xdb\xf1\xbf'
p465
tp466
Rp467
aFnan
aFnan
a(lp468
F-1.1371170674299849
aF-0.5427820988782903
aF-0.17923902570453037
aF0.4598045218925052
atp469
a(F0.7599999999999998
(lp470
F-1.115381
aFnan
aFnan
a(lp471
g3
(g7
S"'\xb6\xe9c\x99\xd8\xf1\xbf"
p472
tp473
Rp474
aFnan
aFnan
a(lp475
F-1.1367956189037152
aF-0.5543947345359598
aF-0.18972276965631985
aF0.43710466976452533
atp476
a(F0.77
(lp477
F-1.114456
aFnan
aFnan
a(lp478
g3
(g7
S'F\xd6[M\xd0\xd4\xf1\xbf'
p479
tp480
Rp481
aFnan
aFnan
a(lp482
F-1.1363291345925783
aF-0.5656263808727401
aF-0.19981885084294024
aF0.41502245968901896
atp483
a(F0.7799999999999998
(lp484
F-1.113388
aFnan
aFnan
a(lp485
g3
(g7
S'\x1dcb\xc0o\xd0\xf1\xbf'
p486
tp487
Rp488
aFnan
aFnan
a(lp489
F-1.135726696711882
aF-0.5764915635268901
aF-0.2095418643710301
aF0.3935378681965417
atp490
a(F0.79
(lp491
F-1.112183
aFnan
aFnan
a(lp492
g3
(g7
S's\xaeD\x92\x80\xcb\xf1\xbf'
p493
tp494
Rp495
aFnan
aFnan
a(lp496
F-1.1349968568157107
aF-0.5870042367304702
aF-0.21890583472295014
aF0.3726314977794709
atp497
a(F0.7999999999999998
(lp498
F-1.11085
aFnan
aFnan
a(lp499
g3
(g7
S':\x15\x04\x11\x0b\xc6\xf1\xbf'
p500
tp501
Rp502
aFnan
aFnan
a(lp503
F-1.1341476667574544
aF-0.5971778019824805
aF-0.22792423484935986
aF0.3522845697473158
atp504
a(F0.81
(lp505
F-1.109397
aFnan
aFnan
a(lp506
g3
(g7
S'\xbc\xbf?\x0b\x17\xc0\xf1\xbf'
p507
tp508
Rp509
aFnan
aFnan
a(lp510
F-1.1331867080463258
aF-0.6070251257887402
aF-0.23661000429692042
aF0.3324789173205963
atp511
a(F0.8199999999999998
(lp512
F-1.10783
aFnan
aFnan
a(lp513
g3
(g7
S'\x9fC\xb5\xd7\xab\xb9\xf1\xbf'
p514
tp515
Rp516
aFnan
aFnan
a(lp517
F-1.132121119729398
aF-0.6165585566588602
aF-0.24497556656033967
aF0.3131969787186981
atp518
a(F0.8300000000000001
(lp519
F-1.106156
aFnan
aFnan
a(lp520
g3
(g7
S'\x88]e\\\xd0\xb2\xf1\xbf'
p521
tp522
Rp523
aFnan
aFnan
a(lp524
F-1.130957624904268
aF-0.62578994151913
aF-0.25303284581739
aF0.29442179003554825
atp525
a(F0.8399999999999999
(lp526
F-1.104381
aFnan
aFnan
a(lp527
g3
(g7
S'\x80\xacb\x15\x8b\xab\xf1\xbf'
p528
tp529
Rp530
aFnan
aFnan
a(lp531
F-1.129702555948949
aF-0.6347306416723001
aF-0.2607932831774402
aF0.2761369777338596
atp532
a(F0.8500000000000001
(lp533
F-1.102511
aFnan
aFnan
a(lp534
g3
(g7
S'\xe1\xffN\x1b\xe2\xa3\xf1\xbf'
p535
tp536
Rp537
aFnan
aFnan
a(lp538
F-1.1283618785363037
aF-0.6433915484078603
aF-0.2682678525473805
aF0.2583267506235234
atp539
a(F0.8599999999999999
(lp540
F-1.100551
aFnan
aFnan
a(lp541
g3
(g7
S'\xa4\x0c\x8b)\xdb\x9b\xf1\xbf'
p542
tp543
Rp544
aFnan
aFnan
a(lp545
F-1.1269412144899034
aF-0.6517830983451
aF-0.27546707619741967
aF0.24097589122138394
atp546
a(F0.8700000000000001
(lp547
F-1.098507
aFnan
aFnan
a(lp548
g3
(g7
S't\x90\x1b\xa4{\x93\xf1\xbf'
p549
tp550
Rp551
aFnan
aFnan
a(lp552
F-1.125445863526723
aF-0.6599152885701699
aF-0.2824010400884894
aF0.22406974642037347
atp553
a(F0.8799999999999999
(lp554
F-1.096383
aFnan
aFnan
a(lp555
g3
(g7
S'h.F\x9d\xc8\x8a\xf1\xbf'
p556
tp557
Rp558
aFnan
aFnan
a(lp559
F-1.1238808239217275
aF-0.6677976916094303
aF-0.2890794090041499
aF0.20759421742225725
atp560
a(F0.8900000000000001
(lp561
F-1.094184
aFnan
aFnan
a(lp562
g3
(g7
S'\x08<\xe8\xda\xc6\x81\xf1\xbf'
p563
tp564
Rp565
aFnan
aFnan
a(lp566
F-1.122250812128265
aF-0.6754394702684502
aF-0.29551144151741027
aF0.1915357489132849
atp567
a(F0.8999999999999999
(lp568
F-1.091914
aFnan
aFnan
a(lp569
g3
(g7
S'\xf2\xee\x88\xdbzx\xf1\xbf'
p570
tp571
Rp572
aFnan
aFnan
a(lp573
F-1.1205602813772166
aF-0.6828493923494505
aF-0.3017060048060705
aF0.17588131748299718
atp574
a(F0.9100000000000001
(lp575
F-1.089578
aFnan
aFnan
a(lp576
g3
(g7
S'l\x9c(\xdb\xe8n\xf1\xbf'
p577
tp578
Rp579
aFnan
aFnan
a(lp580
F-1.1188134392814457
aF-0.6900358452519798
aF-0.3076715893228197
aF0.1606184193059562
atp581
a(F0.9199999999999999
(lp582
F-1.087178
aFnan
aFnan
a(lp583
g3
(g7
S'x7\xce\xd7\x14e\xf1\xbf'
p584
tp585
Rp586
aFnan
aFnan
a(lp587
F-1.1170142644648302
aF-0.69700685045014
aF-0.31341632331435976
aF0.1457350571216707
atp588
a(F0.9299999999999997
(lp589
F-1.084719
aFnan
aFnan
a(lp590
g3
(g7
S'\xf4\x81\xd4\x95\x02[\xf1\xbf'
p591
tp592
Rp593
aFnan
aFnan
a(lp594
F-1.1151665222390958
aF-0.7037700778341001
aF-0.31894798717892003
aF0.13121972656217656
atp595
a(F0.94
(lp596
F-1.082204
aFnan
aFnan
a(lp597
g3
(g7
S'BE\xf8\xa3\xb5P\xf1\xbf'
p598
tp599
Rp600
aFnan
aFnan
a(lp601
F-1.1132737793499572
aF-0.7103328598976604
aF-0.3242740276452402
aF0.11706140188680737
atp602
a(F0.9499999999999997
(lp603
F-1.079637
aFnan
aFnan
a(lp604
g3
(g7
S'\x92\xdb(_1F\xf1\xbf'
p605
tp606
Rp607
aFnan
aFnan
a(lp608
F-1.111339417813399
aF-0.7167022057483006
aF-0.32940157175100016
aF0.1032495211931699
atp609
a(F0.96
(lp610
F-1.07702
aFnan
aFnan
a(lp611
g3
(g7
S'\x18\x7f\x1c\xf6x;\xf1\xbf'
p612
tp613
Rp614
aFnan
aFnan
a(lp615
F-1.1093666478653872
aF-0.7228848149144201
aF-0.3343374405971401
aF0.08977397117930702
atp616
a(F0.9699999999999998
(lp617
F-1.074356
aFnan
aFnan
a(lp618
g3
(g7
S'9%\xaal\x8f0\xf1\xbf'
p619
tp620
Rp621
aFnan
aFnan
a(lp622
F-1.1073585200527747
aF-0.7288870909241001
aF-0.33908816285358
aF0.07662507153636516
atp623
a(F0.98
(lp624
F-1.071647
aFnan
aFnan
a(lp625
g3
(g7
S'&a\xea\x9ew%\xf1\xbf'
p626
tp627
Rp628
aFnan
aFnan
a(lp629
F-1.1053179364889183
aF-0.73471515462631
aF-0.3436599879893897
aF0.06379355905379935
atp630
a(F0.9899999999999998
(lp631
F-1.068898
aFnan
aFnan
a(lp632
g3
(g7
S'E\x1a!D4\x1a\xf1\xbf'
p633
tp634
Rp635
aFnan
aFnan
a(lp636
F-1.1032476613020685
aF-0.7403748572272799
aF-0.34805889920127975
aF0.051270571519679405
atp637
a(F1.0
(lp638
F-1.066109
aFnan
aFnan
a(lp639
g3
(g7
S'\xe9Kr\xf1\xc7\x0e\xf1\xbf'
p640
tp641
Rp642
aFnan
aFnan
a(lp643
F-1.1011503303102146
aF-0.7458717930174702
aF-0.3522906260177898
aF0.03904763149858509
atp644
a(F1.0099999999999998
(lp645
F-1.063283
aFnan
aFnan
a(lp646
g3
(g7
S'b\x88c\x1c5\x03\xf1\xbf'
p647
tp648
Rp649
aFnan
aFnan
a(lp650
F-1.099028459949329
aF-0.7512113117625501
aF-0.35636065655385013
aF0.027116630066849834
atp651
a(F1.02
(lp652
F-1.060423
aFnan
aFnan
a(lp653
g3
(g7
S'\x84\x88,\x1d~\xf7\xf0\xbf'
p654
tp655
Rp656
aFnan
aFnan
a(lp657
F-1.0968844554896124
aF-0.7563985307364601
aF-0.36027424939566
aF0.015469810582852718
atp658
a(F1.0299999999999998
(lp659
F-1.057531
aFnan
aFnan
a(lp660
g3
(g7
S'\xce\x17\xd90\xa5\xeb\xf0\xbf'
p661
tp662
Rp663
aFnan
aFnan
a(lp664
F-1.0947206185747993
aF-0.7614383463771601
aF-0.36403644509769995
aF0.00409975256549996
atp665
a(F1.04
(lp666
F-1.054608
aFnan
aFnan
a(lp667
g3
(g7
S'\xca\x9c>{\xac\xdf\xf0\xbf'
p668
tp669
Rp670
aFnan
aFnan
a(lp671
F-1.09253915411847
aF-0.7663354455472903
aF-0.3676520772757301
aF-0.007000644250479517
atp672
a(F1.0499999999999998
(lp673
F-1.051657
aFnan
aFnan
a(lp674
g3
(g7
S'\x98{\xc7\x08\x96\xd3\xf0\xbf'
p675
tp676
Rp677
aFnan
aFnan
a(lp678
F-1.0903421765911652
aF-0.7710943163840901
aF-0.37112578328153034
aF-0.017838175618524563
atp679
a(F1.06
(lp680
F-1.048679
aFnan
aFnan
a(lp681
g3
(g7
S'\xfc\x02\x17\xd0c\xc7\xf0\xbf'
p682
tp683
Rp684
aFnan
aFnan
a(lp685
F-1.0881317157383412
aF-0.7757192587294701
aF-0.3744620144514099
aF-0.028419348185958867
atp686
a(F1.0699999999999998
(lp687
F-1.045677
aFnan
aFnan
a(lp688
g3
(g7
S'\xb6\n\x88\xb3\x17\xbb\xf0\xbf'
p689
tp690
Rp691
aFnan
aFnan
a(lp692
F-1.0859097217614204
aF-0.7802143941294702
aF-0.37766504591935013
aF-0.03875039454926872
atp693
a(F1.08
(lp694
F-1.042652
aFnan
aFnan
a(lp695
g3
(g7
S'C\xcb\x88\x82\xb3\xae\xf0\xbf'
p696
tp697
Rp698
aFnan
aFnan
a(lp699
F-1.0836780699995439
aF-0.7845836753983404
aF-0.3807389859909403
aF-0.04883728791267587
atp700
a(F1.0899999999999999
(lp701
F-1.039605
aFnan
aFnan
a(lp702
g3
(g7
S'\x98[\xd6\xfa8\xa2\xf0\xbf'
p703
tp704
Rp705
aFnan
aFnan
a(lp706
F-1.0814385651480007
aF-0.78883089574512
aF-0.38368778507707985
aF-0.05868575631070852
atp707
a(F1.1
(lp708
F-1.036539
aFnan
aFnan
a(lp709
g3
(g7
S'\x1d4\x9a\xc9\xa9\x95\xf0\xbf'
p710
tp711
Rp712
aFnan
aFnan
a(lp713
F-1.0791929450483324
aF-0.7929596974619602
aF-0.3865152441881598
aF-0.06830129636041685
atp714
a(F1.1099999999999999
(lp715
F-1.033454
aFnan
aFnan
a(lp716
g3
(g7
S'\x04\xd5k\x8c\x07\x89\xf0\xbf'
p717
tp718
Rp719
aFnan
aFnan
a(lp720
F-1.0769428840816513
aF-0.7969735801761005
aF-0.3892250229911802
aF-0.0776891865155481
atp721
a(F1.12
(lp722
F-1.030353
aFnan
aFnan
a(lp723
g3
(g7
S'\xf089\xd2S|\xf0\xbf'
p724
tp725
Rp726
aFnan
aFnan
a(lp727
F-1.07468999620402
aF-0.8008759086727804
aF-0.39182064743817985
aF-0.08685449980043987
atp728
a(F1.13
(lp729
F-1.027237
aFnan
aFnan
a(lp730
g3
(g7
S'm\xc1\x17\x1c\x90o\xf0\xbf'
p731
tp732
Rp733
aFnan
aFnan
a(lp734
F-1.0724358376489498
aF-0.8046699202929202
aF-0.39430551697082
aF-0.09580211600685933
atp735
a(F1.1400000000000001
(lp736
F-1.024107
aFnan
aFnan
a(lp737
g3
(g7
S'\xf8\x1a\x00\xde\xbdb\xf0\xbf'
p738
tp739
Rp740
aFnan
aFnan
a(lp741
F-1.070181909333388
aF-0.8083587319171003
aF-0.39668291131309985
aF-0.10453673334216136
atp742
a(F1.15
(lp743
F-1.020964
aFnan
aFnan
a(lp744
g3
(g7
S'\x86\xd6v\x7f\xdeU\xf0\xbf'
p745
tp746
Rp747
aFnan
aFnan
a(lp748
F-1.0679296589929002
aF-0.8119453465450905
aF-0.3989559968624905
aF-0.11306287952209022
atp749
a(F1.1600000000000001
(lp750
F-1.017837
aF-1.017837
aF-1.01781
a(lp751
g3
(g7
S'\xb5\xb5l\xfa\x06\r\xf1\xbf'
p752
tp753
Rp754
ag3
(g7
S'\x0e^\x92;\x06\x18\xea\xbf'
p755
tp756
Rp757
ag3
(g7
S'\xca?r\x0f\x15\x13\xbf\xbf'
p758
tp759
Rp760
a(lp761
F-1.0656804830763589
aF-0.8154326594839904
aF-0.40112783269298985
aF-0.12138492230550094
atp762
a(F1.17
(lp763
F-1.014813
aF-1.014813
aF-1.014646
a(lp764
g3
(g7
S'\xad\xa3\xaf.\xd5\x03\xf1\xbf'
p765
tp766
Rp767
ag3
(g7
S'>\x19\xf8C\xcd3\xea\xbf'
p768
tp769
Rp770
ag3
(g7
S'\x01\x8av\x1f\xb0\x93\xc0\xbf'
p771
tp772
Rp773
a(lp774
F-1.0634357284237825
aF-0.8188234641573201
aF-0.4032013761829799
aF-0.1295070794728274
atp775
a(F1.1800000000000002
(lp776
F-1.011897
aF-1.011897
aF-1.011474
a(lp777
g3
(g7
S'.\xb2db\xa9\xfa\xf0\xbf'
p778
tp779
Rp780
ag3
(g7
S'~\x98\xd1\x8f\xcfN\xea\xbf'
p781
tp782
Rp783
ag3
(g7
S"\xad\xef\xdd'k\x97\xc1\xbf"
p784
tp785
Rp786
a(lp787
F-1.0611966937531627
aF-0.8221204575500103
aF-0.4051794882836502
aF-0.1374334282535563
atp788
a(F1.19
(lp789
F-1.009085
aF-1.009085
aF-1.008293
a(lp790
g3
(g7
S'v\xd7\x9a\xe5\x84\xf1\xf0\xbf'
p791
tp792
Rp793
ag3
(g7
S'\xb2\xaa\x03\x96\x12i\xea\xbf'
p794
tp795
Rp796
ag3
(g7
S'\xa7\xd8\xfb\xb9\xdc\x94\xc2\xbf'
p797
tp798
Rp799
a(lp800
F-1.0589646309794583
aF-0.8253262453048004
aF-0.40706493844339975
aF-0.14516791421115124
atp801
a(F1.1999999999999997
(lp802
F-1.006373
aF-1.006373
aF-1.005107
a(lp803
g3
(g7
S'h=!\xfch\xe8\xf0\xbf'
p804
tp805
Rp806
ag3
(g7
S'\x90\xbc\xf7\x9e\x9b\x82\xea\xbf'
p807
tp808
Rp809
ag3
(g7
S'\xd0}\x0c\xe6$\x8c\xc3\xbf'
p810
tp811
Rp812
a(lp813
F-1.0567407463857472
aF-0.8284433464849701
aF-0.40886040920410976
aF-0.15271435959649188
atp814
a(F1.21
(lp815
F-1.003756
aF-1.003756
aF-1.001915
a(lp816
g3
(g7
S'\xce\xf5\xce\xddV\xdf\xf0\xbf'
p817
tp818
Rp819
ag3
(g7
S'|\xe7\xfe\xc6o\x9b\xea\xbf'
p820
tp821
Rp822
ag3
(g7
S'\xac\xdfK\xc4b}\xc4\xbf'
p823
tp824
Rp825
a(lp826
F-1.0545262016670516
aF-0.8314741980204802
aF-0.4105685004863401
aF-0.16007647118396784
atp827
a(F1.2199999999999998
(lp828
F-1.001233
aF-1.001233
aF-0.998718
a(lp829
g3
(g7
S'G"\xc3\xb6O\xd6\xf0\xbf'
p830
tp831
Rp832
ag3
(g7
S'\xbc\xa1\x8b\x00\x94\xb3\xea\xbf'
p833
tp834
Rp835
ag3
(g7
S'\x96\xad\xbb\x84\xb4h\xc5\xbf'
p836
tp837
Rp838
a(lp839
F-1.0523221148633948
aF-0.8344211588528705
aF-0.41219173357911
aF-0.16725784760563508
atp840
a(F1.23
(lp841
F-0.9988
aF-0.9988
aF-0.995519
a(lp842
g3
(g7
S'\x1e\xb9\x9e\xa7T\xcd\xf0\xbf'
p843
tp844
Rp845
ag3
(g7
S'\x12}D\x16\r\xcb\xea\xbf'
p846
tp847
Rp848
ag3
(g7
S'\xd6\xdb\xd5}7N\xc6\xbf'
p849
tp850
Rp851
a(lp852
F-1.0501295612007722
aF-0.8372865137970701
aF-0.4137325548528298
aF-0.17426198620116648
atp853
a(F1.2399999999999998
(lp854
F-0.996453
aF-0.996453
aF-0.992317
a(lp855
g3
(g7
S'\x8b\xcb\xb8\xc5f\xc4\xf0\xbf'
p856
tp857
Rp858
ag3
(g7
S'2\x08\xf2\xac\xdf\xe1\xea\xbf'
p859
tp860
Rp861
ag3
(g7
S'\x10<E:\x08.\xc7\xbf'
p862
tp863
Rp864
a(lp865
F-1.0479495738515876
aF-0.8400724771347602
aF-0.4151933392098598
aF-0.18109228940242184
atp866
a(F1.25
(lp867
F-0.99419
aF-0.99419
aF-0.989114
a(lp868
g3
(g7
S'\xb5ZN\x1b\x87\xbb\xf0\xbf'
p869
tp870
Rp871
ag3
(g7
S'&3JE\x10\xf8\xea\xbf'
p872
tp873
Rp874
ag3
(g7
S'\xb5\xb3\xa5\x85B\x08\xc8\xbf'
p875
tp876
Rp877
a(lp878
F-1.0457831446307593
aF-0.84278119595692
aF-0.4165763932910201
aF-0.18775207067251037
atp879
a(F1.2599999999999998
(lp880
F-0.992008
aF-0.992008
aF-0.98591
a(lp881
g3
(g7
S'\xc3h\xae\xa7\xb6\xb2\xf0\xbf'
p882
tp883
Rp884
ag3
(g7
S'\x82L\x9b=\xa3\r\xeb\xbf'
p885
tp886
Rp887
ag3
(g7
S'P#[x\x01\xdd\xc8\xbf'
p888
tp889
Rp890
a(lp891
F-1.043631224637048
aF-0.8454147532705899
aF-0.41788395845250986
aF-0.1942445600199611
atp892
a(F1.27
(lp893
F-0.989903
aF-0.989903
aF-0.982707
a(lp894
g3
(g7
S'a+c_\xf6\xa9\xf0\xbf'
p895
tp896
Rp897
ag3
(g7
S'\x88\xe2X\xd3\x9c"\xeb\xbf'
p898
tp899
Rp900
ag3
(g7
S'XP\x8b\x82_\xac\xc9\xbf'
p901
tp902
Rp903
a(lp904
F-1.041494724852523
aF-0.84797517088653
aF-0.41911821353047
aF-0.2005729091094362
atp905
a(F1.2799999999999998
(lp906
F-0.987873
aF-0.987873
aF-0.979506
a(lp907
g3
(g7
S'\x8b\xdbX,G\xa1\xf0\xbf'
p908
tp909
Rp910
ag3
(g7
S'\xfao\x8c$\x017\xeb\xbf'
p911
tp912
Rp913
ag3
(g7
S'\x0e\xf4Evvv\xca\xbf'
p914
tp915
Rp916
a(lp917
F-1.0393745167072828
aF-0.8504644121017003
aF-0.42028127740706
aF-0.20674019599016638
atp918
a(F1.29
(lp919
F-0.985915
aF-0.985915
aF-0.976307
a(lp920
g3
(g7
S'\x85\xcb\x02\xee\xa9\x98\xf0\xbf'
p921
tp922
Rp923
ag3
(g7
S'\x82\xf7+1\xd4J\xeb\xbf'
p924
tp925
Rp926
ag3
(g7
S'\xfd\x05\xe5\x90_;\xcb\xbf'
p927
tp928
Rp929
a(lp930
F-1.0372714326192354
aF-0.85288438419205
aF-0.4213752113933499
aF-0.21274942946369382
atp931
a(F1.2999999999999998
(lp932
F-0.984028
aF-0.984028
aF-0.973111
a(lp933
g3
(g7
S'\xb78\x7fy\x1f\x90\xf0\xbf'
p934
tp935
Rp936
ag3
(g7
S' hX\xdc\x19^\xeb\xbf'
p937
tp938
Rp939
ag3
(g7
S'\xff\x00\xb4\x833\xfb\xcb\xbf'
p940
tp941
Rp942
a(lp943
F-1.0351862665152507
aF-0.85523694072913
aF-0.4224020214425698
aF-0.21860355311219837
atp944
a(F1.31
(lp945
F-0.982207
aF-0.982207
aF-0.969918
a(lp946
g3
(g7
S'\x87G\xba\x99\xa8\x87\xf0\xbf'
p947
tp948
Rp949
ag3
(g7
S'<\xa9\x85\xed\xd5p\xeb\xbf'
p950
tp951
Rp952
ag3
(g7
S'\xc7;\xe7{\n\xb6\xcc\xbf'
p953
tp954
Rp955
a(lp956
F-1.0331197743402925
aF-0.8575238837341098
aF-0.4233636602074698
aF-0.22430544900857668
atp957
a(F1.3199999999999998
(lp958
F-0.980452
aF-0.980452
aF-0.966731
a(lp959
g3
(g7
S'6\x86\x90\x0fF\x7f\xf0\xbf'
p960
tp961
Rp962
ag3
(g7
S'\xcb\t\x8e\x11\x0c\x83\xeb\xbf'
p963
tp964
Rp965
ag3
(g7
S'\x97\xc4\xef)\xfck\xcd\xbf'
p966
tp967
Rp968
a(lp969
F-1.0310726745596064
aF-0.8597469656818302
aF-0.42426202895404963
aF-0.2298579411285725
atp970
a(F1.33
(lp971
F-0.97876
aF-0.97876
aF-0.963549
a(lp972
g3
(g7
S'\x92F\xf1\x91\xf8v\xf0\xbf'
p973
tp974
Rp975
ag3
(g7
S'\xf0\xb9\xb2\xdb\xbf\x94\xeb\xbf'
p976
tp977
Rp978
ag3
(g7
S'\xda\x896\xc8\x1f\x1d\xce\xbf'
p979
tp980
Rp981
a(lp982
F-1.0290456486585855
aF-0.86190789136691
aF-0.42509897934366975
aF-0.2352637984850837
atp983
a(F1.3399999999999999
(lp984
F-0.977127
aF-0.977127
aF-0.960372
a(lp985
g3
(g7
S'\xee\x0e\x01\xce\xc0n\xf0\xbf'
p986
tp987
Rp988
ag3
(g7
S'\xff\xdf\x8a\xc6\xf4\xa5\xeb\xbf'
p989
tp990
Rp991
ag3
(g7
S'\xbdXI!\x8c\xc9\xce\xbf'
p992
tp993
Rp994
a(lp995
F-1.0270393416439516
aF-0.8640083196432902
aF-0.4258763150949099
aF-0.24052573800389834
atp996
a(F1.35
(lp997
F-0.975554
aF-0.975554
aF-0.957203
a(lp998
g3
(g7
S'{Z<g\x9ff\xf0\xbf'
p999
tp1000
Rp1001
ag3
(g7
S'\x13\xba\xe24\xae\xb6\xeb\xbf'
p1002
tp1003
Rp1004
ag3
(g7
S'\x90\xc3\x83\x95Wq\xcf\xbf'
p1005
tp1006
Rp1007
a(lp1008
F-1.0250543625494672
aF-0.8660498650477304
aF-0.42659579353538984
aF-0.24564642715951224
atp1009
a(F1.3599999999999999
(lp1010
F-0.974036
aF-0.974036
aF-0.954041
a(lp1011
g3
(g7
S'x\xd4\x9a\xf7\x94^\xf0\xbf'
p1012
tp1013
Rp1014
ag3
(g7
S'O-\x8cr\xef\xc6\xeb\xbf'
p1015
tp1016
Rp1017
ag3
(g7
S'B\xfd\x1e\x10L\n\xd0\xbf'
p1018
tp1019
Rp1020
a(lp1021
F-1.0230912849486027
aF-0.8680340993172797
aF-0.42725912705365937
aF-0.2506284863883964
atp1022
a(F1.37
(lp1023
F-0.972573
aF-0.972573
aF-0.950888
a(lp1024
g3
(g7
S'P5\xb3\x0f\xa2V\xf0\xbf'
p1025
tp1026
Rp1027
ag3
(g7
S'`\x0c"\xb5\xbb\xd6\xeb\xbf'
p1028
tp1029
Rp1030
ag3
(g7
S'\xc3HE\xae\xb1Y\xd0\xbf'
p1031
tp1032
Rp1033
a(lp1034
F-1.0211506474764347
aF-0.8699625528100904
aF-0.4278679844599499
aF-0.2554744912969346
atp1035
a(F1.38
(lp1036
F-0.971163
aF-0.971163
aF-0.947742
a(lp1037
g3
(g7
S'\x07\xd5\xdf6\xc7N\xf0\xbf'
p1038
tp1039
Rp1040
ag3
(g7
S'\xf63\xbf\x1c\x16\xe6\xeb\xbf'
p1041
tp1042
Rp1043
ag3
(g7
S'7\x0b\xc6D\xe7\xa6\xd0\xbf'
p1044
tp1045
Rp1046
a(lp1047
F-1.0192329543618281
aF-0.8718367158377301
aF-0.42842399226440964
aF-0.26018697467971086
atp1048
a(F1.3900000000000001
(lp1049
F-0.969803
aF-0.969803
aF-0.944607
a(lp1050
g3
(g7
S'\xad\x13d\xeb\x04G\xf0\xbf'
p1051
tp1052
Rp1053
ag3
(g7
S'\xcc\xac\xaa\xb4\x01\xf5\xeb\xbf'
p1054
tp1055
Rp1056
ag3
(g7
S'\x95c5G\xf7\xf1\xd0\xbf'
p1057
tp1058
Rp1059
a(lp1060
F-1.017338675971795
aF-0.8736580399176099
aF-0.42892873588057
aF-0.264768428363415
atp1061
a(F1.4
(lp1062
F-0.968491
aF-0.968491
aF-0.941481
a(lp1063
g3
(g7
S'\xd3\x99\x92\xa2[?\xf0\xbf'
p1064
tp1065
Rp1066
ag3
(g7
S'\xbb\xba\xf9s\x81\x03\xec\xbf'
p1067
tp1068
Rp1069
ag3
(g7
S'\xbe\xeb\xf8\xfe\xeb:\xd1\xbf'
p1070
tp1071
Rp1072
a(lp1073
F-1.0154682493681433
aF-0.8754279389521205
aF-0.4293837607609798
aF-0.2692213048900856
atp1074
a(F1.4100000000000001
(lp1075
F-0.967227
aF-0.967227
aF-0.938365
a(lp1076
g3
(g7
S'\x04\x87\xf4\xc8\xcb7\xf0\xbf'
p1077
tp1078
Rp1079
ag3
(g7
S'!\xdd(>\x98\x11\xec\xbf'
p1080
tp1081
Rp1082
ag3
(g7
S'\x1d\x0b\xee\x8c\xcf\x81\xd1\xbf'
p1083
tp1084
Rp1085
a(lp1086
F-1.0136220788776322
aF-0.8771477903418703
aF-0.4297905734718698
aF-0.27354801905329684
atp1087
a(F1.42
(lp1088
F-0.966008
aF-0.966008
aF-0.93526
a(lp1089
g3
(g7
S'f\x88q\xc2U0\xf0\xbf'
p1090
tp1091
Rp1092
ag3
(g7
S'\x9d\x80\xac\xe3H\x1f\xec\xbf'
p1093
tp1094
Rp1095
ag3
(g7
S'\xfd\x18\xeb\xea\xab\xc6\xd1\xbf'
p1096
tp1097
Rp1098
a(lp1099
F-1.0118005366753318
aF-0.8788189360384603
aF-0.43015064271244
aF-0.27775094929928773
atp1100
a(F1.4300000000000002
(lp1101
F-0.964833
aF-0.964833
aF-0.932167
a(lp1102
g3
(g7
S'F\xe3x\xea\xf9(\xf0\xbf'
p1103
tp1104
Rp1105
ag3
(g7
S'\xd3Cz"\x96,\xec\xbf'
p1106
tp1107
Rp1108
ag3
(g7
S'\xcd\x89\x1e\xed\x8a\t\xd2\xbf'
p1109
tp1110
Rp1111
a(lp1112
F-1.0100039633818627
aF-0.8804426835432602
aF-0.4304654002844997
aF-0.281832439004706
atp1113
a(F1.44
(lp1114
F-0.9637
aF-0.9637
aF-0.929086
a(lp1115
g3
(g7
S'\x11h+\x94\xb8!\xf0\xbf'
p1116
tp1117
Rp1118
ag3
(g7
S'#a\x8b\xa6\x829\xec\xbf'
p1119
tp1120
Rp1121
ag3
(g7
S'8\x12OCvJ\xd2\xbf'
p1122
tp1123
Rp1124
a(lp1125
F-1.0082326686738303
aF-0.88202030685628
aF-0.43073624201707966
aF-0.28579479764109883
atp1126
a(F1.4499999999999997
(lp1127
F-0.962607
aF-0.962607
aF-0.926017
a(lp1128
g3
(g7
S'\x82S\x86\n\x92\x1a\xf0\xbf'
p1129
tp1130
Rp1131
ag3
(g7
S'\x81\x03Y\n\x11F\xec\xbf'
p1132
tp1133
Rp1134
ag3
(g7
S'\xedk\xffyw\x89\xd2\xbf'
p1135
tp1136
Rp1137
a(lp1138
F-1.0064869319078005
aF-0.8835530473808004
aF-0.4309645286507198
aF-0.2896403018364087
atp1139
a(F1.46
(lp1140
F-0.961554
aF-0.961554
aF-0.922961
a(lp1141
g3
(g7
S'\x87\x10\x8f\x90\x86\x13\xf0\xbf'
p1142
tp1143
Rp1144
ag3
(g7
S'\x9b\xf8R\xd7CR\xec\xbf'
p1145
tp1146
Rp1147
ag3
(g7
S'\xa3(x\xfb\x97\xc6\xd2\xbf'
p1148
tp1149
Rp1150
a(lp1151
F-1.0047670027570634
aF-0.8850421147870001
aF-0.43115158668507997
aF-0.2933711963420357
atp1152
a(F1.4699999999999998
(lp1153
F-0.960539
aF-0.960539
aF-0.919918
a(lp1154
g3
(g7
S'c\xd7\x7fa\x96\x0c\xf0\xbf'
p1155
tp1156
Rp1157
ag3
(g7
S'\x91]Q\x86\x1d^\xec\xbf'
p1158
tp1159
Rp1160
ag3
(g7
S',\xdd\xb9\x10\xe1\x01\xd3\xbf'
p1161
tp1162
Rp1163
a(lp1164
F-1.0030731018609569
aF-0.8864886878390504
aF-0.4312987091938498
aF-0.2969896949138822
atp1165
a(F1.48
(lp1166
F-0.95956
aF-0.95956
aF-0.916889
a(lp1167
g3
(g7
S'\xe0\x1c\xf5\xb0\xc1\x05\xf0\xbf'
p1168
tp1169
Rp1170
ag3
(g7
S'P\xaf\x01\x80\xa0i\xec\xbf'
p1171
tp1172
Rp1173
ag3
(g7
S'\xea\xbfY\xe2[;\xd3\xbf'
p1174
tp1175
Rp1176
a(lp1177
F-1.001405421486019
aF-0.8878939151886504
aF-0.43140715660969015
aF-0.3004979811148605
atp1178
a(F1.4899999999999998
(lp1179
F-0.958617
aF-0.958617
aF-0.913874
a(lp1180
g3
(g7
S'6\x977V\x11\xfe\xef\xbf'
p1181
tp1182
Rp1183
ag3
(g7
S'\xfb\xa8O\x1d\xcft\xec\xbf'
p1184
tp1185
Rp1186
ag3
(g7
S'\xe8\x7fJy\x11s\xd3\xbf'
p1187
tp1188
Rp1189
a(lp1190
F-0.9997641261986474
aF-0.8892589161380601
aF-0.43147815748234025
aF-0.30389820904565223
atp1191
a(F1.5
(lp1192
F-0.957707
aF-0.957707
aF-0.910874
a(lp1193
g3
(g7
S'ip\xc0\xe9\xd6\xf0\xef\xbf'
p1194
tp1195
Rp1196
ag3
(g7
S'\xd1X\xca\xa7\xab\x7f\xec\xbf'
p1197
tp1198
Rp1199
ag3
(g7
S'\xd03\x93\xbf\n\xa9\xd3\xbf'
p1200
tp1201
Rp1202
a(lp1203
F-0.9981493535483528
aF-0.8905847813755606
aF-0.43151290921230034
aF-0.3071925040101669
atp1204
a(F1.5099999999999998
(lp1205
F-0.95683
aF-0.95683
aF-0.907888
a(lp1206
g3
(g7
S'x\x8b;X\xd4\xe3\xef\xbf'
p1207
tp1208
Rp1209
ag3
(g7
S'\xc0\xb4\x05Z8\x8a\xec\xbf'
p1210
tp1211
Rp1212
ag3
(g7
S'\xc5\xd8\xf5\x80P\xdd\xd3\xbf'
p1213
tp1214
Rp1215
a(lp1216
F-0.9965612147610567
aF-0.8918725736854402
aF-0.43151257876230004
aF-0.3103829631212428
atp1217
a(F1.52
(lp1218
F-0.955984
aF-0.955984
aF-0.904917
a(lp1219
g3
(g7
S'\xd4Y\x9e\xcf\t\xd7\xef\xbf'
p1220
tp1221
Rp1222
ag3
(g7
S'3\xfd\xf8_w\x94\xec\xbf'
p1223
tp1224
Rp1225
ag3
(g7
S'\x18\xcd\x86k\xeb\x0f\xd4\xbf'
p1226
tp1227
Rp1228
a(lp1229
F-0.9949997954416243
aF-0.8931233286347503
aF-0.43147830334838994
aF-0.31347165585175524
atp1230
a(F1.5299999999999998
(lp1231
F-0.955169
aF-0.955169
aF-0.901962
a(lp1232
g3
(g7
S'\x82\xb9~pw\xca\xef\xbf'
p1233
tp1234
Rp1235
ag3
(g7
S';8Z\xd7j\x9e\xec\xbf'
p1236
tp1237
Rp1238
ag3
(g7
S'\x8b\xab6\x10\xe4@\xd4\xbf'
p1239
tp1240
Rp1241
a(lp1242
F-0.9934651562851246
aF-0.8943380552389103
aF-0.4314111911126698
aF-0.31646062453608487
atp1243
a(F1.54
(lp1244
F-0.954383
aF-0.954383
aF-0.899022
a(lp1245
g3
(g7
S'\xd8\xb9uN\x1d\xbe\xef\xbf'
p1246
tp1247
Rp1248
ag3
(g7
S'\xd2\xe9\xf6\xcf\x14\xa8\xec\xbf'
p1249
tp1250
Rp1251
ag3
(g7
S'#\x89O\xe3Bp\xd4\xbf'
p1252
tp1253
Rp1254
a(lp1255
F-0.9919573337954778
aF-0.8955177366072403
aF-0.43131232177854023
aF-0.3193518848257919
atp1256
a(F1.5499999999999998
(lp1257
F-0.953626
aF-0.953626
aF-0.896099
a(lp1258
g3
(g7
S'\xeeb\x83p\xfb\xb1\xef\xbf'
p1259
tp1260
Rp1261
ag3
(g7
S'\xc1X\nLw\xb1\xec\xbf'
p1262
tp1263
Rp1264
ag3
(g7
S'6\xd4\xe6<\x10\x9e\xd4\xbf'
p1265
tp1266
Rp1267
a(lp1268
F-0.9904763410114276
aF-0.8966633305706401
aF-0.4311827472905397
aF-0.3221474261038717
atp1269
a(F1.56
(lp1270
F-0.952896
aF-0.952896
aF-0.893192
a(lp1271
g3
(g7
S'NKs\xd1\x11\xa6\xef\xbf'
p1272
tp1273
Rp1274
ag3
(g7
S'\xf4u\x91@\x94\xba\xec\xbf'
p1275
tp1276
Rp1277
ag3
(g7
S'\r\xb3DYT\xca\xd4\xbf'
p1278
tp1279
Rp1280
a(lp1281
F-0.9890221682384007
aF-0.8977757702920702
aF-0.4310234924391896
aF-0.3248492118607781
atp1282
a(F1.5699999999999998
(lp1283
F-0.952192
aF-0.952192
aF-0.890302
a(lp1284
g3
(g7
S',\xefA``\x9a\xef\xbf'
p1285
tp1286
Rp1287
ag3
(g7
S'8\x96\x9c\x95m\xc3\xec\xbf'
p1288
tp1289
Rp1290
ag3
(g7
S'\xb0\xbeAY\x17\xf5\xd4\xbf'
p1291
tp1292
Rp1293
a(lp1294
F-0.9875947837858563
aF-0.8988559648611903
aF-0.43083555547208996
aF-0.32745918003546337
atp1295
a(F1.58
(lp1296
F-0.951513
aF-0.951513
aF-0.887428
a(lp1297
g3
(g7
S'\xbb\x9d\x82\x00\xe7\x8e\xef\xbf'
p1298
tp1299
Rp1300
ag3
(g7
S'\x01"\x9f&\x05\xcc\xec\xbf'
p1301
tp1302
Rp1303
ag3
(g7
S'u\x08\x9cBa\x1e\xd5\xbf'
p1304
tp1305
Rp1306
a(lp1307
F-0.986194134708902
aF-0.8999047998741502
aF-0.43061990869224975
aF-0.32997924332460715
atp1308
a(F1.5899999999999999
(lp1309
F-0.950859
aF-0.950859
aF-0.884572
a(lp1310
g3
(g7
S'g\xe9\xc5\x8a\xa5\x83\xef\xbf'
p1311
tp1312
Rp1313
ag3
(g7
S'IQ\xbd\xc2\\\xd4\xec\xbf'
p1314
tp1315
Rp1316
ag3
(g7
S'*\xf6C\x00:F\xd5\xbf'
p1317
tp1318
Rp1319
a(lp1320
F-0.9848201475536312
aF-0.9009231379991806
aF-0.4303774990438401
aF-0.3324112894623287
atp1321
a(F1.6
(lp1322
F-0.950228
aF-0.950228
aF-0.881732
a(lp1323
g3
(g7
S'\x1e~\x00\xcd\x9bx\xef\xbf'
p1324
tp1325
Rp1326
ag3
(g7
S'h\x1c\x18-v\xdc\xec\xbf'
p1327
tp1328
Rp1329
ag3
(g7
S'\xc4\xd8\xa1b\xa9l\xd5\xbf'
p1330
tp1331
Rp1332
a(lp1333
F-0.9834727291053615
aF-0.9019118195291302
aF-0.43010924868658973
aF-0.33475718147327777
atp1334
a(F1.6099999999999999
(lp1335
F-0.94962
aF-0.94962
aF-0.878911
a(lp1336
g3
(g7
S'X,\xf2\x8a\xc9m\xef\xbf'
p1337
tp1338
Rp1339
ag3
(g7
S'\xcf_\x17\x1dS\xe4\xec\xbf'
p1340
tp1341
Rp1342
ag3
(g7
S'_\xa6\xd4\x1f\xb7\x91\xd5\xbf'
p1343
tp1344
Rp1345
a(lp1346
F-0.9821517671383714
aF-0.9028716629209099
aF-0.4298160555587098
aF-0.3370187579008381
atp1347
a(F1.62
(lp1348
F-0.949034
aF-0.949034
aF-0.876107
a(lp1349
g3
(g7
S'\xa7#\x8d~.c\xef\xbf'
p1350
tp1351
Rp1352
ag3
(g7
S']_\xb2>\xf5\xeb\xec\xbf'
p1353
tp1354
Rp1355
ag3
(g7
S'M\x96\xea\xd3j\xb5\xd5\xbf'
p1356
tp1357
Rp1358
a(lp1359
F-0.9808571311669891
aF-0.9038034653230902
aF-0.42949879392924967
aF-0.33919783301312006
atp1360
a(F1.63
(lp1361
F-0.948468
aF-0.948468
aF-0.873321
a(lp1362
g3
(g7
S'\x06+]X\xcaX\xef\xbf'
p1363
tp1364
Rp1365
ag3
(g7
S'}\xa9\xb62^\xf3\xec\xbf'
p1366
tp1367
Rp1368
ag3
(g7
S'\xb2\r\x14\x01\xcc\xd7\xd5\xbf'
p1369
tp1370
Rp1371
a(lp1372
F-0.9795886731966165
aF-0.9047080030916702
aF-0.42915831493992995
aF-0.341296196988163
atp1373
a(F1.6400000000000001
(lp1374
F-0.947924
aF-0.947924
aF-0.870554
a(lp1375
g3
(g7
S'\x14\xbb\xee\xbf\x9cN\xef\xbf'
p1376
tp1377
Rp1378
ag3
(g7
S'rk\r\x8f\x8f\xfa\xec\xbf'
p1379
tp1380
Rp1381
ag3
(g7
S'\xa8_\xd1\x0f\xe2\xf8\xd5\xbf'
p1382
tp1383
Rp1384
a(lp1385
F-0.9783462284738986
aF-0.9055860322945204
aF-0.4287954471367601
aF-0.3433156160804112
atp1386
a(F1.65
(lp1387
F-0.947398
aF-0.947398
aF-0.867804
a(lp1388
g3
(g7
S'\xa3\xdf5T\xa5D\xef\xbf'
p1389
tp1390
Rp1391
ag3
(g7
S'\x8dF\xff\xde\x8a\x01\xed\xbf'
p1392
tp1393
Rp1394
ag3
(g7
S'\x9d\xdf\x1bO\xb4\x18\xd6\xbf'
p1395
tp1396
Rp1397
a(lp1398
F-0.9771296162352775
aF-0.9064382892049302
aF-0.4284109969919096
aF-0.3452578327701215
atp1399
a(F1.6600000000000001
(lp1400
F-0.946892
aF-0.946892
aF-0.865074
a(lp1401
g3
(g7
S'\xb8\xbf\xf4\xab\xe3:\xef\xbf'
p1402
tp1403
Rp1404
ag3
(g7
S'>\xb4v\xa3Q\x08\xed\xbf'
p1405
tp1406
Rp1407
ag3
(g7
S'\xaa\xb2\x8a\xf4I7\xd6\xbf'
p1408
tp1409
Rp1410
a(lp1411
F-0.975938640453015
aF-0.9072654907846603
aF-0.42800574941573993
aF-0.34712456589731444
atp1412
a(F1.67
(lp1413
F-0.946404
aF-0.946404
aF-0.862361
a(lp1414
g3
(g7
S'I\xa0!VW1\xef\xbf'
p1415
tp1416
Rp1417
ag3
(g7
S'\x1d\xf1@S\xe5\x0e\xed\xbf'
p1418
tp1419
Rp1420
ag3
(g7
S'$\xbds\x1c\xaaT\xd6\xbf'
p1421
tp1422
Rp1423
a(lp1424
F-0.9747730905774087
aF-0.9080683351562904
aF-0.42758046825927015
aF-0.34891751078153116
atp1425
a(F1.6800000000000002
(lp1426
F-0.945933
aF-0.945933
aF-0.859668
a(lp1427
g3
(g7
S":TL\xda\xff'\xef\xbf"
p1428
tp1429
Rp1430
ag3
(g7
S'\x8d\x8fM[G\x15\xed\xbf'
p1431
tp1432
Rp1433
ag3
(g7
S'\xde"\t\xca\xdbp\xd6\xbf'
p1434
tp1435
Rp1436
a(lp1437
F-0.9736327422748509
aF-0.9088475020657705
aF-0.4271358968073301
aF-0.350638339329219
atp1438
a(F1.69
(lp1439
F-0.94548
aF-0.94548
aF-0.856993
a(lp1440
g3
(g7
S'\x92\xeb\x02\xb9\xdc\x1e\xef\xbf'
p1441
tp1442
Rp1443
ag3
(g7
S'\xa9\xa6\xec\x1ey\x1b\xed\xbf'
p1444
tp1445
Rp1446
ag3
(g7
S'~\xb8s\xe7\xe5\x8b\xd6\xbf'
p1447
tp1448
Rp1449
a(lp1450
F-0.9725173581604045
aF-0.9096036533348605
aF-0.4266727582623601
aF-0.3522887001298654
atp1451
a(F1.6999999999999997
(lp1452
F-0.945042
aF-0.945042
aF-0.854338
a(lp1453
g3
(g7
S'\x0c\x8a5l\xed\x15\xef\xbf'
p1454
tp1455
Rp1456
ag3
(g7
S'\xff\xab\x0b\xf8{!\xed\xbf'
p1457
tp1458
Rp1459
ag3
(g7
S'\xb3\xa7\xeaE\xcf\xa5\xd6\xbf'
p1460
tp1461
Rp1462
a(lp1463
F-0.9714266885242191
aF-0.9103374333038803
aF-0.42619175621891986
aF-0.35387021854204975
atp1464
a(F1.71
(lp1465
F-0.944621
aF-0.944621
aF-0.851701
a(lp1466
g3
(g7
S'\xde=\x99g1\r\xef\xbf'
p1467
tp1468
Rp1469
ag3
(g7
S"\t\xfbp7Q'\xed\xbf"
p1470
tp1471
Rp1472
ag3
(g7
S'J\xbf\xc8\x9d\x9e\xbe\xd6\xbf'
p1473
tp1474
Rp1475
a(lp1476
F-0.9703604720506817
aF-0.9110494692648403
aF-0.42569357512919975
aF-0.3553844967709579
atp1477
a(F1.7199999999999998
(lp1478
F-0.944214
aF-0.944214
aF-0.849084
a(lp1479
g3
(g7
S'\xe6\xc0\t\x19\xa8\x04\xef\xbf'
p1480
tp1481
Rp1482
ag3
(g7
S'\xed\x12\xf6$\xfa,\xed\xbf'
p1483
tp1484
Rp1485
ag3
(g7
S'\xb6\xb2\x9f\x8eZ\xd6\xd6\xbf'
p1486
tp1487
Rp1488
a(lp1489
F-0.9693184365296728
aF-0.9117403718852005
aF-0.4251788807594
aF-0.3568331139384071
atp1490
a(F1.73
(lp1491
F-0.943822
aF-0.943822
aF-0.846486
a(lp1492
g3
(g7
S'\x8d\xfe\xe9\xe8P\xfc\xee\xbf'
p1493
tp1494
Rp1495
ag3
(g7
S'7\x8b\xc0\xffw2\xed\xbf'
p1496
tp1497
Rp1498
ag3
(g7
S'.\x96I\x9f\t\xed\xd6\xbf'
p1499
tp1500
Rp1501
a(lp1502
F-0.9683002995588635
aF-0.9124107356222804
aF-0.42464832063716007
aF-0.35821762614645647
atp1503
a(F1.7399999999999998
(lp1504
F-0.943444
aF-0.943444
aF-0.843908
a(lp1505
g3
(g7
S'\xecE\x83:+\xf4\xee\xbf'
p1506
tp1507
Rp1508
ag3
(g7
S'\xca\xc8y\xfe\xcb7\xed\xbf'
p1509
tp1510
Rp1511
ag3
(g7
S'\x85\xed\xf8=\xb2\x02\xd7\xbf'
p1512
tp1513
Rp1514
a(lp1515
F-0.9673057692363588
aF-0.9130611391285806
aF-0.42410252449
aF-0.3595395665358504
atp1516
a(F1.75
(lp1517
F-0.94308
aF-0.94308
aF-0.841349
a(lp1518
g3
(g7
S'\xff\x02cl6\xec\xee\xbf'
p1519
tp1520
Rp1521
ag3
(g7
S'\xefs\x85O\xf7<\xed\xbf'
p1522
tp1523
Rp1524
ag3
(g7
S'`\x9bG\xc0Z\x17\xd7\xbf'
p1525
tp1526
Rp1527
a(lp1528
F-0.9663345448426235
aF-0.9136921456480401
aF-0.42354210467510006
aF-0.3608004453403062
atp1529
a(F1.7599999999999998
(lp1530
F-0.942729
aF-0.942729
aF-0.838809
a(lp1531
g3
(g7
S'\xf2\xef\xb6\xd8q\xe4\xee\xbf'
p1532
tp1533
Rp1534
ag3
(g7
S'\xf9\xb66\x19\xfbA\xed\xbf'
p1535
tp1536
Rp1537
ag3
(g7
S'R\xecDc\t+\xd7\xbf'
p1538
tp1539
Rp1540
a(lp1541
F-0.9653863175112727
aF-0.9143043034034402
aF-0.4229676566
aF-0.36200174993763606
atp1542
a(F1.77
(lp1543
F-0.94239
aF-0.94239
aF-0.836289
a(lp1544
g3
(g7
S'$\x94\xa7\xd5\xdc\xdc\xee\xbf'
p1545
tp1546
Rp1547
ag3
(g7
S'.E\x04z\xd8F\xed\xbf'
p1548
tp1549
Rp1550
ag3
(g7
S'v\x0f\x83K\xc4=\xd7\xbf'
p1551
tp1552
Rp1553
a(lp1554
F-0.9644607708875164
aF-0.9148981459749503
aF-0.4223797591348501
aF-0.3631449448987427
atp1555
a(F1.7799999999999998
(lp1556
F-0.942063
aF-0.942063
aF-0.833789
a(lp1557
g3
(g7
S'\x05\x02\xb1\xb5v\xd5\xee\xbf'
p1558
tp1559
Rp1560
ag3
(g7
S'\x954\xbb\x88\x90K\xed\xbf'
p1561
tp1562
Rp1563
ag3
(g7
S'\xa29$\x85\x91O\xd7\xbf'
p1564
tp1565
Rp1566
a(lp1567
F-0.9635575817738414
aF-0.9154741926701204
aF-0.4217789750158001
aF-0.36423147203540807
atp1568
a(F1.79
(lp1569
F-0.941749
aF-0.941749
aF-0.831309
a(lp1570
g3
(g7
S'\xde\xb4\xf9\xc7>\xce\xee\xbf'
p1571
tp1572
Rp1573
ag3
(g7
S'b\xa9\xb0T$P\xed\xbf'
p1574
tp1575
Rp1576
ag3
(g7
S'9\xb2\xe7\x03w`\xd7\xbf'
p1577
tp1578
Rp1579
a(lp1580
F-0.9626764207620466
aF-0.9160329488852701
aF-0.4211658512400096
aF-0.3652627504477825
atp1581
a(F1.7999999999999998
(lp1582
F-0.941445
aF-0.941445
aF-0.828848
a(lp1583
g3
(g7
S'\xa5|\xa7X4\xc7\xee\xbf'
p1584
tp1585
Rp1586
ag3
(g7
S'\xb5\\\xf2\xe5\x94T\xed\xbf'
p1587
tp1588
Rp1589
ag3
(g7
S'w\x0e7\xa3zp\xd7\xbf'
p1590
tp1591
Rp1592
a(lp1593
F-0.961816952851127
aF-0.9165749064585703
aF-0.42054091945196975
aF-0.3662401765725223
atp1594
a(F1.81
(lp1595
F-0.941153
aF-0.941153
aF-0.826407
a(lp1596
g3
(g7
S'rX2\xb1V\xc0\xee\xbf'
p1597
tp1598
Rp1599
ag3
(g7
S'q\xfbu=\xe3X\xed\xbf'
p1600
tp1601
Rp1602
ag3
(g7
S'\t\xc83&\xa2\x7f\xd7\xbf'
p1603
tp1604
Rp1605
a(lp1606
F-0.9609788380501081
aF-0.9171005440147001
aF-0.41990469632153976
aF-0.3671651242322013
atp1607
a(F1.8199999999999998
(lp1608
F-0.94087
aF-0.94087
aF-0.823986
a(lp1609
g3
(g7
S'\x8b4\xb5\x18\xa5\xb9\xee\xbf'
p1610
tp1611
Rp1612
ag3
(g7
S'\xd7iGU\x10]\xed\xbf'
p1613
tp1614
Rp1615
ag3
(g7
S'dp\xc57\xf3\x8d\xd7\xbf'
p1616
tp1617
Rp1618
a(lp1619
F-0.960161731965528
aF-0.9176103273014702
aF-0.4192576839136097
aF-0.3680389446869914
atp1620
a(F1.83
(lp1621
F-0.940598
aF-0.940598
aF-0.821585
a(lp1622
g3
(g7
S'`v<\xd4\x1e\xb3\xee\xbf'
p1623
tp1624
Rp1625
ag3
(g7
S'\xd2\xed\xb5 \x1da\xed\xbf'
p1626
tp1627
Rp1628
ag3
(g7
S'\xe8\xaf\xa8js\x9b\xd7\xbf'
p1629
tp1630
Rp1631
a(lp1632
F-0.9593652863729387
aF-0.9181047095184401
aF-0.41860037004953976
aF-0.36886296668922025
atp1633
a(F1.8399999999999999
(lp1634
F-0.940336
aF-0.940336
aF-0.819204
a(lp1635
g3
(g7
S"2>\x12'\xc3\xac\xee\xbf"
p1636
tp1637
Rp1638
ag3
(g7
S'%?\x80\x8c\ne\xed\xbf'
p1639
tp1640
Rp1641
ag3
(g7
S'\xd8B\x7f9(\xa8\xd7\xbf'
p1642
tp1643
Rp1644
a(lp1645
F-0.9585891497717453
aF-0.9185841316375205
aF-0.41793322866047977
aF-0.36963849654152425
atp1646
a(F1.85
(lp1647
F-0.940083
aF-0.940083
aF-0.816842
a(lp1648
g3
(g7
S'\x7fY\x08S\x91\xa6\xee\xbf'
p1649
tp1650
Rp1651
ag3
(g7
S')\x8d\xff~\xd9h\xed\xbf'
p1652
tp1653
Rp1654
ag3
(g7
S'\r$\xe1\x06\x17\xb4\xd7\xbf'
p1655
tp1656
Rp1657
a(lp1658
F-0.9578329679232377
aF-0.9190490227160003
aF-0.41725672013275933
aF-0.37036681815931166
atp1659
a(F1.8599999999999999
(lp1660
F-0.939839
aF-0.939839
aF-0.814501
a(lp1661
g3
(g7
S'#\xd1\xbf\x98\x88\xa0\xee\xbf'
p1662
tp1663
Rp1664
ag3
(g7
S'\xdfsQ\xd8\x8al\xed\xbf'
p1665
tp1666
Rp1667
ag3
(g7
S'>\x02o\x1dE\xbf\xd7\xbf'
p1668
tp1669
Rp1670
a(lp1671
F-0.9570963843712297
aF-0.9194998002018305
aF-0.41657129164510986
aF-0.3710491931379094
atp1672
a(F1.87
(lp1673
F-0.939604
aF-0.939604
aF-0.812179
a(lp1674
g3
(g7
S'"\x06\xee7\xa8\x9a\xee\xbf'
p1675
tp1676
Rp1677
ag3
(g7
S'\xfa\xeb\x80r\x1fp\xed\xbf'
p1678
tp1679
Rp1680
ag3
(g7
S'\xc0=\xe6\xaf\xb7\xc9\xd7\xbf'
p1681
tp1682
Rp1683
a(lp1684
F-0.9563790409449128
aF-0.9199368702314801
aF-0.41587737749849973
aF-0.371686860825287
atp1685
a(F1.88
(lp1686
F-0.939378
aF-0.939378
aF-0.809877
a(lp1687
g3
(g7
S'nZ\x9fo\xef\x94\xee\xbf'
p1688
tp1689
Rp1690
ag3
(g7
S'\xe99\xae!\x98s\xed\xbf'
p1691
tp1692
Rp1693
ag3
(g7
S'\xd7s6\xd9s\xd3\xd7\xbf'
p1694
tp1695
Rp1696
a(lp1697
F-0.9556805782438688
aF-0.9203606279205003
aF-0.41517539943787984
aF-0.3722810384004406
atp1698
a(F1.8900000000000001
(lp1699
F-0.939159
aF-0.939159
aF-0.807595
a(lp1700
g3
(g7
S'!Tw~]\x8f\xee\xbf'
p1701
tp1702
Rp1703
ag3
(g7
S'\xff\xde5\xb4\xf5v\xed\xbf'
p1704
tp1705
Rp1706
ag3
(g7
S'\xb2\xd5\x98\x9c~\xdc\xd7\xbf'
p1707
tp1708
Rp1709
a(lp1710
F-0.9550006361047318
aF-0.9207714576468502
aF-0.4144657669667503
aF-0.3728329209582979
atp1711
a(F1.9
(lp1712
F-0.938948
aF-0.938948
aF-0.805333
a(lp1713
g3
(g7
S'\xce9\xee\xa2\xf1\x89\xee\xbf'
p1714
tp1715
Rp1716
ag3
(g7
S'\x1e\x94\xd6\xf28z\xed\xbf'
p1717
tp1718
Rp1719
ag3
(g7
S'CK\xa9\xe5\xdc\xe4\xd7\xbf'
p1720
tp1721
Rp1722
a(lp1723
F-0.9543388540494613
aF-0.9211697333272499
aF-0.41374887765408985
aF-0.37334368160115794
atp1724
a(F1.9100000000000001
(lp1725
F-0.938745
aF-0.938745
aF-0.80309
a(lp1726
g3
(g7
S'Z"\x8c\x1b\xab\x84\xee\xbf'
p1727
tp1728
Rp1729
ag3
(g7
S'8Q\xd6\xa0b}\xed\xbf'
p1730
tp1731
Rp1732
ag3
(g7
S'\x10\x93\x81\x88\x93\xec\xd7\xbf'
p1733
tp1734
Rp1735
a(lp1736
F-0.9536948717150817
aF-0.9215558186865905
aF-0.4130251174341103
aF-0.3738144715373874
atp1737
a(F1.92
(lp1738
F-0.938549
aF-0.938549
aF-0.800868
a(lp1739
g3
(g7
S"6s!'\x89\x7f\xee\xbf"
p1740
tp1741
Rp1742
ag3
(g7
S'\x9fi&|s\x80\xed\xbf'
p1743
tp1744
Rp1745
ag3
(g7
S'QY\xd6A\xa7\xf3\xd7\xbf'
p1746
tp1747
Rp1748
a(lp1749
F-0.9530683292647157
aF-0.9219300675206805
aF-0.41229486089886025
aF-0.3742464201872236
atp1750
a(F1.9300000000000002
(lp1751
F-0.93836
aF-0.93836
aF-0.798665
a(lp1752
g3
(g7
S'\xdc\xcb\xfc\x04\x8bz\xee\xbf'
p1753
tp1754
Rp1755
ag3
(g7
S'\xfe\xbc\x86=l\x83\xed\xbf'
p1756
tp1757
Rp1758
ag3
(g7
S'\xd0p\x16\xb7\x1c\xfa\xd7\xbf'
p1759
tp1760
Rp1761
a(lp1762
F-0.952458867779906
aF-0.9222928239522898
aF-0.4115584715838498
aF-0.37464063529638336
atp1763
a(F1.94
(lp1764
F-0.938178
aF-0.938178
aF-0.796482
a(lp1765
g3
(g7
S'\xc2c\x1e\xf5\xafu\xee\xbf'
p1766
tp1767
Rp1768
ag3
(g7
S'\x11\x0b\xa8\x98M\x86\xed\xbf'
p1769
tp1770
Rp1771
ag3
(g7
S'\xdb*\x8cv\xf8\xff\xd7\xbf'
p1772
tp1773
Rp1774
a(lp1775
F-0.9518661296343608
aF-0.9226444226809203
aF-0.41081630224673976
aF-0.3749982030573586
atp1776
a(F1.9500000000000002
(lp1777
F-0.938002
aF-0.938002
aF-0.794318
a(lp1778
g3
(g7
S'\xc4\xd3h8\xf7p\xee\xbf'
p1779
tp1780
Rp1781
ag3
(g7
S'vdM<\x18\x89\xed\xbf'
p1782
tp1783
Rp1784
ag3
(g7
S'\xfb\xe2\x80\xf7>\x05\xd8\xbf'
p1785
tp1786
Rp1787
a(lp1788
F-0.9512897588489222
aF-0.9229851892261103
aF-0.41006869513944977
aF-0.375320188238717
atp1789
a(F1.96
(lp1790
F-0.937832
aF-0.937832
aF-0.792174
a(lp1791
g3
(g7
S'\x10Y\xcf\x10`l\xee\xbf'
p1792
tp1793
Rp1794
ag3
(g7
S'\x15\xcbl\xd2\xcc\x8b\xed\xbf'
p1795
tp1796
Rp1797
ag3
(g7
S'\x86\xbbb\x9a\xf4\t\xd8\xbf'
p1798
tp1799
Rp1800
a(lp1801
F-0.9507294014281639
aF-0.9233154401648304
aF-0.40931598227360977
aF-0.3756076343224156
atp1802
a(F1.9699999999999998
(lp1803
F-0.937669
aF-0.937669
aF-0.790049
a(lp1804
g3
(g7
S'\xf3\x8a\x81\xc1\xe9g\xee\xbf'
p1805
tp1806
Rp1807
ag3
(g7
S'\x93\xf5N\x00l\x8e\xed\xbf'
p1808
tp1809
Rp1810
ag3
(g7
S'\x0e\x98\xec\xa8\x1d\x0e\xd8\xbf'
p1811
tp1812
Rp1813
a(lp1814
F-0.9501847056784217
aF-0.9236354833625902
aF-0.40855848567960945
aF-0.3758615636492076
atp1815
a(F1.98
(lp1816
F-0.937511
aF-0.937511
aF-0.787944
a(lp1817
g3
(g7
S'\x93\x96\x14\x8f\x93c\xee\xbf'
p1818
tp1819
Rp1820
ag3
(g7
S'\xe3O\xaef\xf6\x90\xed\xbf'
p1821
tp1822
Rp1823
ag3
(g7
S'ZTPV\xbe\x11\xd8\xbf'
p1824
tp1825
Rp1826
a(lp1827
F-0.9496553225078104
aF-0.9239456181990107
aF-0.40779651765937114
aF-0.3760829775722593
atp1828
a(F1.9899999999999998
(lp1829
F-0.937359
aF-0.937359
aF-0.785859
a(lp1830
g3
(g7
S'x\xfe\xa9\xbf\\_\xee\xbf'
p1831
tp1832
Rp1833
ag3
(g7
S'\xab.\xd5\xa1l\x93\xed\xbf'
p1834
tp1835
Rp1836
ag3
(g7
S'H3c\xbf\xda\x14\xd8\xbf'
p1837
tp1838
Rp1839
a(lp1840
F-0.949140905708147
aF-0.9242461357875602
aF-0.40703038103302014
aF-0.37627285661874277
atp1841
a(F2.0
(lp1842
F-0.937213
aF-0.937213
aF-0.783793
a(lp1843
g3
(g7
S'\x02\xeb\x13\x9bD[\xee\xbf'
p1844
tp1845
Rp1846
ag3
(g7
S'0;\xbbI\xcf\x95\xed\xbf'
p1847
tp1848
Rp1849
ag3
(g7
S'!\x84\xcc\xeav\x17\xd8\xbf'
p1850
tp1851
Rp1852
a(lp1853
F-0.9486411122191777
aF-0.9245373191896301
aF-0.40626036937951004
aF-0.37643216065959145
atp1854
a(F2.01
(lp1855
F-0.937071
aF-0.937071
aF-0.781746
a(lp1856
g3
(g7
S'P\x19\xf7jJW\xee\xbf'
p1857
tp1858
Rp1859
ag3
(g7
S'.,"\xf2\x1e\x98\xed\xbf'
p1860
tp1861
Rp1862
ag3
(g7
S'Gy6\xc9\x96\x19\xd8\xbf'
p1863
tp1864
Rp1865
a(lp1866
F-0.9481556023754728
aF-0.9248194436235104
aF-0.40548676727149
aF-0.3765618290871261
atp1867
a(F2.02
(lp1868
F-0.936935
aF-0.936935
aF-0.779718
a(lp1869
g3
(g7
S'rp\xeazmS\xee\xbf'
p1870
tp1871
Rp1872
ag3
(g7
S'\x14\xbd\xb1*\\\x9a\xed\xbf'
p1873
tp1874
Rp1875
ag3
(g7
S'\x13%\x815>\x1b\xd8\xbf'
p1876
tp1877
Rp1878
a(lp1879
F-0.9476840401362231
aF-0.9250927766678703
aF-0.40470985050443004
aF-0.3766627810005769
atp1880
a(F2.0300000000000002
(lp1881
F-0.936804
aF-0.936804
aF-0.777709
a(lp1882
g3
(g7
S'HD\x94\x18\xadO\xee\xbf'
p1883
tp1884
Rp1885
ag3
(g7
S'\xa8\xef\x12\x7f\x87\x9c\xed\xbf'
p1886
tp1887
Rp1888
ag3
(g7
S'\xa8\x87\xf7\xf4p\x1c\xd8\xbf'
p1889
tp1890
Rp1891
a(lp1892
F-0.9472260932981351
aF-0.92535757846007
aF-0.4039298863201499
aF-0.3767359153990746
atp1893
a(F2.04
(lp1894
F-0.936677
aF-0.936677
aF-0.77572
a(lp1895
g3
(g7
S'\x8ec\xc5\x93\x08L\xee\xbf'
p1896
tp1897
Rp1898
ag3
(g7
S'Q\xa6\nw\xa1\x9e\xed\xbf'
p1899
tp1900
Rp1901
ag3
(g7
S'\x96\xb0\x86\xb72\x1d\xd8\xbf'
p1902
tp1903
Rp1904
a(lp1905
F-0.9467814336922953
aF-0.9256141018897304
aF-0.4031471336249703
aF-0.3767821113822344
atp1906
a(F2.05
(lp1907
F-0.936555
aF-0.936555
aF-0.773749
a(lp1908
g3
(g7
S'\x00\xed\x91>\x7fH\xee\xbf'
p1909
tp1910
Rp1911
ag3
(g7
S'W\x8d\x93\x96\xaa\xa0\xed\xbf'
p1912
tp1913
Rp1914
ag3
(g7
S'\xa5\xdf\xf6\x17\x87\x1d\xd8\xbf'
p1915
tp1916
Rp1917
a(lp1918
F-0.9463497373648402
aF-0.9258625927872501
aF-0.4023618432026298
aF-0.37680222835796884
atp1919
a(F2.06
(lp1920
F-0.936437
aF-0.936437
aF-0.771798
a(lp1921
g3
(g7
S'\xb3\nhm\x10E\xee\xbf'
p1922
tp1923
Rp1924
ag3
(g7
S'\xbd^\xf7]\xa3\xa2\xed\xbf'
p1925
tp1926
Rp1927
ag3
(g7
S'~\x86&\x9cq\x1d\xd8\xbf'
p1928
tp1929
Rp1930
a(lp1931
F-0.9459306847423558
aF-0.92610329010764
aF-0.4015742579219602
aF-0.3767971062571638
atp1932
a(F2.0700000000000003
(lp1933
F-0.936323
aF-0.936323
aF-0.769865
a(lp1934
g3
(g7
S'-\x92$w\xbbA\xee\xbf'
p1935
tp1936
Rp1937
ag3
(g7
S'\xf8\x84\xe7I\x8c\xa4\xed\xbf'
p1938
tp1939
Rp1940
ag3
(g7
S'\x96$G\xb5\xf5\x1c\xd8\xbf'
p1941
tp1942
Rp1943
a(lp1944
F-0.9455239607819457
aF-0.9263364261097702
aF-0.40078461293959006
aF-0.3767675657550839
atp1945
a(F2.08
(lp1946
F-0.936213
aF-0.936213
aF-0.76795
a(lp1947
g3
(g7
S'i\xb1%\xb5\x7f>\xee\xbf'
p1948
tp1949
Rp1950
ag3
(g7
S'\xdb$\x95\xd3e\xa6\xed\xbf'
p1951
tp1952
Rp1953
ag3
(g7
S'\xe7\xee\x1b\xc0\x16\x1c\xd8\xbf'
p1954
tp1955
Rp1956
a(lp1957
F-0.9451292551071157
aF-0.92656222653127
aF-0.3999931358978498
aF-0.37671440849929355
atp1958
a(F2.09
(lp1959
F-0.936107
aF-0.936107
aF-0.766055
a(lp1960
g3
(g7
S'\xc6\x9e[\x83\\;\xee\xbf'
p1961
tp1962
Rp1963
ag3
(g7
S'-\x83\xc8p0\xa8\xed\xbf'
p1964
tp1965
Rp1966
ag3
(g7
S'E\x16:\x05\xd8\x1a\xd8\xbf'
p1967
tp1968
Rp1969
a(lp1970
F-0.9447462621291931
aF-0.9267809107587703
aF-0.39920004711770996
aF-0.37663841734351616
atp1971
a(F2.0999999999999996
(lp1972
F-0.936005
aF-0.936005
aF-0.764178
a(lp1973
g3
(g7
S'\xe6sW@Q8\xee\xbf'
p1974
tp1975
Rp1976
ag3
(g7
S'}\xe3\xf7\x93\xec\xa9\xed\xbf'
p1977
tp1978
Rp1979
ag3
(g7
S'\xec\xafJ\xb9<\x19\xd8\xbf'
p1980
tp1981
Rp1982
a(lp1983
F-0.9443746811554062
aF-0.9269926919943001
aF-0.3984055597873797
aF-0.37654035658738316
atp1984
a(F2.11
(lp1985
F-0.935906
aF-0.935906
aF-0.762319
a(lp1986
g3
(g7
S'd5XM]5\xee\xbf'
p1987
tp1988
Rp1989
ag3
(g7
S'\xcd\xc8]\xac\x9a\xab\xed\xbf'
p1990
tp1991
Rp1992
ag3
(g7
S'\xa9\x13N\xfdG\x17\xd8\xbf'
p1993
tp1994
Rp1995
a(lp1996
F-0.9440142164836903
aF-0.9271977774172002
aF-0.3976098801460801
aF-0.3764209722215188
atp1997
a(F2.12
(lp1998
F-0.935811
aF-0.935811
aF-0.760479
a(lp1999
g3
(g7
S'\\%V\x0e\x802\xee\xbf'
p2000
tp2001
Rp2002
ag3
(g7
S'\x0c\xb4\x0e&;\xad\xed\xbf'
p2003
tp2004
Rp2005
ag3
(g7
S'\x85\xa5\xe0\xde\xfc\x14\xd8\xbf'
p2006
tp2007
Rp2008
a(lp2009
F-0.9436645774850763
aF-0.9273963683423302
aF-0.3968132076637098
aF-0.37628099217780336
atp2010
a(F2.13
(lp2011
F-0.93572
aF-0.93572
aF-0.758656
a(lp2012
g3
(g7
S'\xf0i\x0c\xea\xb8/\xee\xbf'
p2013
tp2014
Rp2015
ag3
(g7
S'\xb6R\x0ej\xce\xae\xed\xbf'
p2016
tp2017
Rp2018
ag3
(g7
S'-\xe8\x80X^\x12\xd8\xbf'
p2019
tp2020
Rp2021
a(lp2022
F-0.9433254786738963
aF-0.9275886603741902
aF-0.3960157352160299
aF-0.3761211265842826
atp2023
a(F2.1399999999999997
(lp2024
F-0.935631
aF-0.935631
aF-0.756852
a(lp2025
g3
(g7
S'\x14\x1b\x01J\x07-\xee\xbf'
p2026
tp2027
Rp2028
ag3
(g7
S"\x80'd\xdeT\xb0\xed\xbf"
p2029
tp2030
Rp2031
ag3
(g7
S'@\xc2\xd6Qo\x0f\xd8\xbf'
p2032
tp2033
Rp2034
a(lp2035
F-0.9429966397663933
aF-0.9277748435572298
aF-0.39521764925578984
aF-0.3759420680244463
atp2036
a(F2.15
(lp2037
F-0.935546
aF-0.935546
aF-0.755066
a(lp2038
g3
(g7
S'\x80\xd4\x8b\x9aj*\xee\xbf'
p2039
tp2040
Rp2041
ag3
(g7
S'\xee\xb8/\xe6\xce\xb1\xed\xbf'
p2042
tp2043
Rp2044
ag3
(g7
S',\xdd\xfb\x9f2\x0c\xd8\xbf'
p2045
tp2046
Rp2047
a(lp2048
F-0.9426777857285198
aF-0.9279551025227003
aF-0.39441912997976003
aF-0.37574449180051966
atp2049
a(F2.16
(lp2050
F-0.935464
aF-0.935464
aF-0.753298
a(lp2051
g3
(g7
S"\x82\xcb\xdaJ\xe2'\xee\xbf"
p2052
tp2053
Rp2054
ag3
(g7
S'\xc75\xbc\xe1<\xb3\xed\xbf'
p2055
tp2056
Rp2057
ag3
(g7
S'\xf2\xff\xc4\x05\xab\x08\xd8\xbf'
p2058
tp2059
Rp2060
a(lp2061
F-0.9423686468129376
aF-0.92812961663156
aF-0.3936203514918197
aF-0.375529056200321
atp2062
a(F2.17
(lp2063
F-0.935384
aF-0.935384
aF-0.751547
a(lp2064
g3
(g7
S'6\x8d\xf6\xccm%\xee\xbf'
p2065
tp2066
Rp2067
ag3
(g7
S'K\xa8\x93.\x9f\xb4\xed\xbf'
p2068
tp2069
Rp2070
ag3
(g7
S'\xf7Q\x0c4\xdb\x04\xd8\xbf'
p2071
tp2072
Rp2073
a(lp2074
F-0.9420689585862537
aF-0.9282985601141803
aF-0.3928214819622006
aF-0.37529640276741605
atp2075
a(F2.1799999999999997
(lp2076
F-0.935308
aF-0.935308
aF-0.749815
a(lp2077
g3
(g7
S'\xc6h\xc4\x95\x0c#\xee\xbf'
p2078
tp2079
Rp2080
ag3
(g7
S"\xe8\xaa\x91'\xf6\xb5\xed\xbf"
p2081
tp2082
Rp2083
ag3
(g7
S'\xa9\\\xfc\xc9\xc5\x00\xd8\xbf'
p2084
tp2085
Rp2086
a(lp2087
F-0.9417784619465912
aF-0.9284621022064503
aF-0.39202268378298993
aF-0.37504715657400856
atp2088
a(F2.19
(lp2089
F-0.935234
aF-0.935234
aF-0.748099
a(lp2090
g3
(g7
S'<\xa3\x07\x1d\xbe \xee\xbf'
p2091
tp2092
Rp2093
ag3
(g7
S'\x1f\xab\xf5$B\xb7\xed\xbf'
p2094
tp2095
Rp2096
ag3
(g7
S'E\xcf[Um\xfc\xd7\xbf'
p2097
tp2098
Rp2099
a(lp2100
F-0.9414969031323382
aF-0.9286204072826403
aF-0.39122411371994004
aF-0.37478192649654124
atp2101
a(F2.2
(lp2102
F-0.935162
aF-0.935162
aF-0.746401
a(lp2103
g3
(g7
S'\xba|a\xdd\x81\x1e\xee\xbf'
p2104
tp2105
Rp2106
ag3
(g7
S'\xfa\xb9t|\x83\xb8\xed\xbf'
p2107
tp2108
Rp2109
ag3
(g7
S'\xde\xbb\xd9R\xd4\xf7\xd7\xbf'
p2110
tp2111
Rp2112
a(lp2113
F-0.9412240337222987
aF-0.9287736349850203
aF-0.3904259230607199
aF-0.37450130549308047
atp2114
a(F2.21
(lp2115
F-0.935094
aF-0.935094
aF-0.744721
a(lp2116
g3
(g7
S'x\x1bPTW\x1c\xee\xbf'
p2117
tp2118
Rp2119
ag3
(g7
S';\xefJ\x81\xba\xb9\xed\xbf'
p2120
tp2121
Rp2122
ag3
(g7
S'\xb8}Z.\xfd\xf2\xd7\xbf'
p2123
tp2124
Rp2125
a(lp2126
F-0.9409596106278137
aF-0.9289219403503697
aF-0.38962825775988985
aF-0.3742058708830565
atp2127
a(F2.2199999999999998
(lp2128
F-0.935027
aF-0.935027
aF-0.743057
a(lp2129
g3
(g7
S'\xc4~,\x02>\x1a\xee\xbf'
p2130
tp2131
Rp2132
ag3
(g7
S'.TL\x84\xe7\xba\xed\xbf'
p2133
tp2134
Rp2135
ag3
(g7
S'\xec\x9aDC\xea\xed\xd7\xbf'
p2136
tp2137
Rp2138
a(lp2139
F-0.9407033960778436
aF-0.9290654739330705
aF-0.38883125857997014
aF-0.3738961846269561
atp2140
a(F2.23
(lp2141
F-0.934963
aF-0.934963
aF-0.741411
a(lp2142
g3
(g7
S"\xccV'j5\x18\xee\xbf"
p2143
tp2144
Rp2145
ag3
(g7
S'Y}\xf5\xd3\n\xbc\xed\xbf'
p2146
tp2147
Rp2148
ag3
(g7
S'\xb9\x9d\xce\xdc\x9d\xe8\xd7\xbf'
p2149
tp2150
Rp2151
a(lp2152
F-0.9404551575959986
aF-0.9292043819258802
aF-0.38803506122993947
aF-0.37357279360955054
atp2153
a(F2.24
(lp2154
F-0.934901
aF-0.934901
aF-0.739781
a(lp2155
g3
(g7
S'~\x18E\x12=\x16\xee\xbf'
p2156
tp2157
Rp2158
ag3
(g7
S'b\xa3{\xbc$\xbd\xed\xbf'
p2159
tp2160
Rp2161
ag3
(g7
S'yrL6\x1a\xe3\xd7\xbf'
p2162
tp2163
Rp2164
a(lp2165
F-0.9402146679720003
aF-0.92933880627707
aF-0.3872397964999302
aF-0.37323622992133926
atp2166
a(F2.25
(lp2167
F-0.934841
aF-0.934841
aF-0.738169
a(lp2168
g3
(g7
S'\x84+Y\x83T\x14\xee\xbf'
p2169
tp2170
Rp2171
ag3
(g7
S'\xaae\xdc\x875\xbe\xed\xbf'
p2172
tp2173
Rp2174
ag3
(g7
S'\xe69}{a\xdd\xd7\xbf'
p2175
tp2176
Rp2177
a(lp2178
F-0.9399817052266001
aF-0.92946888480508
aF-0.38644559039299936
aF-0.3728870111416691
atp2179
a(F2.26
(lp2180
F-0.934784
aF-0.934784
aF-0.736573
a(lp2181
g3
(g7
S'\x8bM\x00I{\x12\xee\xbf'
p2182
tp2183
Rp2184
ag3
(g7
S'}&\xed}=\xbf\xed\xbf'
p2185
tp2186
Rp2187
ag3
(g7
S'L\x06\xd9\xc8u\xd7\xd7\xbf'
p2188
tp2189
Rp2190
a(lp2191
F-0.9397560525707587
aF-0.9295947513102906
aF-0.38565256425381056
aF-0.3725256406215508
atp2192
a(F2.27
(lp2193
F-0.934728
aF-0.934728
aF-0.734993
a(lp2194
g3
(g7
S'LA\x9a\xf1\xb0\x10\xee\xbf'
p2195
tp2196
Rp2197
ag3
(g7
S'U\x0bj\xe4<\xc0\xed\xbf'
p2198
tp2199
Rp2200
ag3
(g7
S'z\x8d\xde+Y\xd1\xd7\xbf'
p2201
tp2202
Rp2203
a(lp2204
F-0.9395374983596771
aF-0.9297165356841601
aF-0.38486083489440004
aF-0.3721526077663017
atp2205
a(F2.2800000000000002
(lp2206
F-0.934675
aF-0.934675
aF-0.73343
a(lp2207
g3
(g7
S'\xc6\xceB\x0e\xf5\x0e\xee\xbf'
p2208
tp2209
Rp2210
ag3
(g7
S'\x18\x97\x04\xff3\xc1\xed\xbf'
p2211
tp2212
Rp2213
ag3
(g7
S'\xbb\xac`\xa3\r\xcb\xd7\xbf'
p2214
tp2215
Rp2216
a(lp2217
F-0.9393258360418825
aF-0.9298343640154803
aF-0.3840705147168605
aF-0.37176838831755776
atp2218
a(F2.29
(lp2219
F-0.934623
aF-0.934623
aF-0.731884
a(lp2220
g3
(g7
S'\x84&\xca2G\r\xee\xbf'
p2221
tp2222
Rp2223
ag3
(g7
S'\x1b\xf1q\x0f#\xc2\xed\xbf'
p2224
tp2225
Rp2226
ag3
(g7
S'\x84\xac\xd3\x1f\x95\xc4\xd7\xbf'
p2227
tp2228
Rp2229
a(lp2230
F-0.9391208641038273
aF-0.9299483586942502
aF-0.3832817118332896
aF-0.3713734446343518
atp2231
a(F2.3
(lp2232
F-0.934573
aF-0.934573
aF-0.730353
a(lp2233
g3
(g7
S'\xec\xb7\xac\xf5\xa6\x0b\xee\xbf'
p2234
tp2235
Rp2236
ag3
(g7
S'\xbb\xcexU\n\xc3\xed\xbf'
p2237
tp2238
Rp2239
ag3
(g7
S'\x1e<\x9a\x83\xf1\xbd\xd7\xbf'
p2240
tp2241
Rp2242
a(lp2243
F-0.9389223860105155
aF-0.9300586385129102
aF-0.3824945301829103
aF-0.3709682259731743
atp2244
a(F2.31
(lp2245
F-0.934525
aF-0.934525
aF-0.728839
a(lp2246
g3
(g7
S'^\x84\n\xf0\x13\n\xee\xbf'
p2247
tp2248
Rp2249
ag3
(g7
S'\x13\x08\xff\x0e\xea\xc3\xed\xbf'
p2250
tp2251
Rp2252
ag3
(g7
S'\xbc\x06R\xa3$\xb7\xd7\xbf'
p2253
tp2254
Rp2255
a(lp2256
F-0.9387302101423622
aF-0.93016531876515
aF-0.38170906964651025
aF-0.3705531687665865
atp2257
a(F2.3200000000000003
(lp2258
F-0.934478
aF-0.934478
aF-0.72734
a(lp2259
g3
(g7
S'd\xf7\x9d\xbd\x8d\x08\xee\xbf'
p2260
tp2261
Rp2262
ag3
(g7
S'r\xd3\x16x\xc2\xc4\xed\xbf'
p2263
tp2264
Rp2265
ag3
(g7
S'\x82\xca\x1fF0\xb0\xd7\xbf'
p2266
tp2267
Rp2268
a(lp2269
F-0.938544149728596
aF-0.9302685113421905
aF-0.3809254261580903
aF-0.37012869690003314
atp2270
a(F2.33
(lp2271
F-0.934433
aF-0.934433
aF-0.725858
a(lp2272
g3
(g7
S'4V\xb2\xfc\x13\x07\xee\xbf'
p2273
tp2274
Rp2275
ag3
(g7
S'C\xae\x0b\xcb\x93\xc5\xed\xbf'
p2276
tp2277
Rp2278
ag3
(g7
S'2\xf3\xfa%\x16\xa9\xd7\xbf'
p2279
tp2280
Rp2281
a(lp2282
F-0.9383640227776535
aF-0.9303683248267103
aF-0.38014369181401036
aF-0.36969522198687593
atp2283
a(F2.34
(lp2284
F-0.93439
aF-0.93439
aF-0.724391
a(lp2285
g3
(g7
S'`\xd4\x19N\xa6\x05\xee\xbf'
p2286
tp2287
Rp2288
ag3
(g7
S'\xe2\xf8n@^\xc6\xed\xbf'
p2289
tp2290
Rp2291
ag3
(g7
S':\xa1\xf8\xef\xd7\xa1\xd7\xbf'
p2292
tp2293
Rp2294
a(lp2295
F-0.938189652005018
aF-0.9304648645845897
aF-0.37936395497966957
aF-0.3692531436413615
atp2296
a(F2.3499999999999996
(lp2297
F-0.934348
aF-0.934348
aF-0.722939
a(lp2298
g3
(g7
S'\xaaM#UD\x04\xee\xbf'
p2299
tp2300
Rp2301
ag3
(g7
S'\xca;$\x0f"\xc7\xed\xbf'
p2302
tp2303
Rp2304
ag3
(g7
S'F\x00\x96Dw\x9a\xd7\xbf'
p2305
tp2306
Rp2307
a(lp2308
F-0.9380208647584612
aF-0.9305582328541901
aF-0.3785863003934697
aF-0.3688028497490485
atp2309
a(F2.36
(lp2310
F-0.934307
aF-0.934307
aF-0.721503
a(lp2311
g3
(g7
S'.\xb7\x8f\xb7\xed\x02\xee\xbf'
p2312
tp2313
Rp2314
ag3
(g7
S'L"ml\xdf\xc7\xed\xbf'
p2315
tp2316
Rp2317
ag3
(g7
S'h\xed\x01\xb8\xf5\x92\xd7\xbf'
p2318
tp2319
Rp2320
a(lp2321
F-0.9378574929412243
aF-0.9306485288335103
aF-0.37781080926851024
aF-0.3683447167347453
atp2322
a(F2.37
(lp2323
F-0.934268
aF-0.934268
aF-0.720082
a(lp2324
g3
(g7
S'\xc4R\x87\x1d\xa2\x01\xee\xbf'
p2325
tp2326
Rp2327
ag3
(g7
S'P)\xf5\x8b\x96\xc8\xed\xbf'
p2328
tp2329
Rp2330
ag3
(g7
S'j\xe1e\xd2T\x8b\xd7\xbf'
p2331
tp2332
Rp2333
a(lp2334
F-0.9376993729334445
aF-0.9307358487651903
aF-0.3770375593918303
aF-0.3678791098277749
atp2335
a(F2.38
(lp2336
F-0.93423
aF-0.93423
aF-0.718676
a(lp2337
g3
(g7
S' \xa8\x8e1a\x00\xee\xbf'
p2338
tp2339
Rp2340
ag3
(g7
S'\xbe\xff\xdc\x9fG\xc9\xed\xbf'
p2341
tp2342
Rp2343
ag3
(g7
S'[\x0e.\x10\x96\x83\xd7\xbf'
p2344
tp2345
Rp2346
a(lp2347
F-0.9375463455119222
aF-0.9308202860192903
aF-0.3762666252214301
aF-0.36740638332432735
atp2348
a(F2.3899999999999997
(lp2349
F-0.934194
aF-0.934194
aF-0.717286
a(lp2350
g3
(g7
S'\xefP{\xa0*\xff\xed\xbf'
p2351
tp2352
Rp2353
ag3
(g7
S'\xc3\xa0\xc5\xd8\xf2\xc9\xed\xbf'
p2354
tp2355
Rp2356
ag3
(g7
S'n\x98P\xe2\xba{\xd7\xbf'
p2357
tp2358
Rp2359
a(lp2360
F-0.9373982557686106
aF-0.93090193117407
aF-0.3754980779807499
aF-0.3669268808465689
atp2361
a(F2.4
(lp2362
F-0.934159
aF-0.934159
aF-0.71591
a(lp2363
g3
(g7
S'\xde\x9bh\x19\xfe\xfd\xed\xbf'
p2364
tp2365
Rp2366
ag3
(g7
S'-$\xdbe\x98\xca\xed\xbf'
p2367
tp2368
Rp2369
ag3
(g7
S'U\xf9\x93\xae\xc4s\xd7\xbf'
p2370
tp2371
Rp2372
a(lp2373
F-0.9372549530279415
aF-0.9309808720946705
aF-0.37473198575122996
aF-0.36644093559870783
atp2374
a(F2.41
(lp2375
F-0.934125
aF-0.934125
aF-0.714549
a(lp2376
g3
(g7
S'\xd6\x17\xacM\xdb\xfc\xed\xbf'
p2377
tp2378
Rp2379
ag3
(g7
S'vK\xdft8\xcb\xed\xbf'
p2380
tp2381
Rp2382
ag3
(g7
S'\x03p\xd4\xcf\xb4k\xd7\xbf'
p2383
tp2384
Rp2385
a(lp2386
F-0.9371162907634651
aF-0.9310571940098805
aF-0.3739684135624606
aF-0.36594887061960507
atp2387
a(F2.42
(lp2388
F-0.934092
aF-0.934092
aF-0.713203
a(lp2389
g3
(g7
S'(\x00\xca\xf0\xc1\xfb\xed\xbf'
p2390
tp2391
Rp2392
ag3
(g7
S'\x97\xc432\xd3\xcb\xed\xbf'
p2393
tp2394
Rp2395
ag3
(g7
S'(xH\x96\x8cc\xd7\xbf'
p2396
tp2397
Rp2398
a(lp2399
F-0.9369821265136175
aF-0.9311309795868001
aF-0.37320742348022024
aF-0.3654509990318526
atp2400
a(F2.4299999999999997
(lp2401
F-0.934061
aF-0.934061
aF-0.711871
a(lp2402
g3
(g7
S'\xd2\x9ei\xb8\xb1\xfa\xed\xbf'
p2403
tp2404
Rp2405
ag3
(g7
S'\xcf/\xe4\xc8h\xcc\xed\xbf'
p2406
tp2407
Rp2408
ag3
(g7
S'(J\xc4GM[\xd7\xbf'
p2409
tp2410
Rp2411
a(lp2412
F-0.9368523217971984
aF-0.9312023090037607
aF-0.37244907469249977
aF-0.3649476242873409
atp2413
a(F2.44
(lp2414
F-0.93403
aF-0.93403
aF-0.710553
a(lp2415
g3
(g7
S'\x98\xa2I\\\xaa\xf9\xed\xbf'
p2416
tp2417
Rp2418
ag3
(g7
S'\xc9\xdf\xafb\xf9\xcc\xed\xbf'
p2419
tp2420
Rp2421
ag3
(g7
S'zQ\xfc\x1f\xf8R\xd7\xbf'
p2422
tp2423
Rp2424
a(lp2425
F-0.9367267420285135
aF-0.9312712600212701
aF-0.37169342359342944
aF-0.3644390404090454
atp2426
a(F2.45
(lp2427
F-0.934
aF-0.934
aF-0.70925
a(lp2428
g3
(g7
S'8p4\x96\xab\xf8\xed\xbf'
p2429
tp2430
Rp2431
ag3
(g7
S'TX\x13(\x85\xcd\xed\xbf'
p2432
tp2433
Rp2434
ag3
(g7
S'v\x96\xc6P\x8eJ\xd7\xbf'
p2435
tp2436
Rp2437
a(lp2438
F-0.9366052564323631
aF-0.9313379080511001
aF-0.37094052386511994
aF-0.36392553222899604
atp2439
a(F2.46
(lp2440
F-0.933972
aF-0.933972
aF-0.707961
a(lp2441
g3
(g7
S'\xdcx\xf4!\xb5\xf7\xed\xbf'
p2442
tp2443
Rp2444
ag3
(g7
S'K\x91Q@\x0c\xce\xed\xbf'
p2445
tp2446
Rp2447
ag3
(g7
S'"\x1c[\x02\x11B\xd7\xbf'
p2448
tp2449
Rp2450
a(lp2451
F-0.936487737959193
aF-0.93140232622367
aF-0.37019042655764983
aF-0.3634073756224463
atp2452
a(F2.4699999999999998
(lp2453
F-0.933944
aF-0.933944
aF-0.706686
a(lp2454
g3
(g7
S'\x0e\x95H\xbd\xc6\xf6\xed\xbf'
p2455
tp2456
Rp2457
ag3
(g7
S'\xc0\xf8|\xd1\x8e\xce\xed\xbf'
p2458
tp2459
Rp2460
ag3
(g7
S']\x1f\x93S\x819\xd7\xbf'
p2461
tp2462
Rp2463
a(lp2464
F-0.9363740632003625
aF-0.9314645854535902
aF-0.3694431801670095
aF-0.3628848377379568
atp2465
a(F2.48
(lp2466
F-0.933918
aF-0.933918
aF-0.705425
a(lp2467
g3
(g7
S":o\xd8'\xe0\xf5\xed\xbf"
p2468
tp2469
Rp2470
ag3
(g7
S'$;\x80\x00\r\xcf\xed\xbf'
p2471
tp2472
Rp2473
ag3
(g7
S"dD'Z\xe00\xd7\xbf"
p2474
tp2475
Rp2476
a(lp2477
F-0.9362641123038661
aF-0.93152475450356
aF-0.36869883071123977
aF-0.36235817722360397
atp2478
a(F2.49
(lp2479
F-0.933892
aF-0.933892
aF-0.704177
a(lp2480
g3
(g7
S'\xd6\xf7(#\x01\xf5\xed\xbf'
p2481
tp2482
Rp2483
ag3
(g7
S'(\xcb&\xf1\x86\xcf\xed\xbf'
p2484
tp2485
Rp2486
ag3
(g7
S'a\x9e\xec"/(\xd7\xbf'
p2487
tp2488
Rp2489
a(lp2490
F-0.9361577688903201
aF-0.9315829000464402
aF-0.3679574218046198
aF-0.3618276444489992
atp2491
a(F2.5
(lp2492
F-0.933867
aF-0.933867
aF-0.702944
a(lp2493
g3
(g7
S'^\xf8\x90r)\xf4\xed\xbf'
p2494
tp2495
Rp2496
ag3
(g7
S'\x108%\xc6\xfc\xcf\xed\xbf'
p2497
tp2498
Rp2499
ag3
(g7
S'?\x9f\x10\xb2n\x1f\xd7\xbf'
p2500
tp2501
Rp2502
a(lp2503
F-0.9360549199698291
aF-0.9316390867259107
aF-0.36721899473023
aF-0.36129348172334014
atp2504
a(F2.51
(lp2505
F-0.933843
aF-0.933843
aF-0.701723
a(lp2506
g3
(g7
S'\xc0\xb5-\xdbX\xf3\xed\xbf'
p2507
tp2508
Rp2509
ag3
(g7
S'\xeeB!\xa1n\xd0\xed\xbf'
p2510
tp2511
Rp2512
ag3
(g7
S';\xdaS\x03\xa0\x16\xd7\xbf'
p2513
tp2514
Rp2515
a(lp2516
F-0.9359554558592929
aF-0.9316933772152806
aF-0.3664835885104804
aF-0.3607559235091763
atp2517
a(F2.52
(lp2518
F-0.93382
aF-0.93382
aF-0.700516
a(lp2519
g3
(g7
S'n\xb3\xd7#\x8f\xf2\xed\xbf'
p2520
tp2521
Rp2522
ag3
(g7
S'\x15\xc0\xb9\xa2\xdc\xd0\xed\xbf'
p2523
tp2524
Rp2525
ag3
(g7
S'\xf6\xa6C\n\xc4\r\xd7\xbf'
p2526
tp2527
Rp2528
a(lp2529
F-0.9358592701006335
aF-0.9317458322748302
aF-0.3657512399760493
aF-0.36021519663209617
atp2530
a(F2.5300000000000002
(lp2531
F-0.933798
aF-0.933798
aF-0.699323
a(lp2532
g3
(g7
S'\xca\x94\x17\x15\xcc\xf1\xed\xbf'
p2533
tp2534
Rp2535
ag3
(g7
S'^C\x8e\xeaF\xd1\xed\xbf'
p2536
tp2537
Rp2538
ag3
(g7
S'\xb9\x9dr\xb2\xdb\x04\xd7\xbf'
p2539
tp2540
Rp2541
a(lp2542
F-0.935766259379897
aF-0.93179651080764
aF-0.36502198383311996
aF-0.3596715204862125
atp2543
a(F2.54
(lp2544
F-0.933776
aF-0.933776
aF-0.698142
a(lp2545
g3
(g7
S'\x84!\x1by\x0f\xf1\xed\xbf'
p2546
tp2547
Rp2548
ag3
(g7
S'\xbc\x95F\x97\xad\xd1\xed\xbf'
p2549
tp2550
Rp2551
ag3
(g7
S'\xc4\xef\xaf\xdf\xe7\xfb\xd6\xbf'
p2552
tp2553
Rp2554
a(lp2555
F-0.9356763234473399
aF-0.9318454699138601
aF-0.3642958527289201
aF-0.35912510723550994
atp2556
a(F2.55
(lp2557
F-0.933755
aF-0.933755
aF-0.696975
a(lp2558
g3
(g7
S'jk\xaa\x1bY\xf0\xed\xbf'
p2559
tp2560
Rp2561
ag3
(g7
S'2\xf6\x99\xc6\x10\xd2\xed\xbf'
p2562
tp2563
Rp2564
ag3
(g7
S'L\x91=n\xe9\xf2\xd6\xbf'
p2565
tp2566
Rp2567
a(lp2568
F-0.9355893650384638
aF-0.9318927649434902
aF-0.3635728773155699
aF-0.35857616201089515
atp2569
a(F2.56
(lp2570
F-0.933735
aF-0.933735
aF-0.69582
a(lp2571
g3
(g7
S'\xfc\x1d\x1d\xca\xa8\xef\xed\xbf'
p2572
tp2573
Rp2574
ag3
(g7
S'\xec)V\x95p\xd2\xed\xbf'
p2575
tp2576
Rp2577
ag3
(g7
S'\xb0B\x053\xe1\xe9\xd6\xbf'
p2578
tp2579
Rp2580
a(lp2581
F-0.9355052897962525
aF-0.9319384495477704
aF-0.3628530863124103
aF-0.35802488310313696
atp2582
a(F2.5700000000000003
(lp2583
F-0.933716
aF-0.933716
aF-0.694678
a(lp2584
g3
(g7
S'2\xf6OS\xfe\xee\xed\xbf'
p2585
tp2586
Rp2587
ag3
(g7
S'\xb5Xf\x1f\xcd\xd2\xed\xbf'
p2588
tp2589
Rp2590
ag3
(g7
S'#w\xcc\xfb\xcf\xe0\xd6\xbf'
p2591
tp2592
Rp2593
a(lp2594
F-0.9354240061945285
aF-0.9319825757291003
aF-0.36213650656674023
aF-0.3574714621516813
atp2595
a(F2.58
(lp2596
F-0.933697
aF-0.933697
aF-0.693549
a(lp2597
g3
(g7
S'\xe0d\x9a\x87Y\xee\xed\xbf'
p2598
tp2599
Rp2600
ag3
(g7
S'\xe0\xba\xd9\x7f&\xd3\xed\xbf'
p2601
tp2602
Rp2603
ag3
(g7
S'\xb4\x0fg\x8f\xb6\xd7\xd6\xbf'
p2604
tp2605
Rp2606
a(lp2607
F-0.93534542546254
aF-0.9320251938896401
aF-0.3614231631130003
aF-0.3569160843292097
atp2608
a(F2.59
(lp2609
F-0.933678
aF-0.933678
aF-0.692432
a(lp2610
g3
(g7
S'\x00_\xc48\xba\xed\xed\xbf'
p2611
tp2612
Rp2613
ag3
(g7
S'\xe4\x18\xea\xd0|\xd3\xed\xbf'
p2614
tp2615
Rp2616
ag3
(g7
S'C\xf5\xe8\xad\x95\xce\xd6\xbf'
p2617
tp2618
Rp2619
a(lp2620
F-0.9352694615108414
aF-0.9320663528785906
aF-0.3607130792304305
aF-0.35635892852208795
atp2621
a(F2.5999999999999996
(lp2622
F-0.933661
aF-0.933661
aF-0.691328
a(lp2623
g3
(g7
S'qW\xfc9 \xed\xed\xbf'
p2624
tp2625
Rp2626
ag3
(g7
S'\x1b\x18\x02,\xd0\xd3\xed\xbf'
p2627
tp2628
Rp2629
ag3
(g7
S'A\x99\xd6\x10n\xc5\xd6\xbf'
p2630
tp2631
Rp2632
a(lp2633
F-0.9351960308583618
aF-0.9321061000380303
aF-0.36000627649939
aF-0.35580016750681714
atp2634
a(F2.61
(lp2635
F-0.933644
aF-0.933644
aF-0.690236
a(lp2636
g3
(g7
S'\x8el\xcd_\x8b\xec\xed\xbf'
p2637
tp2638
Rp2639
ag3
(g7
S'\xc1\\\xc3\xa9 \xd4\xed\xbf'
p2640
tp2641
Rp2642
ag3
(g7
S'sLTk@\xbc\xd6\xbf'
p2643
tp2644
Rp2645
a(lp2646
F-0.9351250525609353
aF-0.9321444812475403
aF-0.3593027748559597
aF-0.35523996812225406
atp2647
a(F2.62
(lp2648
F-0.933628
aF-0.933628
aF-0.689156
a(lp2649
g3
(g7
S'\xf6\xc2\x15\x80\xfb\xeb\xed\xbf'
p2650
tp2651
Rp2652
ag3
(g7
S'L\x83\x0cbn\xd4\xed\xbf'
p2653
tp2654
Rp2655
ag3
(g7
S'\x03\x81Tj\r\xb3\xd6\xbf'
p2656
tp2657
Rp2658
a(lp2659
F-0.9350564481411245
aF-0.9321815409676703
aF-0.35860259264544947
aF-0.35467849143789504
atp2660
a(F2.63
(lp2661
F-0.933612
aF-0.933612
aF-0.688088
a(lp2662
g3
(g7
S'\x00\x13\xfdqp\xeb\xed\xbf'
p2663
tp2664
Rp2665
ag3
(g7
S'A\xea\xfek\xb9\xd4\xed\xbf'
p2666
tp2667
Rp2668
ag3
(g7
S'\xb0\xf6\xc4\xb4\xd5\xa9\xd6\xbf'
p2669
tp2670
Rp2671
a(lp2672
F-0.934990141519478
aF-0.9322173222820501
aF-0.3579057466743503
aF-0.3541158929182118
atp2673
a(F2.6399999999999997
(lp2674
F-0.933596
aF-0.933596
aF-0.687032
a(lp2675
g3
(g7
S'\xaac\xeb\r\xea\xea\xed\xbf'
p2676
tp2677
Rp2678
ag3
(g7
S'\x91S\x04\xde\x01\xd5\xed\xbf'
p2679
tp2680
Rp2681
ag3
(g7
S'8\xc9\xba\xeb\x99\xa0\xd6\xbf'
p2682
tp2683
Rp2684
a(lp2685
F-0.9349260589470889
aF-0.93225186693836
aF-0.3572122522610005
aF-0.3535523225829309
atp2686
a(F2.65
(lp2687
F-0.933582
aF-0.933582
aF-0.685988
a(lp2688
g3
(g7
S'\xa2\xfd\x7f-h\xea\xed\xbf'
p2689
tp2690
Rp2691
ag3
(g7
S'\x8f]\xd4\xcdG\xd5\xed\xbf'
p2692
tp2693
Rp2694
ag3
(g7
S'fq\x9d\xaaZ\x97\xd6\xbf'
p2695
tp2696
Rp2697
a(lp2698
F-0.93486412893974
aF-0.9322852153881502
aF-0.3565221232848301
aF-0.35298792516348
atp2699
a(F2.66
(lp2700
F-0.933567
aF-0.933567
aF-0.684955
a(lp2701
g3
(g7
S'\x9c\x89\x88\xab\xea\xe9\xed\xbf'
p2702
tp2703
Rp2704
ag3
(g7
S'\x93\xd1yP\x8b\xd5\xed\xbf'
p2705
tp2706
Rp2707
ag3
(g7
S'>\xb7P\x87\x18\x8e\xd6\xbf'
p2708
tp2709
Rp2710
a(lp2711
F-0.9348042822132815
aF-0.9323174068254502
aF-0.35583537223443046
aF-0.3524228402555883
atp2712
a(F2.67
(lp2713
F-0.933553
aF-0.933553
aF-0.683935
a(lp2714
g3
(g7
S'4g\xf8cq\xe9\xed\xbf'
p2715
tp2716
Rp2717
ag3
(g7
S'\t\xd1Wz\xcc\xd5\xed\xbf'
p2718
tp2719
Rp2720
ag3
(g7
S'\x99\x9a]\x12\xd4\x84\xd6\xbf'
p2721
tp2722
Rp2723
a(lp2724
F-0.934746451620616
aF-0.9323484792244301
aF-0.35515201025437004
aF-0.3518572024681034
atp2725
a(F2.6799999999999997
(lp2726
F-0.93354
aF-0.93354
aF-0.682925
a(lp2727
g3
(g7
S'\x122\xe03\xfc\xe8\xed\xbf'
p2728
tp2729
Rp2730
ag3
(g7
S'\xd9\xd6._\x0b\xd6\xed\xbf'
p2731
tp2732
Rp2733
ag3
(g7
S'\xcd1\x1a\xd7\x8d{\xd6\xbf'
p2734
tp2735
Rp2736
a(lp2737
F-0.9346905720900073
aF-0.9323784693758301
aF-0.35447204719068964
aF-0.3512911415680522
atp2738
a(F2.69
(lp2739
F-0.933527
aF-0.933527
aF-0.681927
a(lp2740
g3
(g7
S'7|e\xf9\x8a\xe8\xed\xbf'
p2741
tp2742
Rp2743
ag3
(g7
S'\xe4\x95!\x12H\xd6\xed\xbf'
p2744
tp2745
Rp2746
ag3
(g7
S'\xe8\x85\xd0[Fr\xd6\xbf'
p2747
tp2748
Rp2749
a(lp2750
F-0.9346365805648754
aF-0.9324074129223706
aF-0.3537954916351503
aF-0.35072478262199386
atp2751
a(F2.7
(lp2752
F-0.933515
aF-0.933515
aF-0.680941
a(lp2753
g3
(g7
S'\x88\xb8\xba\x93\x1d\xe8\xed\xbf'
p2754
tp2755
Rp2756
ag3
(g7
S'\xe9\xb4\xb9\xa5\x82\xd6\xed\xbf'
p2757
tp2758
Rp2759
ag3
(g7
S'Ww\xe4!\xfeh\xd6\xbf'
p2760
tp2761
Rp2762
a(lp2763
F-0.9345844159449971
aF-0.9324353443932102
aF-0.3531223509685296
aF-0.35015824613389157
atp2764
a(F2.71
(lp2765
F-0.933503
aF-0.933503
aF-0.679965
a(lp2766
g3
(g7
S'VY\x17\xe3\xb3\xe7\xed\xbf'
p2767
tp2768
Rp2769
ag3
(g7
S'\xfce\xec+\xbb\xd6\xed\xbf'
p2770
tp2771
Rp2772
ag3
(g7
S'p\x9f\xf8\xa5\xb5_\xd6\xbf'
p2773
tp2774
Rp2775
a(lp2776
F-0.9345340190291536
aF-0.93246229723735
aF-0.3524526314025299
aF-0.34959164817927607
atp2777
a(F2.7199999999999998
(lp2778
F-0.933491
aF-0.933491
aF-0.679001
a(lp2779
g3
(g7
S'\xb6"\xb0\xc8M\xe7\xed\xbf'
p2780
tp2781
Rp2782
ag3
(g7
S'\xe0\xdc\x1e\xb6\xf1\xd6\xed\xbf'
p2783
tp2784
Rp2785
ag3
(g7
S'hD\x12`mV\xd6\xbf'
p2786
tp2787
Rp2788
a(lp2789
F-0.9344853324592653
aF-0.9324883038561
aF-0.35178633802064
aF-0.34902510053604374
atp2790
a(F2.73
(lp2791
F-0.93348
aF-0.93348
aF-0.678047
a(lp2792
g3
(g7
S'\x94\xa5\xaf&\xeb\xe6\xed\xbf'
p2793
tp2794
Rp2795
ag3
(g7
S'\x17\xa0*U&\xd7\xed\xbf'
p2796
tp2797
Rp2798
ag3
(g7
S'\x9cS\xbc\xc3%M\xd6\xbf'
p2799
tp2800
Rp2801
a(lp2802
F-0.9344383006656922
aF-0.9325133956344904
aF-0.3511234748179101
aF-0.3484587108117075
atp2803
a(F2.74
(lp2804
F-0.933469
aF-0.933469
aF-0.677104
a(lp2805
g3
(g7
S'~\xf8.\xe0\x8b\xe6\xed\xbf'
p2806
tp2807
Rp2808
ag3
(g7
S'\x8e\xc0a\x19Y\xd7\xed\xbf'
p2809
tp2810
Rp2811
ag3
(g7
S'\xc8})@\xdfC\xd6\xbf'
p2812
tp2813
Rp2814
a(lp2815
F-0.93439286981426
aF-0.9325376029719503
aF-0.3504640447396699
aF-0.3478925825674792
atp2816
a(F2.75
(lp2817
F-0.933458
aF-0.933458
aF-0.676172
a(lp2818
g3
(g7
S'D\x97.\xd9/\xe6\xed\xbf'
p2819
tp2820
Rp2821
ag3
(g7
S'U\xed\x92\x12\x8a\xd7\xed\xbf'
p2822
tp2823
Rp2824
ag3
(g7
S'0^U@\x9a:\xd6\xbf'
p2825
tp2826
Rp2827
a(lp2828
F-0.9343489877544253
aF-0.9325609553119802
aF-0.3498080497191797
aF-0.3473268154388936
atp2829
a(F2.76
(lp2830
F-0.933448
aF-0.933448
aF-0.675251
a(lp2831
g3
(g7
S'Hv\x8f\xf6\xd6\xe5\xed\xbf'
p2832
tp2833
Rp2834
ag3
(g7
S'\xebg\rP\xb9\xd7\xed\xbf'
p2835
tp2836
Rp2837
ag3
(g7
S'^\xc5$+W1\xd6\xbf'
p2838
tp2839
Rp2840
a(lp2841
F-0.9343066039688849
aF-0.9325834811709202
aF-0.3491554907141801
aF-0.34676150525327476
atp2842
a(F2.77
(lp2843
F-0.933438
aF-0.933438
aF-0.67434
a(lp2844
g3
(g7
S'ZE\x0c\x1e\x81\xe5\xed\xbf'
p2845
tp2846
Rp2847
ag3
(g7
S'\xc0\xdd\xa4\xe0\xe6\xd7\xed\xbf'
p2848
tp2849
Rp2850
ag3
(g7
S"\xeb'\x85c\x16(\xd6\xbf"
p2851
tp2852
Rp2853
a(lp2854
F-0.934265669524545
aF-0.9326052081659603
aF-0.3485063677425599
aF-0.34619674414409407
atp2855
a(F2.7800000000000002
(lp2856
F-0.933429
aF-0.933429
aF-0.673439
a(lp2857
g3
(g7
S'\x93\xdd26.\xe5\xed\xbf'
p2858
tp2859
Rp2860
ag3
(g7
S'\x86!\xb5\xd2\x12\xd8\xed\xbf'
p2861
tp2862
Rp2863
ag3
(g7
S'\xee,\x8bH\xd8\x1e\xd6\xbf'
p2864
tp2865
Rp2866
a(lp2867
F-0.93422613702471
aF-0.9326261630422301
aF-0.3478606799169296
aF-0.34563262066212896
atp2868
a(F2.79
(lp2869
F-0.93342
aF-0.93342
aF-0.672549
a(lp2870
g3
(g7
S'\xfa\xe4]&\xde\xe4\xed\xbf'
p2871
tp2872
Rp2873
ag3
(g7
S'\x94\xce%4=\xd8\xed\xbf'
p2874
tp2875
Rp2876
ag3
(g7
S'\xeds\x905\x9d\x15\xd6\xbf'
p2877
tp2878
Rp2879
a(lp2880
F-0.9341879605628081
aF-0.9326463716992803
aF-0.3472184254784003
aF-0.34506921988378125
atp2881
a(F2.8
(lp2882
F-0.933411
aF-0.933411
aF-0.671669
a(lp2883
g3
(g7
S'\\\x94\xae\xd6\x90\xe4\xed\xbf'
p2884
tp2885
Rp2886
ag3
(g7
S'\xd8\xc6m\x12f\xd8\xed\xbf'
p2887
tp2888
Rp2889
ag3
(g7
S'\xc6\x80P\x82e\x0c\xd6\xbf'
p2890
tp2891
Rp2892
a(lp2893
F-0.9341510956770767
aF-0.93266585921648
aF-0.3465796018292392
aF-0.3445066235162929
atp2894
a(F2.81
(lp2895
F-0.933402
aF-0.933402
aF-0.670799
a(lp2896
g3
(g7
S'\x92\xb2\x060F\xe4\xed\xbf'
p2897
tp2898
Rp2899
ag3
(g7
S'\x13\x9f\x96z\x8d\xd8\xed\xbf'
p2900
tp2901
Rp2902
ag3
(g7
S'R\xe1\x04\x831\x03\xd6\xbf'
p2903
tp2904
Rp2905
a(lp2906
F-0.9341154993067726
aF-0.9326846498779303
aF-0.34594420556471017
aF-0.34394491000013727
atp2907
a(F2.8200000000000003
(lp2908
F-0.933394
aF-0.933394
aF-0.669939
a(lp2909
g3
(g7
S'\x90\xb7\x02\x1c\xfe\xe3\xed\xbf'
p2910
tp2911
Rp2912
ag3
(g7
S'\xab\xee?y\xb3\xd8\xed\xbf'
p2913
tp2914
Rp2915
ag3
(g7
S'\xa7\x8d\x80\x88\x01\xfa\xd5\xbf'
p2916
tp2917
Rp2918
a(lp2919
F-0.9340811297495163
aF-0.9327027671965503
aF-0.34531223250404997
aF-0.3433841546086232
atp2920
a(F2.83
(lp2921
F-0.933386
aF-0.933386
aF-0.669088
a(lp2922
g3
(g7
S'\x0e\x1a\xf4\x84\xb8\xe3\xed\xbf'
p2923
tp2924
Rp2925
ag3
(g7
S'\xa0\x84\xa2\x1a\xd8\xd8\xed\xbf'
p2926
tp2927
Rp2928
ag3
(g7
S'\xfa\x89J\xe0\xd5\xf0\xd5\xbf'
p2929
tp2930
Rp2931
a(lp2932
F-0.9340479466198426
aF-0.9327202339374204
aF-0.34468367772055974
aF-0.3428244295447767
atp2933
a(F2.84
(lp2934
F-0.933378
aF-0.933378
aF-0.668248
a(lp2935
g3
(g7
S'\xa8\xc5\xdbUu\xe3\xed\xbf'
p2936
tp2937
Rp2938
ag3
(g7
S'\xa1\x84\x93j\xfb\xd8\xed\xbf'
p2939
tp2940
Rp2941
ag3
(g7
S'\xdb\xc0\xb7\xd4\xae\xe7\xd5\xbf'
p2942
tp2943
Rp2944
a(lp2945
F-0.9340159108088996
aF-0.9327370721404304
aF-0.3440585355707499
aF-0.34226580403539
atp2946
a(F2.8499999999999996
(lp2947
F-0.933371
aF-0.933371
aF-0.667417
a(lp2948
g3
(g7
S'Q\xbddz4\xe3\xed\xbf'
p2949
tp2950
Rp2951
ag3
(g7
S'%n\x87t\x1d\xd9\xed\xbf'
p2952
tp2953
Rp2954
ag3
(g7
S'D5\x04\xad\x8c\xde\xd5\xbf'
p2955
tp2956
Rp2957
a(lp2958
F-0.9339849844454116
aF-0.9327533031423104
aF-0.3434367997228104
aF-0.34170834442268855
atp2959
a(F2.86
(lp2960
F-0.933363
aF-0.933363
aF-0.666596
a(lp2961
g3
(g7
S'\xcf\xe2\xde\xde\xf5\xe2\xed\xbf'
p2962
tp2963
Rp2964
ag3
(g7
S'\xe5\x0b\x95C>\xd9\xed\xbf'
p2965
tp2966
Rp2967
ag3
(g7
S'zwk\xado\xd5\xd5\xbf'
p2968
tp2969
Rp2970
a(lp2971
F-0.9339551308576918
aF-0.9327689475979899
aF-0.3428184631842092
aF-0.3411521142532974
atp2972
a(F2.87
(lp2973
F-0.933356
aF-0.933356
aF-0.665784
a(lp2974
g3
(g7
S'\xf6\xe79p\xb9\xe2\xed\xbf'
p2975
tp2976
Rp2977
ag3
(g7
S'\xb1Mx\xe2]\xd9\xed\xbf'
p2978
tp2979
Rp2980
ag3
(g7
S'\xcck@\x17X\xcc\xd5\xbf'
p2981
tp2982
Rp2983
a(lp2984
F-0.9339263145368468
aF-0.9327840255013401
aF-0.34220351832846
aF-0.34059717436474296
atp2985
a(F2.88
(lp2986
F-0.93335
aF-0.93335
aF-0.664982
a(lp2987
g3
(g7
S'l`\x00\x1c\x7f\xe2\xed\xbf'
p2988
tp2989
Rp2990
ag3
(g7
S'\xa0\x07\x95[|\xd9\xed\xbf'
p2991
tp2992
Rp2993
ag3
(g7
S'\xa1k\x04)F\xc3\xd5\xbf'
p2994
tp2995
Rp2996
a(lp2997
F-0.9338985011008952
aF-0.9327985562051601
aF-0.34159195692118005
aF-0.3400435829695938
atp2998
a(F2.8899999999999997
(lp2999
F-0.933343
aF-0.933343
aF-0.664189
a(lp3000
g3
(g7
S'\x8e\x00S\xd0F\xe2\xed\xbf'
p3001
tp3002
Rp3003
ag3
(g7
S'q\xa4\xf9\xb8\x99\xd9\xed\xbf'
p3004
tp3005
Rp3006
ag3
(g7
S'\xd3\xbe}\x1e:\xba\xd5\xbf'
p3007
tp3008
Rp3009
a(lp3010
F-0.9338716572601857
aF-0.9328125584408004
aF-0.3409837701454
aF-0.33949139573722414
atp3011
a(F2.9
(lp3012
F-0.933337
aF-0.933337
aF-0.663405
a(lp3013
g3
(g7
S'\x82\xfb\xe3{\x10\xe2\xed\xbf'
p3014
tp3015
Rp3016
ag3
(g7
S'X\xbfa\x04\xb6\xd9\xed\xbf'
p3017
tp3018
Rp3019
ag3
(g7
S'\xaap\xcd04\xb1\xd5\xbf'
p3020
tp3021
Rp3022
a(lp3023
F-0.9338457507836749
aF-0.9328260503370801
aF-0.34037894862611995
aF-0.3389406658732343
atp3024
a(F2.91
(lp3025
F-0.933331
aF-0.933331
aF-0.66263
a(lp3026
g3
(g7
S'\\\x82\xf2\r\xdc\xe1\xed\xbf'
p3027
tp3028
Rp3029
ag3
(g7
S'\x8b\xa48G\xd1\xd9\xed\xbf'
p3030
tp3031
Rp3032
ag3
(g7
S'd\x86\x84\x964\xa8\xd5\xbf'
p3033
tp3034
Rp3035
a(lp3036
F-0.9338207504661783
aF-0.9328390494385004
aF-0.33977748245404005
aF-0.3383914441966221
atp3037
a(F2.92
(lp3038
F-0.933325
aF-0.933325
aF-0.661864
a(lp3039
g3
(g7
S'\x8enFv\xa9\xe1\xed\xbf'
p3040
tp3041
Rp3042
ag3
(g7
S'\xfd\xcb\x9b\x8a\xeb\xd9\xed\xbf'
p3043
tp3044
Rp3045
ag3
(g7
S'Z\xad\xb8\x83;\x9f\xd5\xbf'
p3046
tp3047
Rp3048
a(lp3049
F-0.9337966260968233
aF-0.93285157272328
aF-0.3391793612089807
aF-0.33784377921502584
atp3050
a(F2.9299999999999997
(lp3051
F-0.933319
aF-0.933319
aF-0.661107
a(lp3052
g3
(g7
S'\x96\x04,\xa5x\xe1\xed\xbf'
p3053
tp3054
Rp3055
ag3
(g7
S'\xf23]\xd7\x04\xda\xed\xbf'
p3056
tp3057
Rp3058
ag3
(g7
S'r5\x18*I\x96\xd5\xbf'
p3059
tp3060
Rp3061
a(lp3062
F-0.9337733484282065
aF-0.9328636366204802
aF-0.33858457398204
aF-0.33729771719739354
atp3063
a(F2.94
(lp3064
F-0.933314
aF-0.933314
aF-0.660359
a(lp3065
g3
(g7
S'\x9e\xddo\x8bI\xe1\xed\xbf'
p3066
tp3067
Rp3068
ag3
(g7
S'-\xb2\x056\x1d\xda\xed\xbf'
p3069
tp3070
Rp3071
ag3
(g7
S'\xa8\x9c\xfd\xb8]\x8d\xd5\xbf'
p3072
tp3073
Rp3074
a(lp3075
F-0.9337508891466548
aF-0.9328752570268702
aF-0.3379931093976696
aF-0.3367533022450947
atp3076
a(F2.95
(lp3077
F-0.933309
aF-0.933309
aF-0.659619
a(lp3078
g3
(g7
S'\x08\xecZ\x1a\x1c\xe1\xed\xbf'
p3079
tp3080
Rp3081
ag3
(g7
S'\xfc-\xd7\xae4\xda\xed\xbf'
p3082
tp3083
Rp3084
ag3
(g7
S'Lr\x82]y\x84\xd5\xbf'
p3085
tp3086
Rp3087
a(lp3088
F-0.9337292208432479
aF-0.9328864493231196
aF-0.3374049556346795
aF-0.3362105763606321
atp3089
a(F2.96
(lp3090
F-0.933303
aF-0.933303
aF-0.658888
a(lp3091
g3
(g7
S'\xc4\xa2\xaeC\xf0\xe0\xed\xbf'
p3092
tp3093
Rp3094
ag3
(g7
S'\xe2\xcd\xceIK\xda\xed\xbf'
p3095
tp3096
Rp3097
ag3
(g7
S'\x03\xbd\x91B\x9c{\xd5\xbf'
p3098
tp3099
Rp3100
a(lp3101
F-0.9337083169858363
aF-0.93289722838966
aF-0.3368201004468197
aF-0.3356695795145732
atp3102
a(F2.9699999999999998
(lp3103
F-0.933298
aF-0.933298
aF-0.658166
a(lp3104
g3
(g7
S'::\xa1\xf9\xc5\xe0\xed\xbf'
p3105
tp3106
Rp3107
ag3
(g7
S'\x8b\x12\xa7\x0ea\xda\xed\xbf'
p3108
tp3109
Rp3110
ag3
(g7
S'\x19\xe1\xf9\x90\xc6r\xd5\xbf'
p3111
tp3112
Rp3113
a(lp3114
F-0.9336881518918915
aF-0.9329076086219905
aF-0.33623853118275016
aF-0.33513034971066774
atp3115
a(F2.98
(lp3116
F-0.933294
aF-0.933294
aF-0.657452
a(lp3117
g3
(g7
S'\xae\x0f\xda.\x9d\xe0\xed\xbf'
p3118
tp3119
Rp3120
ag3
(g7
S'\xcb\xe0\xd9\x04v\xda\xed\xbf'
p3121
tp3122
Rp3123
ag3
(g7
S's\xf8}o\xf8i\xd5\xbf'
p3124
tp3125
Rp3126
a(lp3127
F-0.9336687007021184
aF-0.9329176039455203
aF-0.33566023480534
aF-0.3345929230489506
atp3128
a(F2.99
(lp3129
F-0.933289
aF-0.933289
aF-0.656746
a(lp3130
g3
(g7
S'<$n\xd6u\xe0\xed\xbf'
p3131
tp3132
Rp3133
ag3
(g7
S'\x0b\x7f\xa23\x8a\xda\xed\xbf'
p3134
tp3135
Rp3136
ag3
(g7
S'z\xb0\xe6\x022a\xd5\xbf'
p3137
tp3138
Rp3139
a(lp3140
F-0.9336499393549569
aF-0.9329272278300503
aF-0.3350851979103701
aF-0.3340573337870934
atp3141
a(F3.0
(lp3142
F-0.933285
aF-0.933285
aF-0.656048
a(lp3143
g3
(g7
S'\xe7\xb4\xdc\xe3O\xe0\xed\xbf'
p3144
tp3145
Rp3146
ag3
(g7
S'\x91\x80\xff\xa1\x9d\xda\xed\xbf'
p3147
tp3148
Rp3149
ag3
(g7
S'\xb9\xb6\x12nsX\xd5\xbf'
p3150
tp3151
Rp3152
a(lp3153
F-0.933631844561799
aF-0.9329364933037304
aF-0.33451340674483
aF-0.33352361440016043
atp3154
a(F3.01
(lp3155
F-0.93328
aF-0.93328
aF-0.655359
a(lp3156
g3
(g7
S'\x1c\xee\x0bK+\xe0\xed\xbf'
p3157
tp3158
Rp3159
ag3
(g7
S'\x9a\xa2\xb4V\xb0\xda\xed\xbf'
p3160
tp3161
Rp3162
ag3
(g7
S'\xb5\x9a\x06\xd2\xbcO\xd5\xbf'
p3163
tp3164
Rp3165
a(lp3166
F-0.9336143937829918
aF-0.9329454129666204
aF-0.33394484722435985
aF-0.3329917956383879
atp3167
a(F3.02
(lp3168
F-0.933276
aF-0.933276
aF-0.654678
a(lp3169
g3
(g7
S'P\xbcE\x00\x08\xe0\xed\xbf'
p3170
tp3171
Rp3172
ag3
(g7
S'\xe9\xa0LX\xc2\xda\xed\xbf'
p3173
tp3174
Rp3175
ag3
(g7
S'\xb7R\xfcM\x0eG\xd5\xbf'
p3176
tp3177
Rp3178
a(lp3179
F-0.9335975652046588
aF-0.9329539990040101
aF-0.33337950495055
aF-0.33246190658364144
atp3180
a(F3.0300000000000002
(lp3181
F-0.933272
aF-0.933272
aF-0.654004
a(lp3182
g3
(g7
S'\x10\xae4\xf8\xe5\xdf\xed\xbf'
p3183
tp3184
Rp3185
ag3
(g7
S'\xc7\xf0\x1a\xad\xd3\xda\xed\xbf'
p3186
tp3187
Rp3188
ag3
(g7
S'n=r\xffg>\xd5\xbf'
p3189
tp3190
Rp3191
a(lp3192
F-0.9335813377160224
aF-0.9329622631990107
aF-0.3328173652273301
aF-0.3319339747040067
atp3193
a(F3.04
(lp3194
F-0.933268
aF-0.933268
aF-0.653339
a(lp3195
g3
(g7
S"f\xf8\xe0'\xc5\xdf\xed\xbf"
p3196
tp3197
Rp3198
ag3
(g7
S'y|=[\xe4\xda\xed\xbf'
p3199
tp3200
Rp3201
ag3
(g7
S'\x14\xc09\x02\xca5\xd5\xbf'
p3202
tp3203
Rp3204
a(lp3205
F-0.9335656908877006
aF-0.9329702169451501
aF-0.3322584130771099
aF-0.33140802590696866
atp3206
a(F3.05
(lp3207
F-0.933265
aF-0.933265
aF-0.652681
a(lp3208
g3
(g7
S'\x84\x89\xad\x84\xa5\xdf\xed\xbf'
p3209
tp3210
Rp3211
ag3
(g7
S'mF\x9eh\xf4\xda\xed\xbf'
p3212
tp3213
Rp3214
ag3
(g7
S'\x9aq\x85p4-\xd5\xbf'
p3215
tp3216
Rp3217
a(lp3218
F-0.9335506049504123
aF-0.9329778712583002
aF-0.3317026332562397
aF-0.330884084590957
atp3219
a(F3.06
(lp3220
F-0.933261
aF-0.933261
aF-0.652031
a(lp3221
g3
(g7
S'\x049U\x04\x87\xdf\xed\xbf'
p3222
tp3223
Rp3224
ag3
(g7
S'\xde\x07\xf5\xda\x03\xdb\xed\xbf'
p3225
tp3226
Rp3227
ag3
(g7
S'B\xe8\xf6b\xa7$\xd5\xbf'
p3228
tp3229
Rp3230
a(lp3231
F-0.9335360607745139
aF-0.9329852367884501
aF-0.33115001027016966
aF-0.3303621736955649
atp3232
a(F3.07
(lp3233
F-0.933257
aF-0.933257
aF-0.651388
a(lp3234
g3
(g7
S'\xda\x0c\xe8\x9ci\xdf\xed\xbf'
p3235
tp3236
Rp3237
ag3
(g7
S'\x03\xbf\xc8\xb7\x12\xdb\xed\xbf'
p3238
tp3239
Rp3240
ag3
(g7
S'\xc2\x1c\xac\xf0"\x1c\xd5\xbf'
p3241
tp3242
Rp3243
a(lp3244
F-0.9335220398501411
aF-0.9329923238310305
aF-0.33060052838797044
aF-0.32984231475024806
atp3245
a(F3.08
(lp3246
F-0.933254
aF-0.933254
aF-0.650753
a(lp3247
g3
(g7
S'\xde\x8f\xc8DM\xdf\xed\xbf'
p3248
tp3249
Rp3250
ag3
(g7
S'\xbe0q\x04!\xdb\xed\xbf'
p3251
tp3252
Rp3253
ag3
(g7
S'\x98iL/\xa7\x13\xd5\xbf'
p3254
tp3255
Rp3256
a(lp3257
F-0.9335085242678323
aF-0.9329991423378705
aF-0.3300541716564504
aF-0.32932452792160744
atp3258
a(F3.09
(lp3259
F-0.933251
aF-0.933251
aF-0.650126
a(lp3260
g3
(g7
S'lD\xa9\xf21\xdf\xed\xbf'
p3261
tp3262
Rp3263
ag3
(g7
S'\x9fd\x18\xc6.\xdb\xed\xbf'
p3264
tp3265
Rp3266
ag3
(g7
S'\xe41\x1534\x0b\xd5\xbf'
p3267
tp3268
Rp3269
a(lp3270
F-0.9334954966999589
aF-0.9330057019280004
aF-0.3295109239139
aF-0.3288088320594207
atp3271
a(F3.1
(lp3272
F-0.933248
aF-0.933248
aF-0.649506
a(lp3273
g3
(g7
S'\xac#\x8a\x9d\x17\xdf\xed\xbf'
p3274
tp3275
Rp3276
ag3
(g7
S'\xd1\r\xbc\x01<\xdb\xed\xbf'
p3277
tp3278
Rp3279
ag3
(g7
S'o\x1f\xe6\x0e\xca\x02\xd5\xbf'
p3280
tp3281
Rp3282
a(lp3283
F-0.9334829403825222
aF-0.9330120118979098
aF-0.3289707688031892
aF-0.3282952447411767
atp3284
a(F3.11
(lp3285
F-0.933245
aF-0.933245
aF-0.648893
a(lp3286
g3
(g7
S'A6\xb6<\xfe\xde\xed\xbf'
p3287
tp3288
Rp3289
ag3
(g7
S'\xd9\xef.\xbcH\xdb\xed\xbf'
p3290
tp3291
Rp3292
ag3
(g7
S'\xe5\x18M\xd4h\xfa\xd4\xbf'
p3293
tp3294
Rp3295
a(lp3296
F-0.9334708390976588
aF-0.93301808123169
aF-0.3284336897847294
aF-0.3277837823155908
atp3297
a(F3.12
(lp3298
F-0.933242
aF-0.933242
aF-0.648287
a(lp3299
g3
(g7
S'9;\xc1\xc7\xe5\xde\xed\xbf'
p3300
tp3301
Rp3302
ag3
(g7
S'\x0e4\x1a\xfaT\xdb\xed\xbf'
p3303
tp3304
Rp3305
ag3
(g7
S'\xca\xc8\x91\x93\x10\xf2\xd4\xbf'
p3306
tp3307
Rp3308
a(lp3309
F-0.9334591771565556
aF-0.9330239186107302
aF-0.32789967014867
aF-0.3272744599445435
atp3310
a(F3.13
(lp3311
F-0.933239
aF-0.933239
aF-0.647689
a(lp3312
g3
(g7
S'Th\x856\xce\xde\xed\xbf'
p3313
tp3314
Rp3315
ag3
(g7
S'V\xba\xfe\xbf`\xdb\xed\xbf'
p3316
tp3317
Rp3318
ag3
(g7
S'\x8a\xec\xc0[\xc1\xe9\xd4\xbf'
p3319
tp3320
Rp3321
a(lp3322
F-0.9334479393830939
aF-0.9330295324232998
aF-0.3273686930270797
aF-0.3267672916442245
atp3323
a(F3.14
(lp3324
F-0.933236
aF-0.933236
aF-0.647097
a(lp3325
g3
(g7
S'\x003!\x81\xb7\xde\xed\xbf'
p3326
tp3327
Rp3328
ag3
(g7
S'nZ6\x12l\xdb\xed\xbf'
p3329
tp3330
Rp3331
ag3
(g7
S'\x184\xb7:{\xe1\xd4\xbf'
p3332
tp3333
Rp3334
a(lp3335
F-0.9334371110977306
aF-0.9330349307736702
aF-0.3268407414053897
aF-0.3262622903246787
atp3336
a(F3.15
(lp3337
F-0.933234
aF-0.933234
aF-0.646512
a(lp3338
g3
(g7
S'\x9d1\xf5\x9f\xa1\xde\xed\xbf'
p3339
tp3340
Rp3341
ag3
(g7
S'\xd6\x1e\xf5\xf4v\xdb\xed\xbf'
p3342
tp3343
Rp3344
ag3
(g7
S'f\xe2+=>\xd9\xd4\xbf'
p3345
tp3346
Rp3347
a(lp3348
F-0.933426678102069
aF-0.9330401214910702
aF-0.32631579813363026
aF-0.3257594678284812
atp3349
a(F3.16
(lp3350
F-0.933231
aF-0.933231
aF-0.645934
a(lp3351
g3
(g7
S'p\n\xa2\x8b\x8c\xde\xed\xbf'
p3352
tp3353
Rp3354
ag3
(g7
S'\xaduJl\x81\xdb\xed\xbf'
p3355
tp3356
Rp3357
ag3
(g7
S'\x88\x1a\xbbn\n\xd1\xd4\xbf'
p3358
tp3359
Rp3360
a(lp3361
F-0.933416626663826
aF-0.9330451121383503
aF-0.3257938459372504
aF-0.3252588349682033
atp3362
a(F3.17
(lp3363
F-0.933229
aF-0.933229
aF-0.645363
a(lp3364
g3
(g7
S'Ps\x06=x\xde\xed\xbf'
p3365
tp3366
Rp3367
ag3
(g7
S'VY"|\x8b\xdb\xed\xbf'
p3368
tp3369
Rp3370
ag3
(g7
S'\x1d\xe2\xef\xd9\xdf\xc8\xd4\xbf'
p3371
tp3372
Rp3373
a(lp3374
F-0.9334069435022718
aF-0.9330499100204106
aF-0.3252748674276101
aF-0.3247604015628283
atp3375
a(F3.1799999999999997
(lp3376
F-0.933226
aF-0.933226
aF-0.644799
a(lp3377
g3
(g7
S'\x16B=\xadd\xde\xed\xbf'
p3378
tp3379
Rp3380
ag3
(g7
S'\xacnF(\x95\xdb\xed\xbf'
p3381
tp3382
Rp3383
ag3
(g7
S'\x98\xd7M\x88\xbe\xc0\xd4\xbf'
p3384
tp3385
Rp3386
a(lp3387
F-0.9333976157741425
aF-0.9330545221923403
aF-0.32475884511202013
aF-0.3242641764730871
atp3388
a(F3.19
(lp3389
F-0.933224
aF-0.933224
aF-0.644241
a(lp3390
g3
(g7
S'\xd7\x88\x9b\xd5Q\xde\xed\xbf'
p3391
tp3392
Rp3393
ag3
(g7
S'\xd3\x1b_t\x9e\xdb\xed\xbf'
p3394
tp3395
Rp3396
ag3
(g7
S'\xc5\x9dZ\x82\xa6\xb8\xd4\xbf'
p3397
tp3398
Rp3399
a(lp3400
F-0.933388631059894
aF-0.9330589554673401
aF-0.3242457614034997
aF-0.323770167635726
atp3401
a(F3.2
(lp3402
F-0.933222
aF-0.933222
aF-0.64369
a(lp3403
g3
(g7
S'\xac\xc7\xae\xaf?\xde\xed\xbf'
p3404
tp3405
Rp3406
ag3
(g7
S'\xec\x98\xf4c\xa7\xdb\xed\xbf'
p3407
tp3408
Rp3409
ag3
(g7
S'd\r\xa7\xcf\x97\xb0\xd4\xbf'
p3410
tp3411
Rp3412
a(lp3413
F-0.9333799773505591
aF-0.9330632164244699
aF-0.3237355986302499
aF-0.32327838209694987
atp3414
a(F3.21
(lp3415
F-0.93322
aF-0.93322
aF-0.643145
a(lp3416
g3
(g7
S'\x84";5.\xde\xed\xbf'
p3417
tp3418
Rp3419
ag3
(g7
S'L\xf2o\xfa\xaf\xdb\xed\xbf'
p3420
tp3421
Rp3422
ag3
(g7
S'U\x10\xd8v\x92\xa8\xd4\xbf'
p3423
tp3424
Rp3425
a(lp3426
F-0.9333716430347309
aF-0.9330673114159903
aF-0.3232283390446504
aF-0.3227888260446477
atp3427
a(F3.2199999999999998
(lp3428
F-0.933218
aF-0.933218
aF-0.642607
a(lp3429
g3
(g7
S'\x1d\xaf9`\x1d\xde\xed\xbf'
p3430
tp3431
Rp3432
ag3
(g7
S'\xf3\x0b\x1c;\xb8\xdb\xed\xbf'
p3433
tp3434
Rp3435
ag3
(g7
S'\xd0K\xaf}\x96\xa0\xd4\xbf'
p3436
tp3437
Rp3438
a(lp3439
F-0.9333636168862289
aF-0.9330712465747405
aF-0.32272396483212057
aF-0.32230150483991066
atp3440
a(F3.23
(lp3441
F-0.933216
aF-0.933216
aF-0.642075
a(lp3442
g3
(g7
S'\xa4\xc8\xd6*\r\xde\xed\xbf'
p3443
tp3444
Rp3445
ag3
(g7
S'c\x94&)\xc0\xdb\xed\xbf'
p3446
tp3447
Rp3448
ag3
(g7
S'K~\x13\xe9\xa3\x98\xd4\xbf'
p3449
tp3450
Rp3451
a(lp3452
F-0.93335588805191
aF-0.9330750278210301
aF-0.32222245811948985
aF-0.32181642304746966
atp3453
a(F3.24
(lp3454
F-0.933214
aF-0.933214
aF-0.641549
a(lp3455
g3
(g7
S'np\xa0\x8f\xfd\xdd\xed\xbf'
p3456
tp3457
Rp3458
ag3
(g7
S'\xfb?\xd1\xc7\xc7\xdb\xed\xbf'
p3459
tp3460
Rp3461
ag3
(g7
S'>\xc8y\xbd\xba\x90\xd4\xbf'
p3462
tp3463
Rp3464
a(lp3465
F-0.9333484463891302
aF-0.9330786612208603
aF-0.32172380133444006
aF-0.32133358481871976
atp3466
a(F3.25
(lp3467
F-0.933212
aF-0.933212
aF-0.641029
a(lp3468
g3
(g7
S'\xac\xd3\xc4\x88\xee\xdd\xed\xbf'
p3469
tp3470
Rp3471
ag3
(g7
S'\x91\x90\xb1\x19\xcf\xdb\xed\xbf'
p3472
tp3473
Rp3474
ag3
(g7
S'\xb6\xf4h\xfd\xda\x88\xd4\xbf'
p3475
tp3476
Rp3477
a(lp3478
F-0.9333412810579953
aF-0.9330821515873301
aF-0.32122797580830975
aF-0.3208529925066833
atp3479
a(F3.26
(lp3480
F-0.93321
aF-0.93321
aF-0.640515
a(lp3481
g3
(g7
S'\xd6\xa20\x11\xe0\xdd\xed\xbf'
p3482
tp3483
Rp3484
ag3
(g7
S'\\g\xd3!\xd6\xdb\xed\xbf'
p3485
tp3486
Rp3487
ag3
(g7
S'\xa9\x1a\xc8\xab\x04\x81\xd4\xbf'
p3488
tp3489
Rp3490
a(lp3491
F-0.9333343826047786
aF-0.9330855045948108
aF-0.32073496389122985
aF-0.32037464881470074
atp3492
a(F3.27
(lp3493
F-0.933208
aF-0.933208
aF-0.640007
a(lp3494
g3
(g7
S'\xd4\xb3\xcd#\xd2\xdd\xed\xbf'
p3495
tp3496
Rp3497
ag3
(g7
S'\xda\xbe\xf8\xe2\xdc\xdb\xed\xbf'
p3498
tp3499
Rp3500
ag3
(g7
S'\xa4da\xca7y\xd4\xbf'
p3501
tp3502
Rp3503
a(lp3504
F-0.9333277415549843
aF-0.9330887253799705
aF-0.3202447475543904
aF-0.31989855540957496
atp3505
a(F3.2800000000000002
(lp3506
F-0.933207
aF-0.933207
aF-0.639506
a(lp3507
g3
(g7
S'H\x8f\xb1\xbb\xc4\xdd\xed\xbf'
p3508
tp3509
Rp3510
ag3
(g7
S'f\xc8\xca_\xe3\xdb\xed\xbf'
p3511
tp3512
Rp3513
ag3
(g7
S'\xf6pJZtq\xd4\xbf'
p3514
tp3515
Rp3516
a(lp3517
F-0.9333213487520673
aF-0.9330918188991406
aF-0.3197573087482402
aF-0.3194247133012729
atp3518
a(F3.29
(lp3519
F-0.933205
aF-0.933205
aF-0.63901
a(lp3520
g3
(g7
S'}\x0e\x1c\xd4\xb7\xdd\xed\xbf'
p3521
tp3522
Rp3523
ag3
(g7
S'm\xbb\xda\x9a\xe9\xdb\xed\xbf'
p3524
tp3525
Rp3526
ag3
(g7
S'.T\xeb[\xbai\xd4\xbf'
p3527
tp3528
Rp3529
a(lp3530
F-0.933315195347361
aF-0.9330947899342001
aF-0.31927262940929985
aF-0.31895312286843847
atp3531
a(F3.3
(lp3532
F-0.933204
aF-0.933204
aF-0.638519
a(lp3533
g3
(g7
S'\x90\x04vh\xab\xdd\xed\xbf'
p3534
tp3535
Rp3536
ag3
(g7
S'?\x9b\xa2\x96\xef\xdb\xed\xbf'
p3537
tp3538
Rp3539
ag3
(g7
S'th\x05\xcf\tb\xd4\xbf'
p3540
tp3541
Rp3542
a(lp3543
F-0.9333092727903404
aF-0.9330976430982004
aF-0.31879069146664024
aF-0.31848378388315896
atp3544
a(F3.31
(lp3545
F-0.933202
aF-0.933202
aF-0.638035
a(lp3546
g3
(g7
S'\x02\xf2Ot\x9f\xdd\xed\xbf'
p3547
tp3548
Rp3549
ag3
(g7
S'\xa3\xfc\x85U\xf5\xdb\xed\xbf'
p3550
tp3551
Rp3552
ag3
(g7
S'\x98\xde\xb9\xb2bZ\xd4\xbf'
p3553
tp3554
Rp3555
a(lp3556
F-0.9333035728191703
aF-0.9331003828409798
aF-0.3183114768481203
aF-0.3180166955348597
atp3557
a(F3.32
(lp3558
F-0.933201
aF-0.933201
aF-0.637556
a(lp3559
g3
(g7
S'\x02\xc3`\xf3\x93\xdd\xed\xbf'
p3560
tp3561
Rp3562
ag3
(g7
S'\xac\xbd\xd2\xd9\xfa\xdb\xed\xbf'
p3563
tp3564
Rp3565
ag3
(g7
S'>+\x90\x05\xc5R\xd4\xbf'
p3566
tp3567
Rp3568
a(lp3569
F-0.933298087451561
aF-0.9331030134543902
aF-0.31783496748635
aF-0.3175518564536789
atp3570
a(F3.33
(lp3571
F-0.933199
aF-0.933199
aF-0.637083
a(lp3572
g3
(g7
S'\x18\x95\x84\xe1\x88\xdd\xed\xbf'
p3573
tp3574
Rp3575
ag3
(g7
S'r\xc0\xc1%\x00\xdc\xed\xbf'
p3576
tp3577
Rp3578
ag3
(g7
S'|0|\xc50K\xd4\xbf'
p3579
tp3580
Rp3581
a(lp3582
F-0.933292808975837
aF-0.9331055390776004
aF-0.31736114532448007
aF-0.31708926473289173
atp3583
a(F3.34
(lp3584
F-0.933198
aF-0.933198
aF-0.636615
a(lp3585
g3
(g7
S'j\x89\xbb:~\xdd\xed\xbf'
p3586
tp3587
Rp3588
ag3
(g7
S'\xa4\x99w;\x05\xdc\xed\xbf'
p3589
tp3590
Rp3591
ag3
(g7
S':N\xe4\xef\xa5C\xd4\xbf'
p3592
tp3593
Rp3594
a(lp3595
F-0.9332877299423612
aF-0.9331079637020606
aF-0.31688999232178006
aF-0.31662891795096776
atp3596
a(F3.35
(lp3597
F-0.933197
aF-0.933197
aF-0.636152
a(lp3598
g3
(g7
S'\xec\x9e(\xfbs\xdd\xed\xbf'
p3599
tp3600
Rp3601
ag3
(g7
S'\xe2=\x05\x1d\n\xdc\xed\xbf'
p3602
tp3603
Rp3604
ag3
(g7
S'\x12,\xa7\x81$<\xd4\xbf'
p3605
tp3606
Rp3607
a(lp3608
F-0.9332828431551807
aF-0.9331102911764301
aF-0.3164214904588301
aF-0.3161708131926287
atp3609
a(F3.36
(lp3610
F-0.933195
aF-0.933195
aF-0.635695
a(lp3611
g3
(g7
S'b\x93\x10\x1fj\xdd\xed\xbf'
p3612
tp3613
Rp3614
ag3
(g7
S'J\xa7h\xcc\x0e\xdc\xed\xbf'
p3615
tp3616
Rp3617
ag3
(g7
S'\x10f!w\xac4\xd4\xbf'
p3618
tp3619
Rp3620
a(lp3621
F-0.9332781416638735
aF-0.9331125252112802
aF-0.3159556217427001
aF-0.3157149470694958
atp3622
a(F3.37
(lp3623
F-0.933194
aF-0.933194
aF-0.635244
a(lp3624
g3
(g7
S'\\\xd0\xd8\xa2`\xdd\xed\xbf'
p3625
tp3626
Rp3627
ag3
(g7
S'\x83v\x8dK\x13\xdc\xed\xbf'
p3628
tp3629
Rp3630
ag3
(g7
S'\xf1\x073\xcc=-\xd4\xbf'
p3631
tp3632
Rp3633
a(lp3634
F-0.9332736187557291
aF-0.9331146693836702
aF-0.3154923682117696
aF-0.31526131574002936
atp3635
a(F3.38
(lp3636
F-0.933193
aF-0.933193
aF-0.634797
a(lp3637
g3
(g7
S'\xf8]\x06\x83W\xdd\xed\xbf'
p3638
tp3639
Rp3640
ag3
(g7
S'\xf0\x90M\x9c\x17\xdc\xed\xbf'
p3641
tp3642
Rp3643
ag3
(g7
S'\xfb\xd9D|\xd8%\xd4\xbf'
p3644
tp3645
Rp3646
a(lp3647
F-0.9332692679481042
aF-0.9331167271416502
aF-0.3150317119404303
aF-0.31480991492881505
atp3648
a(F3.39
(lp3649
F-0.933192
aF-0.933192
aF-0.634356
a(lp3650
g3
(g7
S'\x92\xe1<\xbcN\xdd\xed\xbf'
p3651
tp3652
Rp3653
ag3
(g7
S'\\\xbaq\xc0\x1b\xdc\xed\xbf'
p3654
tp3655
Rp3656
ag3
(g7
S'\x8b\x8eM\x82|\x1e\xd4\xbf'
p3657
tp3658
Rp3659
a(lp3660
F-0.9332650829810963
aF-0.9331187018086203
aF-0.31457363504362
aF-0.3143607399453931
atp3661
a(F3.4
(lp3662
F-0.933191
aF-0.933191
aF-0.633919
a(lp3663
g3
(g7
S'\xeb\x9b=KF\xdd\xed\xbf'
p3664
tp3665
Rp3666
ag3
(g7
S'+!\xb2\xb9\x1f\xdc\xed\xbf'
p3667
tp3668
Rp3669
ag3
(g7
S'\x01\xb4\xd6\xd8)\x17\xd4\xbf'
p3670
tp3671
Rp3672
a(lp3673
F-0.933261057810224
aF-0.9331205965873204
aF-0.31411811968092
aF-0.3139137857022545
atp3674
a(F3.41
(lp3675
F-0.93319
aF-0.93319
aF-0.633488
a(lp3676
g3
(g7
S'\xdcz\xe6,>\xdd\xed\xbf'
p3677
tp3678
Rp3679
ag3
(g7
S'S\xf5\xb6\x89#\xdc\xed\xbf'
p3680
tp3681
Rp3682
ag3
(g7
S'\xef\x93\x01z\xe0\x0f\xd4\xbf'
p3683
tp3684
Rp3685
a(lp3686
F-0.9332571865996575
aF-0.9331224145641204
aF-0.3136651480608204
aF-0.3134690467325625
atp3687
a(F3.42
(lp3688
F-0.933189
aF-0.933189
aF-0.633061
a(lp3689
g3
(g7
S'\x88&1^6\xdd\xed\xbf'
p3690
tp3691
Rp3692
ag3
(g7
S"#\xed\x182'\xdc\xed\xbf"
p3693
tp3694
Rp3695
ag3
(g7
S'\xb8\xdc\x8b_\xa0\x08\xd4\xbf'
p3696
tp3697
Rp3698
a(lp3699
F-0.9332534637153037
aF-0.9331241587127904
aF-0.31321470244456995
aF-0.31302651720711633
atp3700
a(F3.4299999999999997
(lp3701
F-0.933188
aF-0.933188
aF-0.63264
a(lp3702
g3
(g7
S'\x12!2\xdc.\xdd\xed\xbf'
p3703
tp3704
Rp3705
ag3
(g7
S'\x8a\xcea\xb4*\xdc\xed\xbf'
p3706
tp3707
Rp3708
ag3
(g7
S'\r-\xd4\x82i\x01\xd4\xbf'
p3709
tp3710
Rp3711
a(lp3712
F-0.9332498837184473
aF-0.9331258318984101
aF-0.31276676514986984
aF-0.3125861909508816
atp3713
a(F3.44
(lp3714
F-0.933187
aF-0.933187
aF-0.632223
a(lp3715
g3
(g7
S";\xe1\x17\xa4'\xdd\xed\xbf"
p3716
tp3717
Rp3718
ag3
(g7
S'\xdb\xee\x0c\x12.\xdc\xed\xbf'
p3719
tp3720
Rp3721
ag3
(g7
S'\xdbr\xde\xdc;\xfa\xd3\xbf'
p3722
tp3723
Rp3724
a(lp3725
F-0.9332464413592221
aF-0.9331274368809905
aF-0.31232131855447
aF-0.31214806145889695
atp3726
a(F3.45
(lp3727
F-0.933186
aF-0.933186
aF-0.631811
a(lp3728
g3
(g7
S'\x00\x00*\xb3 \xdd\xed\xbf'
p3729
tp3730
Rp3731
ag3
(g7
S"'\xb3\x87L1\xdc\xed\xbf"
p3732
tp3733
Rp3734
ag3
(g7
S'(4Xf\x17\xf3\xd3\xbf'
p3735
tp3736
Rp3737
a(lp3738
F-0.9332431315706342
aF-0.9331289763191304
aF-0.31187834509959017
aF-0.3117121219118551
atp3739
a(F3.46
(lp3740
F-0.933185
aF-0.933185
aF-0.631404
a(lp3741
g3
(g7
S'\xdea\xc8\x06\x1a\xdd\xed\xbf'
p3742
tp3743
Rp3744
ag3
(g7
S'\xde\x062e4\xdc\xed\xbf'
p3745
tp3746
Rp3747
ag3
(g7
S'\xe6\xa2\x9c\x17\xfc\xeb\xd3\xbf'
p3748
tp3749
Rp3750
a(lp3751
F-0.933239949462457
aF-0.9331304527733802
aF-0.31143782729305997
aF-0.31127836519094254
atp3752
a(F3.4699999999999998
(lp3753
F-0.933184
aF-0.933184
aF-0.631001
a(lp3754
g3
(g7
S']oj\x9c\x13\xdd\xed\xbf'
p3755
tp3756
Rp3757
ag3
(g7
S'\x92\xd5^]7\xdc\xed\xbf'
p3758
tp3759
Rp3760
ag3
(g7
S'\x82\x9d\xb8\xe8\xe9\xe4\xd3\xbf'
p3761
tp3762
Rp3763
a(lp3764
F-0.9332368903155648
aF-0.9331318687097102
aF-0.3109997477124501
aF-0.3108467838923945
atp3765
a(F3.48
(lp3766
F-0.933184
aF-0.933184
aF-0.630603
a(lp3767
g3
(g7
S'\x82L\x9eq\r\xdd\xed\xbf'
p3768
tp3769
Rp3770
ag3
(g7
S'\xa9zT6:\xdc\xed\xbf'
p3771
tp3772
Rp3773
ag3
(g7
S't\x8bn\xd1\xe0\xdd\xd3\xbf'
p3774
tp3775
Rp3776
a(lp3777
F-0.9332339495762332
aF-0.9331332265026804
aF-0.3105640890080397
aF-0.31041737034154543
atp3778
a(F3.49
(lp3779
F-0.933183
aF-0.933183
aF-0.630209
a(lp3780
g3
(g7
S'\xe7\x1d\x08\x84\x07\xdd\xed\xbf'
p3781
tp3782
Rp3783
ag3
(g7
S'\xa63M\xf1<\xdc\xed\xbf'
p3784
tp3785
Rp3786
ag3
(g7
S'F\x11:\xc9\xe0\xd6\xd3\xbf'
p3787
tp3788
Rp3789
a(lp3790
F-0.9332311228508243
aF-0.9331345284386903
aF-0.31013083390548973
aF-0.30999011660630477
atp3791
a(F3.5
(lp3792
F-0.933182
aF-0.933182
aF-0.62982
a(lp3793
g3
(g7
S':Ja\xd1\x01\xdd\xed\xbf'
p3794
tp3795
Rp3796
ag3
(g7
S'\xb0\x86w\x8f?\xdc\xed\xbf'
p3797
tp3798
Rp3799
ag3
(g7
S'A\xb2S\xc7\xe9\xcf\xd3\xbf'
p3800
tp3801
Rp3802
a(lp3803
F-0.9332284059003719
aF-0.9331357767188904
aF-0.3096999652085499
aF-0.30956501451035773
atp3804
a(F3.51
(lp3805
F-0.933181
aF-0.933181
aF-0.629435
a(lp3806
g3
(g7
S'\xd8\xcawW\xfc\xdc\xed\xbf'
p3807
tp3808
Rp3809
ag3
(g7
S'k\xaf\xf6\x11B\xdc\xed\xbf'
p3810
tp3811
Rp3812
ag3
(g7
S'\xcdG\xb4\xc2\xfb\xc8\xd3\xbf'
p3813
tp3814
Rp3815
a(lp3816
F-0.9332257946355985
aF-0.9331369734622802
aF-0.30927146580151954
aF-0.30914205564579034
atp3817
a(F3.52
(lp3818
F-0.933181
aF-0.933181
aF-0.629055
a(lp3819
g3
(g7
S'\x0b{-\x14\xf7\xdc\xed\xbf'
p3820
tp3821
Rp3822
ag3
(g7
S'M\x01\xe3yD\xdc\xed\xbf'
p3823
tp3824
Rp3825
ag3
(g7
S'\xd1`\x18\xb2\x16\xc2\xd3\xbf'
p3826
tp3827
Rp3828
a(lp3829
F-0.9332232851118939
aF-0.9331381207085002
aF-0.30884531865160036
aF-0.3087212313853456
atp3830
a(F3.53
(lp3831
F-0.93318
aF-0.93318
aF-0.628679
a(lp3832
g3
(g7
S'\x16qw\x05\xf2\xdc\xed\xbf'
p3833
tp3834
Rp3835
ag3
(g7
S'^IJ\xc8F\xdc\xed\xbf'
p3836
tp3837
Rp3838
ag3
(g7
S'\xeb\x8a\x03\x8c:\xbb\xd3\xbf'
p3839
tp3840
Rp3841
a(lp3842
F-0.9332208735245635
aF-0.9331392204206105
aF-0.30842150681119
aF-0.30830253289438597
atp3843
a(F3.54
(lp3844
F-0.933179
aF-0.933179
aF-0.628307
a(lp3845
g3
(g7
S'\xc6W])\xed\xdc\xed\xbf'
p3846
tp3847
Rp3848
ag3
(g7
S'\x86,0\xfeH\xdc\xed\xbf'
p3849
tp3850
Rp3851
ag3
(g7
S'\x8bl\xc3Fg\xb4\xd3\xbf'
p3852
tp3853
Rp3854
a(lp3855
F-0.9332185562041035
aF-0.9331402744877703
aF-0.30800001341988986
aF-0.3078859511421759
atp3856
a(F3.55
(lp3857
F-0.933179
aF-0.933179
aF-0.627939
a(lp3858
g3
(g7
S'\xbc\xd3\xf8}\xe8\xdc\xed\xbf'
p3859
tp3860
Rp3861
ag3
(g7
S'r\x84\x8e\x1cK\xdc\xed\xbf'
p3862
tp3863
Rp3864
ag3
(g7
S'.\xd8r\xd8\x9c\xad\xd3\xbf'
p3865
tp3866
Rp3867
a(lp3868
F-0.9332163296118016
aF-0.9331412847278803
aF-0.30758082170654044
aF-0.3074714769130679
atp3869
a(F3.56
(lp3870
F-0.933178
aF-0.933178
aF-0.627575
a(lp3871
g3
(g7
S'T\xe6t\x01\xe4\xdc\xed\xbf'
p3872
tp3873
Rp3874
ag3
(g7
S'\xc6\xb5U$M\xdc\xed\xbf'
p3875
tp3876
Rp3877
ag3
(g7
S'\x91\xbd\xfc6\xdb\xa6\xd3\xbf'
p3878
tp3879
Rp3880
a(lp3881
F-0.9332141903352724
aF-0.9331422528900306
aF-0.30716391499113
aF-0.3070591008172066
atp3882
a(F3.57
(lp3883
F-0.933178
aF-0.933178
aF-0.627215
a(lp3884
g3
(g7
S'\xe0Z\r\xb2\xdf\xdc\xed\xbf'
p3885
tp3886
Rp3887
ag3
(g7
S'\xb7\x07m\x16O\xdc\xed\xbf'
p3888
tp3889
Rp3890
ag3
(g7
S'\xfe\xf8\x1eX"\xa0\xd3\xbf'
p3891
tp3892
Rp3893
a(lp3894
F-0.9332121350842858
aF-0.9331431806569898
aF-0.3067492766864495
aF-0.306648813300754
atp3895
a(F3.58
(lp3896
F-0.933177
aF-0.933177
aF-0.62686
a(lp3897
g3
(g7
S'\xd84\x0e\x8e\xdb\xdc\xed\xbf'
p3898
tp3899
Rp3900
ag3
(g7
S'\xb9\xf6\xb2\xf3P\xdc\xed\xbf'
p3901
tp3902
Rp3903
ag3
(g7
S'\x19\x16m1r\x99\xd3\xbf'
p3904
tp3905
Rp3906
a(lp3907
F-0.9332101606866224
aF-0.93314406964756
aF-0.30633689029983957
aF-0.30624060465592695
atp3908
a(F3.59
(lp3909
F-0.933177
aF-0.933177
aF-0.626508
a(lp3910
g3
(g7
S'J$\xd3\x93\xd7\xdc\xed\xbf'
p3911
tp3912
Rp3913
ag3
(g7
S'\xe7\x81\xfd\xbcR\xdc\xed\xbf'
p3914
tp3915
Rp3916
ag3
(g7
S'\xa5\xf1R\xb8\xca\x92\xd3\xbf'
p3917
tp3918
Rp3919
a(lp3920
F-0.9332082640841086
aF-0.9331449214187705
aF-0.3059267394346103
aF-0.3058344650305805
atp3921
a(F3.6
(lp3922
F-0.933176
aF-0.933176
aF-0.62616
a(lp3923
g3
(g7
S'$\xff\xc6\xc1\xd3\xdc\xed\xbf'
p3924
tp3925
Rp3926
ag3
(g7
S'W|\x1asT\xdc\xed\xbf'
p3927
tp3928
Rp3929
ag3
(g7
S'\x85L\x17\xe2+\x8c\xd3\xbf'
p3930
tp3931
Rp3932
a(lp3933
F-0.933206442328784
aF-0.9331457374681903
aF-0.3055188077916302
aF-0.30543038443756465
atp3934
a(F3.61
(lp3935
F-0.933176
aF-0.933176
aF-0.625816
a(lp3936
g3
(g7
S'\xaa=c\x16\xd0\xdc\xed\xbf'
p3937
tp3938
Rp3939
ag3
(g7
S'A\xd7\xcf\x16V\xdc\xed\xbf'
p3940
tp3941
Rp3942
ag3
(g7
S'd8\xde\xa3\x95\x85\xd3\xbf'
p3943
tp3944
Rp3945
a(lp3946
F-0.9332046925791714
aF-0.9331465192360402
aF-0.30511307917051955
aF-0.30502835276354795
atp3947
a(F3.62
(lp3948
F-0.933175
aF-0.933175
aF-0.625475
a(lp3949
g3
(g7
S'$z/\x90\xcc\xdc\xed\xbf'
p3950
tp3951
Rp3952
ag3
(g7
S'c\xe7\xdb\xa8W\xdc\xed\xbf'
p3953
tp3954
Rp3955
ag3
(g7
S'\xe4\x80\xab\xf2\x07\x7f\xd3\xbf'
p3956
tp3957
Rp3958
a(lp3959
F-0.9332030120966162
aF-0.9331472681071603
aF-0.30470953747097984
aF-0.3046283597777929
atp3960
a(F3.63
(lp3961
F-0.933175
aF-0.933175
aF-0.625139
a(lp3962
g3
(g7
S'\xba\xf6\xc0-\xc9\xdc\xed\xbf'
p3963
tp3964
Rp3965
ag3
(g7
S'\xda\xae\xf5)Y\xdc\xed\xbf'
p3966
tp3967
Rp3968
ag3
(g7
S'}\xecd\xc3\x82x\xd3\xbf'
p3969
tp3970
Rp3971
a(lp3972
F-0.9332013982418258
aF-0.9331479854131104
aF-0.30430816669387006
aF-0.3042303951403432
atp3973
a(F3.64
(lp3974
F-0.933174
aF-0.933174
aF-0.624806
a(lp3975
g3
(g7
S'\xfe&\xba\xed\xc5\xdc\xed\xbf'
p3976
tp3977
Rp3978
ag3
(g7
S'K \xcd\x9aZ\xdc\xed\xbf'
p3979
tp3980
Rp3981
ag3
(g7
S'vy\xd4\n\x06r\xd3\xbf'
p3982
tp3983
Rp3984
a(lp3985
F-0.933199848471502
aF-0.9331486724340807
aF-0.3039089509423603
aF-0.30383444841017754
atp3986
a(F3.65
(lp3987
F-0.933174
aF-0.933174
aF-0.624476
a(lp3988
g3
(g7
S'\x9f:\xca\xce\xc2\xdc\xed\xbf'
p3989
tp3990
Rp3991
ag3
(g7
S'\\_\x0b\xfc[\xdc\xed\xbf'
p3992
tp3993
Rp3994
ag3
(g7
S'Dw\xaa\xbd\x91k\xd3\xbf'
p3995
tp3996
Rp3997
a(lp3998
F-0.9331983603350018
aF-0.9331493304007203
aF-0.3035118744228203
aF-0.30344050905283765
atp3999
a(F3.66
(lp4000
F-0.933173
aF-0.933173
aF-0.62415
a(lp4001
g3
(g7
S'p\xad\xac\xcf\xbf\xdc\xed\xbf'
p4002
tp4003
Rp4004
ag3
(g7
S'\x0c\x00SN]\xdc\xed\xbf'
p4005
tp4006
Rp4007
ag3
(g7
S')\x97\x7f\xd0%e\xd3\xbf'
p4008
tp4009
Rp4010
a(lp4011
F-0.9331969314711557
aF-0.9331499604959402
aF-0.30311692144577995
aF-0.3030485664479434
atp4012
a(F3.67
(lp4013
F-0.933173
aF-0.933173
aF-0.623828
a(lp4014
g3
(g7
S'\x10\xdd(\xef\xbc\xdc\xed\xbf'
p4015
tp4016
Rp4017
ag3
(g7
S'\x1cD@\x92^\xdc\xed\xbf'
p4018
tp4019
Rp4020
ag3
(g7
S'\xa8\xe2\xd67\xc2^\xd3\xbf'
p4021
tp4022
Rp4023
a(lp4024
F-0.9331955596052537
aF-0.9331505638566603
aF-0.3027240764266602
aF-0.3026586098963355
atp4025
a(F3.68
(lp4026
F-0.933173
aF-0.933173
aF-0.623509
a(lp4027
g3
(g7
S'\x06\xa0\x11,\xba\xdc\xed\xbf'
p4028
tp4029
Rp4030
ag3
(g7
S'\x8dYi\xc8_\xdc\xed\xbf'
p4031
tp4032
Rp4033
ag3
(g7
S'\xea\xa2\x1f\xe8fX\xd3\xbf'
p4034
tp4035
Rp4036
a(lp4037
F-0.9331942425460514
aF-0.9331511415755799
aF-0.3023333238866201
aF-0.3022706286269982
atp4038
a(F3.69
(lp4039
F-0.933172
aF-0.933172
aF-0.623194
a(lp4040
g3
(g7
S'Y\xdbD\x85\xb7\xdc\xed\xbf'
p4041
tp4042
Rp4043
ag3
(g7
S'\xcb\x8c^\xf1`\xdc\xed\xbf'
p4044
tp4045
Rp4046
ag3
(g7
S'\xce0\xb7\xd5\x13R\xd3\xbf'
p4047
tp4048
Rp4049
a(lp4050
F-0.9331929781827553
aF-0.9331516947026107
aF-0.3019446484531098
aF-0.30188461180365433
atp4051
a(F3.7
(lp4052
F-0.933172
aF-0.933172
aF-0.622882
a(lp4053
g3
(g7
S'\xce&\xab\xf9\xb4\xdc\xed\xbf'
p4054
tp4055
Rp4056
ag3
(g7
S'\xa0\x86\xaa\rb\xdc\xed\xbf'
p4057
tp4058
Rp4059
ag3
(g7
S'\xae\xba\xea\xf4\xc8K\xd3\xbf'
p4060
tp4061
Rp4062
a(lp4063
F-0.9331917644824097
aF-0.9331522242466301
aF-0.30155803486052957
aF-0.30150054853121916
atp4064
a(F3.71
(lp4065
F-0.933172
aF-0.933172
aF-0.622573
a(lp4066
g3
(g7
S'\xf6j7\x88\xb2\xdc\xed\xbf'
p4067
tp4068
Rp4069
ag3
(g7
S'\xa1\x7f\xd2\x1dc\xdc\xed\xbf'
p4070
tp4071
Rp4072
ag3
(g7
S'\x94\xf2\xf89\x86E\xd3\xbf'
p4073
tp4074
Rp4075
a(lp4076
F-0.9331905994871175
aF-0.9331527311769505
aF-0.3011734679507303
aF-0.30111842786190207
atp4077
a(F3.7199999999999998
(lp4078
F-0.933171
aF-0.933171
aF-0.622268
a(lp4079
g3
(g7
S'\xf2\x83\xe6/\xb0\xdc\xed\xbf'
p4080
tp4081
Rp4082
ag3
(g7
S'\x0frV"d\xdc\xed\xbf'
p4083
tp4084
Rp4085
ag3
(g7
S'\x8c\xaf\x13\x99K?\xd3\xbf'
p4086
tp4087
Rp4088
a(lp4089
F-0.9331894813113863
aF-0.9331532164247301
aF-0.3007909326734898
aF-0.30073823880115286
atp4090
a(F3.73
(lp4091
F-0.933171
aF-0.933171
aF-0.621965
a(lp4092
g3
(g7
S'A\xe9\xbe\xef\xad\xdc\xed\xbf'
p4093
tp4094
Rp4095
ag3
(g7
S'GL\xb1\x1be\xdc\xed\xbf'
p4096
tp4097
Rp4098
ag3
(g7
S'\xceya\x06\x199\xd3\xbf'
p4099
tp4100
Rp4101
a(lp4102
F-0.9331884081396207
aF-0.9331536808844101
aF-0.30041041408684976
aF-0.30035997031327827
atp4103
a(F3.74
(lp4104
F-0.933171
aF-0.933171
aF-0.621666
a(lp4105
g3
(g7
S'pY\xd0\xc6\xab\xdc\xed\xbf'
p4106
tp4107
Rp4108
ag3
(g7
S'\x97#Y\nf\xdc\xed\xbf'
p4109
tp4110
Rp4111
ag3
(g7
S'\xda\x0f\xffu\xee2\xd3\xbf'
p4112
tp4113
Rp4114
a(lp4115
F-0.9331873782237331
aF-0.9331541254151605
aF-0.30003189735753966
aF-0.2999836113269766
atp4116
a(F3.75
(lp4117
F-0.93317
aF-0.93317
aF-0.62137
a(lp4118
g3
(g7
S'\xc8\x823\xb4\xa9\xdc\xed\xbf'
p4119
tp4120
Rp4121
ag3
(g7
S'H^\xbf\xeef\xdc\xed\xbf'
p4122
tp4123
Rp4124
ag3
(g7
S'\x86\xd2\x00\xdc\xcb,\xd3\xbf'
p4125
tp4126
Rp4127
a(lp4128
F-0.9331863898806534
aF-0.93315455084207
aF-0.29965536776119
aF-0.29960915074051564
atp4129
a(F3.76
(lp4130
F-0.93317
aF-0.93317
aF-0.621077
a(lp4131
g3
(g7
S'D\xb6\t\xb7\xa7\xdc\xed\xbf'
p4132
tp4133
Rp4134
ag3
(g7
S'\x1e\xe4P\xc9g\xdc\xed\xbf'
p4135
tp4136
Rp4137
ag3
(g7
S"\xaa't,\xb1&\xd3\xbf"
p4138
tp4139
Rp4140
a(lp4141
F-0.9331854414901467
aF-0.9331549579575302
aF-0.2992808106825498
aF-0.29923657742676335
atp4142
a(F3.77
(lp4143
F-0.93317
aF-0.93317
aF-0.620788
a(lp4144
g3
(g7
S'\xe2\x96|\xce\xa5\xdc\xed\xbf'
p4145
tp4146
Rp4147
ag3
(g7
S'\x1cGv\x9ah\xdc\xed\xbf'
p4148
tp4149
Rp4150
ag3
(g7
S'\xec\xce`[\x9e \xd3\xbf'
p4151
tp4152
Rp4153
a(lp4154
F-0.933184531492511
aF-0.9331553475223904
aF-0.29890821161569014
aF-0.29886588023803856
atp4155
a(F3.78
(lp4156
F-0.93317
aF-0.93317
aF-0.620501
a(lp4157
g3
(g7
S'\x15\xd1\xbd\xf9\xa3\xdc\xed\xbf'
p4158
tp4159
Rp4160
ag3
(g7
S'A\xf0\x93bi\xdc\xed\xbf'
p4161
tp4162
Rp4163
ag3
(g7
S'\xa4%\xca\\\x93\x1a\xd3\xbf'
p4164
tp4165
Rp4166
a(lp4167
F-0.933183658386527
aF-0.9331557202672304
aF-0.2985375561640898
aF-0.29849704801071186
atp4168
a(F3.79
(lp4169
F-0.933169
aF-0.933169
aF-0.620217
a(lp4170
g3
(g7
S'd\xce\x068\xa2\xdc\xed\xbf'
p4171
tp4172
Rp4173
ag3
(g7
S'\xc4C\n"j\xdc\xed\xbf'
p4174
tp4175
Rp4176
ag3
(g7
S'\xa9`\xb0$\x90\x14\xd3\xbf'
p4177
tp4178
Rp4179
a(lp4180
F-0.9331828207272781
aF-0.9331560768933905
aF-0.2981688300407098
aF-0.29813006956966104
atp4181
a(F3.8
(lp4182
F-0.933169
aF-0.933169
aF-0.619936
a(lp4183
g3
(g7
S'\xe9o\x98\x88\xa0\xdc\xed\xbf'
p4184
tp4185
Rp4186
ag3
(g7
S'F\xcb5\xd9j\xdc\xed\xbf'
p4187
tp4188
Rp4189
ag3
(g7
S'\x06\xb4\x11\xa7\x94\x0e\xd3\xbf'
p4190
tp4191
Rp4192
a(lp4193
F-0.9331820171241785
aF-0.9331564180741705
aF-0.29780201906802967
aF-0.2977649337324809
atp4194
a(F3.81
(lp4195
F-0.933169
aF-0.933169
aF-0.619658
a(lp4196
g3
(g7
S'4\xcd\xba\xea\x9e\xdc\xed\xbf'
p4197
tp4198
Rp4199
ag3
(g7
S'\xcaZo\x88k\xdc\xed\xbf'
p4200
tp4201
Rp4202
ag3
(g7
S'\xb9u\xeb\xd7\xa0\x08\xd3\xbf'
p4203
tp4204
Rp4205
a(lp4206
F-0.9331812462391212
aF-0.9331567444558804
aF-0.2974371091779798
aF-0.29740162931360803
atp4207
a(F3.82
(lp4208
F-0.933169
aF-0.933169
aF-0.619383
a(lp4209
g3
(g7
S'\xa9\xec\xbc]\x9d\xdc\xed\xbf'
p4210
tp4211
Rp4212
ag3
(g7
S'53\x0c0l\xdc\xed\xbf'
p4213
tp4214
Rp4215
ag3
(g7
S'y+;\xab\xb4\x02\xd3\xbf'
p4216
tp4217
Rp4218
a(lp4219
F-0.9331805067844432
aF-0.93315705665882
aF-0.29707408641191985
aF-0.2970401451281564
atp4220
a(F3.83
(lp4221
F-0.933169
aF-0.933169
aF-0.61911
a(lp4222
g3
(g7
S'.\x88\xf4\xe0\x9b\xdc\xed\xbf'
p4223
tp4224
Rp4225
ag3
(g7
S"-'^\xd0l\xdc\xed\xbf"
p4226
tp4227
Rp4228
ag3
(g7
S'\x86\x92\xff\x14\xd0\xfc\xd2\xbf'
p4229
tp4230
Rp4231
a(lp4232
F-0.9331797975212373
aF-0.9331573552783301
aF-0.2967129369204898
aF-0.29668046999567155
atp4233
a(F3.84
(lp4234
F-0.933168
aF-0.933168
aF-0.618841
a(lp4235
g3
(g7
S'\x06\xce\xbds\x9a\xdc\xed\xbf'
p4236
tp4237
Rp4238
ag3
(g7
S'\x80\xbb\xb3im\xdc\xed\xbf'
p4239
tp4240
Rp4241
ag3
(g7
S'W\x9a9\t\xf3\xf6\xd2\xbf'
p4242
tp4243
Rp4244
a(lp4245
F-0.9331791172575664
aF-0.93315764088571
aF-0.2963536469634492
aF-0.29632259274368283
atp4246
a(F3.85
(lp4247
F-0.933168
aF-0.933168
aF-0.618574
a(lp4248
g3
(g7
S'\xd7${\x15\x99\xdc\xed\xbf'
p4249
tp4250
Rp4251
ag3
(g7
S'\x9dHX\xfcm\xdc\xed\xbf'
p4252
tp4253
Rp4254
ag3
(g7
S'\xecV\xed{\x1d\xf1\xd2\xbf'
p4255
tp4256
Rp4257
a(lp4258
F-0.9331784648467428
aF-0.9331579140291706
aF-0.2959962029095905
aF-0.29596650221115683
atp4259
a(F3.86
(lp4260
F-0.933168
aF-0.933168
aF-0.618309
a(lp4261
g3
(g7
S'\t\xf3\x94\xc5\x97\xdc\xed\xbf'
p4262
tp4263
Rp4264
ag3
(g7
S'\xe7\x19\x94\x88n\xdc\xed\xbf'
p4265
tp4266
Rp4267
ag3
(g7
S'\x13\xe1"aO\xeb\xd2\xbf'
p4268
tp4269
Rp4270
a(lp4271
F-0.9331778391857307
aF-0.9331581752347204
aF-0.2956405912363998
aF-0.2956121872516783
atp4272
a(F3.87
(lp4273
F-0.933168
aF-0.933168
aF-0.618048
a(lp4274
g3
(g7
S'Hey\x83\x96\xdc\xed\xbf'
p4275
tp4276
Rp4277
ag3
(g7
S'\xa0\x88\xac\x0eo\xdc\xed\xbf'
p4278
tp4279
Rp4280
ag3
(g7
S'\x162\xe7\xac\x88\xe5\xd2\xbf'
p4281
tp4282
Rp4283
a(lp4284
F-0.9331772392135135
aF-0.9331584250069399
aF-0.29528679852979955
aF-0.29525963673657557
atp4285
a(F3.88
(lp4286
F-0.933168
aF-0.933168
aF-0.617789
a(lp4287
g3
(g7
S'H;\x9cN\x95\xdc\xed\xbf'
p4288
tp4289
Rp4290
ag3
(g7
S'\x9c\x1e\xe4\x8eo\xdc\xed\xbf'
p4291
tp4292
Rp4293
ag3
(g7
S'_\xf6LS\xc9\xdf\xd2\xbf'
p4294
tp4295
Rp4296
a(lp4297
F-0.9331766639096284
aF-0.9331586638299602
aF-0.2949348114839597
aF-0.2949088395579111
atp4298
a(F3.89
(lp4299
F-0.933168
aF-0.933168
aF-0.617532
a(lp4300
g3
(g7
S'\x10\x92v&\x94\xdc\xed\xbf'
p4301
tp4302
Rp4303
ag3
(g7
S'\xbb\xadz\tp\xdc\xed\xbf'
p4304
tp4305
Rp4306
ag3
(g7
S'\xf6OmH\x11\xda\xd2\xbf'
p4307
tp4308
Rp4309
a(lp4310
F-0.9331761122926441
aF-0.9331588921681302
aF-0.2945846169008499
aF-0.2945597846312455
atp4311
a(F3.9
(lp4312
F-0.933167
aF-0.933167
aF-0.617278
a(lp4313
g3
(g7
S'\xf2\xb2\x86\n\x93\xdc\xed\xbf'
p4314
tp4315
Rp4316
ag3
(g7
S'\xddm\xad~p\xdc\xed\xbf'
p4317
tp4318
Rp4319
ag3
(g7
S'\xe6\x9bh\x80`\xd4\xd2\xbf'
p4320
tp4321
Rp4322
a(lp4323
F-0.9331755834187713
aF-0.9331591104668703
aF-0.2942362016900498
aF-0.2942124608984484
atp4324
a(F3.91
(lp4325
F-0.933167
aF-0.933167
aF-0.617027
a(lp4326
g3
(g7
S'B\xe1O\xfa\x91\xdc\xed\xbf'
p4327
tp4328
Rp4329
ag3
(g7
S'\x8d\x13\xb7\xeep\xdc\xed\xbf'
p4330
tp4331
Rp4332
ag3
(g7
S'\xec\x1bg\xef\xb6\xce\xd2\xbf'
p4333
tp4334
Rp4335
a(lp4336
F-0.9331750763804288
aF-0.9331593191533204
aF-0.29388955286817986
aF-0.2938668573301004
atp4337
a(F3.92
(lp4338
F-0.933167
aF-0.933167
aF-0.616778
a(lp4339
g3
(g7
S'P.Z\xf5\x90\xdc\xed\xbf'
p4340
tp4341
Rp4342
ag3
(g7
S'\xd7\xec\xcfYq\xdc\xed\xbf'
p4343
tp4344
Rp4345
ag3
(g7
S'\x90\xa9\x99\x89\x14\xc9\xd2\xbf'
p4346
tp4347
Rp4348
a(lp4349
F-0.933174590304995
aF-0.9331595186371502
aF-0.2935446575586298
aF-0.29352296292804486
atp4350
a(F3.93
(lp4351
F-0.933167
aF-0.933167
aF-0.616531
a(lp4352
g3
(g7
S'VI2\xfb\x8f\xdc\xed\xbf'
p4353
tp4354
Rp4355
ag3
(g7
S'\xdd\xf6-\xc0q\xdc\xed\xbf'
p4356
tp4357
Rp4358
ag3
(g7
S'CV:Cy\xc3\xd2\xbf'
p4359
tp4360
Rp4361
a(lp4362
F-0.9331741243534373
aF-0.9331597093111802
aF-0.29320150299110015
aF-0.2931807667276621
atp4363
a(F3.94
(lp4364
F-0.933167
aF-0.933167
aF-0.616287
a(lp4365
g3
(g7
S'\xd2Vi\x0b\x8f\xdc\xed\xbf'
p4366
tp4367
Rp4368
ag3
(g7
S'&\xf6\x04"r\xdc\xed\xbf'
p4369
tp4370
Rp4371
ag3
(g7
S'\x81\x07\x8d\x10\xe5\xbd\xd2\xbf'
p4372
tp4373
Rp4374
a(lp4375
F-0.9331736777191629
aF-0.9331598915520705
aF-0.2928600765011102
aF-0.2928402578000869
atp4376
a(F3.95
(lp4377
F-0.933167
aF-0.933167
aF-0.616045
a(lp4378
g3
(g7
S'\xd4\xc3\x94%\x8e\xdc\xed\xbf'
p4379
tp4380
Rp4381
ag3
(g7
S'+\x8d\x86\x7fr\xdc\xed\xbf'
p4382
tp4383
Rp4384
ag3
(g7
S'S\x08\xe0\xe5W\xb8\xd2\xbf'
p4385
tp4386
Rp4387
a(lp4388
F-0.9331732496267419
aF-0.9331600657209604
aF-0.2925203655295801
aF-0.2925014252542771
atp4389
a(F3.96
(lp4390
F-0.933167
aF-0.933167
aF-0.615806
a(lp4391
g3
(g7
S'\x9b\x1eNI\x8d\xdc\xed\xbf'
p4392
tp4393
Rp4394
ag3
(g7
S'\x13P\xe2\xd8r\xdc\xed\xbf'
p4395
tp4396
Rp4397
ag3
(g7
S'Y\x95\x8c\xb7\xd1\xb2\xd2\xbf'
p4398
tp4399
Rp4400
a(lp4401
F-0.9331728393307968
aF-0.9331602321640303
aF-0.2921823576222499
aF-0.29216425823900277
atp4402
a(F3.97
(lp4403
F-0.933166
aF-0.933166
aF-0.615568
a(lp4404
g3
(g7
S',\xef2v\x8c\xdc\xed\xbf'
p4405
tp4406
Rp4407
ag3
(g7
S'B\xddE.s\xdc\xed\xbf'
p4408
tp4409
Rp4410
ag3
(g7
S'[`\xf7yR\xad\xd2\xbf'
p4411
tp4412
Rp4413
a(lp4414
F-0.9331724461148715
aF-0.9331603912132004
aF-0.29184604042926005
aF-0.2918287459447178
atp4415
a(F3.98
(lp4416
F-0.933166
aF-0.933166
aF-0.615333
a(lp4417
g3
(g7
S'#\x92\xe4\xab\x8b\xdc\xed\xbf'
p4418
tp4419
Rp4420
ag3
(g7
S'+\xec\xdc\x7fs\xdc\xed\xbf'
p4421
tp4422
Rp4423
ag3
(g7
S'C\x10\x91!\xda\xa7\xd2\xbf'
p4424
tp4425
Rp4426
a(lp4427
F-0.9331720692903819
aF-0.9331605431865503
aF-0.29151140170455003
aF-0.29149487760537757
atp4428
a(F3.99
(lp4429
F-0.933166
aF-0.933166
aF-0.615101
a(lp4430
g3
(g7
S'\xce\x12\x08\xea\x8a\xdc\xed\xbf'
p4431
tp4432
Rp4433
ag3
(g7
S'\x8be\xd1\xcds\xdc\xed\xbf'
p4434
tp4435
Rp4436
ag3
(g7
S'\x98\xb0\xd6\xa2h\xa2\xd2\xbf'
p4437
tp4438
Rp4439
a(lp4440
F-0.9331717081955393
aF-0.9331606883890102
aF-0.2911784293052898
aF-0.2911626425000209
atp4441
a(F4.0
(lp4442
F-0.933166
aF-0.933166
aF-0.61487
a(lp4443
g3
(g7
S'\xc2\x08F0\x8a\xdc\xed\xbf'
p4444
tp4445
Rp4446
ag3
(g7
S'\xa0rK\x18t\xdc\xed\xbf'
p4447
tp4448
Rp4449
ag3
(g7
S'u(R\xf2\xfd\x9c\xd2\xbf'
p4450
tp4451
Rp4452
a(lp4453
F-0.9331713621943653
aF-0.9331608271127902
aF-0.2908471111913699
aF-0.2908320299544645
atp4454
a(F4.1
(lp4455
F-0.933165
aF-0.933165
aF-0.612677
a(lp4456
g3
(g7
S'\xff\xb0/j\x84\xdc\xed\xbf'
p4457
tp4458
Rp4459
ag3
(g7
S'\x85m\xeb_v\xdc\xed\xbf'
p4460
tp4461
Rp4462
ag3
(g7
S'%\x9d\t\xa8?h\xd2\xbf'
p4463
tp4464
Rp4465
a(lp4466
F-0.9331686090422688
aF-0.9331619141989205
aF-0.2876223391209399
aF-0.2876128331176505
atp4467
a.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

SHELL = /bin/bash
LATEX	= latex
PDFLATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdf
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]+begin\{document\}' *.tex)
STY	:= $(wildcard *.sty)
SRCDEP	:= $(shell egrep -l '^[^%]+begin\{document\}' */*.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);echo "$(LATEX) $<";$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	$(COPY);echo "$(PDFLATEX) $<";$(PDFLATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]+(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]+bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define getstys
	stys=`perl -ne '($$_)=/^[^%]+usepackage\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {if(-e "$$b.sty") {print "$$b.d ";}}' $< $$deps;perl -ne '($$_)=/^[^%]+usetheme\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {if(-e "beamertheme$$b.sty") {print "beamertheme$$b.d ";}}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]+(includegraphics|psfig)(\<.*?\>)?(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[$$#foo])) { if ($$foo[$$#foo] =~ /.eps$$/) { print "$$foo[$$#foo] "; } else { print "$$foo[$$#foo].eps "; }}' $< $$deps`
endef

define getepsgpis
	echo $< $$deps
	`perl -e '%files=();                                                                        \
                        while(<>)                                                                  \
                        {                                                                          \
                           @foo=/^[^%]+(includegraphics|psfig)(\<.*?\>)?(\[.*?\])?\{(.*?)\}/g;  \
                           if (defined($$foo[$$#foo]))                                                  \
                           {                                                                       \
                              $$fn=$$foo[$$#foo];                                                  \
                              if ($$fn =~ /.eps$$/) { $$fn="$$fn"; }                 \
                              else { $$fn="$$fn.eps"; }                                        \
                              if($$fn=~/(^.*)--.*\.eps/) {if(!exists($$files{$$1})) {$$files{$$1}=[];}  \
                                                     push @{$$files{$$1}},$$fn;}                   \
                           }                                                                       \
                        }                                                                          \
                        for $$i (keys(%files)) { print join(" ",@{$$files{$$i}}),": ",$$i,".Mgpi\n";}      \
                        ' $< $$deps >>$@`
endef

define getepspys
	echo $< $$deps
	`perl -e '%files={};                                                                        \
                        while(<>)                                                                  \
                        {                                                                          \
                           @foo=/^[^%]*\\\(includegraphics|psfig)(\<.*?\>)?(\[.*?\])?\{(.*?)\}/g;  \
                           if (defined($$foo[$$#foo]))                                                  \
                           {                                                                       \
                              $$fn=$$foo[$$#foo];                                                  \
                              if ($$fn =~ /.eps$$/) { $$fn="$$fn"; }                 \
                              else { $$fn="$$fn.eps"; }                                        \
                              if($$fn=~/(^.*)-_.*\.eps/) {if(!exists($$files{$$1})) {$$files{$$1}=[];}  \
                                                     push @{$$files{$$1}},$$fn;}                   \
                           }                                                                       \
                        }                                                                          \
                        for $$i (keys(%files)) { print join(" ",@{$$files{$$i}}),": ",$$i,".Mpy\n";}      \
                        ' $< $$deps >>$@`
endef

define getpdfs
	pdfs=`perl -ne '@foo=/^[^%]+(includegraphics|psfig)(\<.*?\>)?(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[$$#foo])) { if ($$foo[$$#foo] =~ /.pdf$$/) { print "$$foo[$$#foo] "; } else { print "$$foo[$$#foo].pdf "; }}' $< $$deps`
endef





define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

all 	: $(TRG)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d) $(TRG:%.dvi=%.end)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo "Dependencies: " $$deps ; \
	$(getbibs) ; echo "Bibs: " $$bibs ; \
	$(geteps) ; echo "EPSes: " $$epses ; \
	$(getstys) ; echo "STYs: " $$stys ; \
	$(getpdfs) ; echo "PDFs: " $$pdfs ; \
	$(manconf) ; echo  "Mandeps: " $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$stys $$mandeps" > $@ ;\
	echo "$*.pdf : $< $$pdfs $$deps $$bibs $$epses $$stys $$mandeps" >> $@ 
	$(getepsgpis)
	$(getepspys)

%.d	: %.sty
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(geteps) ; echo $$epses ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 
	$(getepsgpis)
	$(getepspys)

include $(SRC:.tex=.d)
include $(STY:.sty=.d)

#%-0.eps %-1.eps %-2.eps %-3.eps %-4.eps %-5.eps %-6.eps %-7.eps %-8.eps %-9.eps : %.gpi
#	cd ${@D}; \
#	gnuplot $(notdir $<)

%.Mgpi: %.gpi
	cd ${@D}; \
	gnuplot $(notdir $<)
	touch $@

%.Mpy: %.py
	cd ${@D}; \
	python $(notdir $<)
	touch $@

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@

#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) $<
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
$(PDF) : %.pdf : %.tex
	@$(run-pdflatex)
	echo $@ |grep fig >/dev/null; if [ $$? == 0 ]; then pdfcrop $@ tmp.pdf; cp tmp.pdf $@; fi


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
%.eps: %.sh
	cd ${@D}; \
	./$(@F:.eps=.sh)
%.eps: %.svg
	inkscape -E $@ $(@:.eps=.svg)
%.eps: %.png
	convert -compress zip $(@:.eps=.png) eps3:$@
%.eps: %.tga
	convert -compress zip $(@:.eps=.tga) eps3:$@
%.eps: %.jpeg
	convert -compress zip $(@:.eps=.jpeg) eps3:$@
%.eps: %.dvi
	dvips -E -o $@ $(@:.eps=.dvi)
%.eps: %.fig
	fig2dev -L eps $(@:.eps=.fig) $@
%.png: %.gpx
	 cd ${@D}; \
	 gnuplot $(@F:.png=.gpx)  >$(@F)
%.png: %.xyz
	 cd ${@D}; \
	 ./makemos.sh $(@F:.png=.gpi)  >$(@F)
%.eps: %.gpx
	 cd ${@D}; \
	 gnuplot $(@F:.eps=.gpx)  >$(@F)
%.eps: %.gpi
	 cd ${@D}; \
	 gnuplot $(@F:.eps=.gpi)
#%.eps: %.pdf
#	 cd ${@D}; \
#	 pdf2ps $(@F:.eps=.pdf) $(@F)
%.pdf: %.eps
	 cd ${@D}; \
	 epstopdf $(@F:.pdf=.eps)
%.eps: %.py
	 cd ${@D}; \
	 python $(@F:.eps=.py)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))

